BindAdapt: Joint Camera-Computation Scheduling for Persistent Target Identity in PTZ Tracking

Pan-tilt-zoom (PTZ) tracking can maintain a confident bounding box while following the wrong person. Recovering the designated identity depends on when verification results become available, because tracker memory continues to change while computation is pending. In controlled crossings, delaying the same identity check from before to after a crossing reduces two-second identity retention from 94.2% to 56.8%. We propose BindAdapt, which jointly schedules camera motion, visual operators, and operator start times to preserve target identity under computation and motion budgets. A provenance graph records the shared origins of observations and tracker-memory cues. An identity-response model, trained on paired rendered branches from the same tracker state, predicts result return times and subsequent identity-binding trajectories. A receding-horizon scheduler uses these predictions to select timed actions that minimize expected identity loss. Across 480 PTZ episodes rendered from panoramas, BindAdapt increases correct-target tracking time from 75.2% to 82.3% and reduces wrong binding from 7.3% to 4.4% over DAM4SAM with Chanakya-J at matched service time. Gains persist across three fixed tracking backbones and without artificial delay. On a real PTZ camera, identity success improves from 74.8% with Chanakya-J to 80.3%.

==> numbers_v45.tex <==
\expandafter\def\csname BAval@t17.r01.dam4sam.chanakya.j\endcsname{80.1}
\expandafter\def\csname BAval@t17.r01.bindadapt\endcsname{84.2}
\expandafter\def\csname BAval@t17.r02.dam4sam.chanakya.j\endcsname{79.4}
\expandafter\def\csname BAval@t17.r02.bindadapt\endcsname{84.1}
\expandafter\def\csname BAval@t17.r03.dam4sam.chanakya.j\endcsname{77.8}
\expandafter\def\csname BAval@t17.r03.bindadapt\endcsname{83.5}
\expandafter\def\csname BAval@t17.r04.dam4sam.chanakya.j\endcsname{75.2}
\expandafter\def\csname BAval@t17.r04.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t17.r05.dam4sam.chanakya.j\endcsname{68.5}
\expandafter\def\csname BAval@t17.r05.bindadapt\endcsname{78.1}
\expandafter\def\csname BAval@t17.r06.dam4sam.chanakya.j\endcsname{54.8}
\expandafter\def\csname BAval@t17.r06.bindadapt\endcsname{67.0}
\expandafter\def\csname BAval@delta.sweep.zero\endcsname{4.1}
\expandafter\def\csname BAval@delta.sweep.ref\endcsname{7.1}
\expandafter\def\csname BAval@delta.sweep.two\endcsname{12.2}
\expandafter\def\csname BAval@svc.direct.sid\endcsname{81.3}
\expandafter\def\csname BAval@svc.recal.sid\endcsname{83.6}
\expandafter\def\csname BAval@svc.retrain.sid\endcsname{84.0}
\expandafter\def\csname BAval@delta.svc.recal\endcsname{2.3}
\expandafter\def\csname BAval@delta.svc.retrain\endcsname{0.4}
\expandafter\def\csname BAval@delta.svc.gap\endcsname{2.7}


==> supp_numbers.tex <==
\providecommand{\BAval}[1]{\ifcsname BAval@#1\endcsname\csname BAval@#1\endcsname\else\PackageError{BindAdapt}{Unknown numeric ledger key #1}{}\fi}
\expandafter\def\csname BAval@t01.r01.sid\endcsname{44.0}
\expandafter\def\csname BAval@t01.r01.wrong\endcsname{19.8}
\expandafter\def\csname BAval@t01.r01.recovery\endcsname{42.0}
\expandafter\def\csname BAval@t01.r01.t5\endcsname{3.8}
\expandafter\def\csname BAval@t01.r02.sid\endcsname{58.2}
\expandafter\def\csname BAval@t01.r02.wrong\endcsname{15.3}
\expandafter\def\csname BAval@t01.r02.recovery\endcsname{56.0}
\expandafter\def\csname BAval@t01.r02.t5\endcsname{3.2}
\expandafter\def\csname BAval@t01.r03.sid\endcsname{55.6}
\expandafter\def\csname BAval@t01.r03.wrong\endcsname{17.0}
\expandafter\def\csname BAval@t01.r03.recovery\endcsname{54.0}
\expandafter\def\csname BAval@t01.r03.t5\endcsname{3.3}
\expandafter\def\csname BAval@t01.r04.sid\endcsname{64.5}
\expandafter\def\csname BAval@t01.r04.wrong\endcsname{12.2}
\expandafter\def\csname BAval@t01.r04.recovery\endcsname{64.0}
\expandafter\def\csname BAval@t01.r04.t5\endcsname{2.8}
\expandafter\def\csname BAval@t01.r05.sid\endcsname{65.8}
\expandafter\def\csname BAval@t01.r05.wrong\endcsname{11.8}
\expandafter\def\csname BAval@t01.r05.recovery\endcsname{65.0}
\expandafter\def\csname BAval@t01.r05.t5\endcsname{2.7}
\expandafter\def\csname BAval@t01.r06.sid\endcsname{68.7}
\expandafter\def\csname BAval@t01.r06.wrong\endcsname{10.1}
\expandafter\def\csname BAval@t01.r06.recovery\endcsname{70.0}
\expandafter\def\csname BAval@t01.r06.t5\endcsname{2.5}
\expandafter\def\csname BAval@t01.r07.sid\endcsname{70.3}
\expandafter\def\csname BAval@t01.r07.wrong\endcsname{8.8}
\expandafter\def\csname BAval@t01.r07.recovery\endcsname{72.0}
\expandafter\def\csname BAval@t01.r07.t5\endcsname{2.4}
\expandafter\def\csname BAval@t01.r08.sid\endcsname{82.3}
\expandafter\def\csname BAval@t01.r08.wrong\endcsname{4.4}
\expandafter\def\csname BAval@t01.r08.recovery\endcsname{86.2}
\expandafter\def\csname BAval@t01.r08.t5\endcsname{1.4}
\expandafter\def\csname BAval@t01.r09.sid\endcsname{87.9}
\expandafter\def\csname BAval@t01.r09.wrong\endcsname{1.6}
\expandafter\def\csname BAval@t01.r09.recovery\endcsname{92.0}
\expandafter\def\csname BAval@t01.r09.t5\endcsname{1.2}
\expandafter\def\csname BAval@t02.r01.short\endcsname{78.0}
\expandafter\def\csname BAval@t02.r01.similar\endcsname{67.0}
\expandafter\def\csname BAval@t02.r01.long\endcsname{53.0}
\expandafter\def\csname BAval@t02.r02.short\endcsname{79.0}
\expandafter\def\csname BAval@t02.r02.similar\endcsname{68.0}
\expandafter\def\csname BAval@t02.r02.long\endcsname{54.8}
\expandafter\def\csname BAval@t02.r03.short\endcsname{80.0}
\expandafter\def\csname BAval@t02.r03.similar\endcsname{72.0}
\expandafter\def\csname BAval@t02.r03.long\endcsname{57.6}
\expandafter\def\csname BAval@t02.r04.short\endcsname{82.0}
\expandafter\def\csname BAval@t02.r04.similar\endcsname{74.0}
\expandafter\def\csname BAval@t02.r04.long\endcsname{58.3}
\expandafter\def\csname BAval@t02.r05.short\endcsname{90.2}
\expandafter\def\csname BAval@t02.r05.similar\endcsname{85.4}
\expandafter\def\csname BAval@t02.r05.long\endcsname{73.9}
\expandafter\def\csname BAval@t02.r06.short\endcsname{94.0}
\expandafter\def\csname BAval@t02.r06.similar\endcsname{90.0}
\expandafter\def\csname BAval@t02.r06.long\endcsname{82.0}
\expandafter\def\csname BAval@t03.r01.sid\endcsname{65.9}
\expandafter\def\csname BAval@t03.r01.wrong\endcsname{11.9}
\expandafter\def\csname BAval@t03.r02.sid\endcsname{70.3}
\expandafter\def\csname BAval@t03.r02.wrong\endcsname{8.8}
\expandafter\def\csname BAval@t03.r03.sid\endcsname{77.6}
\expandafter\def\csname BAval@t03.r03.wrong\endcsname{6.3}
\expandafter\def\csname BAval@t03.r04.sid\endcsname{82.3}
\expandafter\def\csname BAval@t03.r04.wrong\endcsname{4.4}
\expandafter\def\csname BAval@t04.r01.sid\endcsname{82.3}
\expandafter\def\csname BAval@t04.r01.wrong\endcsname{4.4}
\expandafter\def\csname BAval@t04.r01.t5\endcsname{1.4}
\expandafter\def\csname BAval@t04.r02.sid\endcsname{77.9}
\expandafter\def\csname BAval@t04.r02.wrong\endcsname{7.1}
\expandafter\def\csname BAval@t04.r02.t5\endcsname{1.9}
\expandafter\def\csname BAval@t04.r03.sid\endcsname{76.0}
\expandafter\def\csname BAval@t04.r03.wrong\endcsname{9.0}
\expandafter\def\csname BAval@t04.r03.t5\endcsname{2.0}
\expandafter\def\csname BAval@t04.r04.sid\endcsname{78.0}
\expandafter\def\csname BAval@t04.r04.wrong\endcsname{7.7}
\expandafter\def\csname BAval@t04.r04.t5\endcsname{1.8}
\expandafter\def\csname BAval@t04.r05.sid\endcsname{79.3}
\expandafter\def\csname BAval@t04.r05.wrong\endcsname{6.8}
\expandafter\def\csname BAval@t04.r05.t5\endcsname{1.6}
\expandafter\def\csname BAval@t04.r06.sid\endcsname{73.7}
\expandafter\def\csname BAval@t04.r06.wrong\endcsname{8.8}
\expandafter\def\csname BAval@t04.r06.t5\endcsname{2.2}
\expandafter\def\csname BAval@t04.r07.sid\endcsname{77.6}
\expandafter\def\csname BAval@t04.r07.wrong\endcsname{6.3}
\expandafter\def\csname BAval@t04.r07.t5\endcsname{1.7}
\expandafter\def\csname BAval@t04.r08.sid\endcsname{80.5}
\expandafter\def\csname BAval@t04.r08.wrong\endcsname{5.8}
\expandafter\def\csname BAval@t04.r08.t5\endcsname{1.5}
\expandafter\def\csname BAval@t05.r01.separable\endcsname{78.0}
\expandafter\def\csname BAval@t05.r01.temporal.q\endcsname{80.1}
\expandafter\def\csname BAval@t05.r01.bindadapt\endcsname{86.1}
\expandafter\def\csname BAval@t05.r01.oracle\endcsname{91.7}
\expandafter\def\csname BAval@t05.r02.separable\endcsname{75.6}
\expandafter\def\csname BAval@t05.r02.temporal.q\endcsname{77.2}
\expandafter\def\csname BAval@t05.r02.bindadapt\endcsname{85.3}
\expandafter\def\csname BAval@t05.r02.oracle\endcsname{90.9}
\expandafter\def\csname BAval@t05.r03.separable\endcsname{71.1}
\expandafter\def\csname BAval@t05.r03.temporal.q\endcsname{73.2}
\expandafter\def\csname BAval@t05.r03.bindadapt\endcsname{83.8}
\expandafter\def\csname BAval@t05.r03.oracle\endcsname{90.1}
\expandafter\def\csname BAval@t05.r04.separable\endcsname{65.9}
\expandafter\def\csname BAval@t05.r04.temporal.q\endcsname{68.7}
\expandafter\def\csname BAval@t05.r04.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t05.r04.oracle\endcsname{87.9}
\expandafter\def\csname BAval@t05.r05.separable\endcsname{53.9}
\expandafter\def\csname BAval@t05.r05.temporal.q\endcsname{57.7}
\expandafter\def\csname BAval@t05.r05.bindadapt\endcsname{75.6}
\expandafter\def\csname BAval@t05.r05.oracle\endcsname{82.9}
\expandafter\def\csname BAval@t05.r06.separable\endcsname{37.9}
\expandafter\def\csname BAval@t05.r06.temporal.q\endcsname{42.1}
\expandafter\def\csname BAval@t05.r06.bindadapt\endcsname{64.0}
\expandafter\def\csname BAval@t05.r06.oracle\endcsname{72.9}
\expandafter\def\csname BAval@t06.r01.temporal.q\endcsname{54.1}
\expandafter\def\csname BAval@t06.r01.joint.belief\endcsname{56.1}
\expandafter\def\csname BAval@t06.r01.bindadapt\endcsname{70.2}
\expandafter\def\csname BAval@t06.r01.oracle\endcsname{77.0}
\expandafter\def\csname BAval@t06.r02.temporal.q\endcsname{62.0}
\expandafter\def\csname BAval@t06.r02.joint.belief\endcsname{64.0}
\expandafter\def\csname BAval@t06.r02.bindadapt\endcsname{77.1}
\expandafter\def\csname BAval@t06.r02.oracle\endcsname{84.0}
\expandafter\def\csname BAval@t06.r03.temporal.q\endcsname{68.7}
\expandafter\def\csname BAval@t06.r03.joint.belief\endcsname{70.3}
\expandafter\def\csname BAval@t06.r03.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t06.r03.oracle\endcsname{87.9}
\expandafter\def\csname BAval@t06.r04.temporal.q\endcsname{72.3}
\expandafter\def\csname BAval@t06.r04.joint.belief\endcsname{74.3}
\expandafter\def\csname BAval@t06.r04.bindadapt\endcsname{84.5}
\expandafter\def\csname BAval@t06.r04.oracle\endcsname{90.2}
\expandafter\def\csname BAval@t06.r05.temporal.q\endcsname{74.7}
\expandafter\def\csname BAval@t06.r05.joint.belief\endcsname{76.1}
\expandafter\def\csname BAval@t06.r05.bindadapt\endcsname{85.6}
\expandafter\def\csname BAval@t06.r05.oracle\endcsname{91.0}
\expandafter\def\csname BAval@t06.r06.temporal.q\endcsname{75.9}
\expandafter\def\csname BAval@t06.r06.joint.belief\endcsname{77.6}
\expandafter\def\csname BAval@t06.r06.bindadapt\endcsname{86.2}
\expandafter\def\csname BAval@t06.r06.oracle\endcsname{91.4}
\expandafter\def\csname BAval@t07.r01.pair.rank.pct\endcsname{67.0}
\expandafter\def\csname BAval@t07.r01.risk.mae\endcsname{0.140}
\expandafter\def\csname BAval@t07.r01.calibration.error\endcsname{0.098}
\expandafter\def\csname BAval@t07.r01.action.regret\endcsname{0.125}
\expandafter\def\csname BAval@t07.r02.pair.rank.pct\endcsname{72.5}
\expandafter\def\csname BAval@t07.r02.risk.mae\endcsname{0.118}
\expandafter\def\csname BAval@t07.r02.calibration.error\endcsname{0.073}
\expandafter\def\csname BAval@t07.r02.action.regret\endcsname{0.091}
\expandafter\def\csname BAval@t07.r03.pair.rank.pct\endcsname{78.0}
\expandafter\def\csname BAval@t07.r03.risk.mae\endcsname{0.096}
\expandafter\def\csname BAval@t07.r03.calibration.error\endcsname{0.056}
\expandafter\def\csname BAval@t07.r03.action.regret\endcsname{0.068}
\expandafter\def\csname BAval@t07.r04.pair.rank.pct\endcsname{88.7}
\expandafter\def\csname BAval@t07.r04.risk.mae\endcsname{0.053}
\expandafter\def\csname BAval@t07.r04.calibration.error\endcsname{0.026}
\expandafter\def\csname BAval@t07.r04.action.regret\endcsname{0.032}
\expandafter\def\csname BAval@t08.r01.sid\endcsname{82.3}
\expandafter\def\csname BAval@t08.r02.sid\endcsname{82.8}
\expandafter\def\csname BAval@t08.r03.sid\endcsname{86.1}
\expandafter\def\csname BAval@t08.r04.sid\endcsname{87.9}
\expandafter\def\csname BAval@t08.r05.sid\endcsname{94.1}
\expandafter\def\csname BAval@t08.r06.sid\endcsname{98.0}
\expandafter\def\csname BAval@t09.r01.groups\endcsname{60}
\expandafter\def\csname BAval@t09.r01.episodes\endcsname{1200}
\expandafter\def\csname BAval@t09.r02.groups\endcsname{20}
\expandafter\def\csname BAval@t09.r02.episodes\endcsname{200}
\expandafter\def\csname BAval@t09.r03.groups\endcsname{40}
\expandafter\def\csname BAval@t09.r03.episodes\endcsname{480}
\expandafter\def\csname BAval@t10.r01.separable\endcsname{68.6}
\expandafter\def\csname BAval@t10.r01.temporal.q\endcsname{70.1}
\expandafter\def\csname BAval@t10.r01.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t10.r02.separable\endcsname{65.3}
\expandafter\def\csname BAval@t10.r02.temporal.q\endcsname{67.0}
\expandafter\def\csname BAval@t10.r02.bindadapt\endcsname{80.1}
\expandafter\def\csname BAval@t10.r03.separable\endcsname{61.8}
\expandafter\def\csname BAval@t10.r03.temporal.q\endcsname{65.2}
\expandafter\def\csname BAval@t10.r03.bindadapt\endcsname{78.1}
\expandafter\def\csname BAval@t10.r04.separable\endcsname{58.9}
\expandafter\def\csname BAval@t10.r04.temporal.q\endcsname{62.9}
\expandafter\def\csname BAval@t10.r04.bindadapt\endcsname{76.1}
\expandafter\def\csname BAval@t10.r05.separable\endcsname{62.4}
\expandafter\def\csname BAval@t10.r05.temporal.q\endcsname{64.9}
\expandafter\def\csname BAval@t10.r05.bindadapt\endcsname{77.1}
\expandafter\def\csname BAval@t11.r01.reference\endcsname{91.2}
\expandafter\def\csname BAval@t11.r01.bindadapt\endcsname{92.0}
\expandafter\def\csname BAval@t11.r01.gain.pp\endcsname{0.8}
\expandafter\def\csname BAval@t11.r02.reference\endcsname{93.9}
\expandafter\def\csname BAval@t11.r02.bindadapt\endcsname{94.1}
\expandafter\def\csname BAval@t11.r02.gain.pp\endcsname{0.2}
\expandafter\def\csname BAval@t11.r03.reference\endcsname{65.9}
\expandafter\def\csname BAval@t11.r03.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t11.r03.gain.pp\endcsname{16.4}
\expandafter\def\csname BAval@t11.r04.reference\endcsname{40.9}
\expandafter\def\csname BAval@t11.r04.bindadapt\endcsname{41.3}
\expandafter\def\csname BAval@t11.r04.gain.pp\endcsname{0.4}
\expandafter\def\csname BAval@t11.r05.reference\endcsname{20.5}
\expandafter\def\csname BAval@t11.r05.bindadapt\endcsname{20.7}
\expandafter\def\csname BAval@t11.r05.gain.pp\endcsname{0.2}
\expandafter\def\csname BAval@t12.r01.sid\endcsname{60.9}
\expandafter\def\csname BAval@t12.r01.wrong\endcsname{14.6}
\expandafter\def\csname BAval@t12.r01.recovery\endcsname{59.0}
\expandafter\def\csname BAval@t12.r01.t5\endcsname{3.0}
\expandafter\def\csname BAval@t12.r02.sid\endcsname{62.5}
\expandafter\def\csname BAval@t12.r02.wrong\endcsname{13.8}
\expandafter\def\csname BAval@t12.r02.recovery\endcsname{61.1}
\expandafter\def\csname BAval@t12.r02.t5\endcsname{2.9}
\expandafter\def\csname BAval@t12.r03.sid\endcsname{65.3}
\expandafter\def\csname BAval@t12.r03.wrong\endcsname{12.2}
\expandafter\def\csname BAval@t12.r03.recovery\endcsname{64.9}
\expandafter\def\csname BAval@t12.r03.t5\endcsname{2.7}
\expandafter\def\csname BAval@t12.r04.sid\endcsname{66.4}
\expandafter\def\csname BAval@t12.r04.wrong\endcsname{11.8}
\expandafter\def\csname BAval@t12.r04.recovery\endcsname{67.1}
\expandafter\def\csname BAval@t12.r04.t5\endcsname{2.6}
\expandafter\def\csname BAval@t12.r05.sid\endcsname{71.0}
\expandafter\def\csname BAval@t12.r05.wrong\endcsname{8.8}
\expandafter\def\csname BAval@t12.r05.recovery\endcsname{73.0}
\expandafter\def\csname BAval@t12.r05.t5\endcsname{2.3}
\expandafter\def\csname BAval@t12.r06.sid\endcsname{62.0}
\expandafter\def\csname BAval@t12.r06.wrong\endcsname{14.3}
\expandafter\def\csname BAval@t12.r06.recovery\endcsname{64.0}
\expandafter\def\csname BAval@t12.r06.t5\endcsname{2.8}
\expandafter\def\csname BAval@t12.r07.sid\endcsname{65.6}
\expandafter\def\csname BAval@t12.r07.wrong\endcsname{10.4}
\expandafter\def\csname BAval@t12.r07.recovery\endcsname{68.0}
\expandafter\def\csname BAval@t12.r07.t5\endcsname{2.5}
\expandafter\def\csname BAval@t12.r08.sid\endcsname{70.3}
\expandafter\def\csname BAval@t12.r08.wrong\endcsname{8.1}
\expandafter\def\csname BAval@t12.r08.recovery\endcsname{74.0}
\expandafter\def\csname BAval@t12.r08.t5\endcsname{2.2}
\expandafter\def\csname BAval@t12.r09.sid\endcsname{66.5}
\expandafter\def\csname BAval@t12.r09.wrong\endcsname{10.9}
\expandafter\def\csname BAval@t12.r09.recovery\endcsname{68.0}
\expandafter\def\csname BAval@t12.r09.t5\endcsname{2.6}
\expandafter\def\csname BAval@t12.r10.sid\endcsname{72.8}
\expandafter\def\csname BAval@t12.r10.wrong\endcsname{7.8}
\expandafter\def\csname BAval@t12.r10.recovery\endcsname{76.1}
\expandafter\def\csname BAval@t12.r10.t5\endcsname{2.1}
\expandafter\def\csname BAval@t12.r11.sid\endcsname{68.0}
\expandafter\def\csname BAval@t12.r11.wrong\endcsname{10.1}
\expandafter\def\csname BAval@t12.r11.recovery\endcsname{69.0}
\expandafter\def\csname BAval@t12.r11.t5\endcsname{2.5}
\expandafter\def\csname BAval@t12.r12.sid\endcsname{71.6}
\expandafter\def\csname BAval@t12.r12.wrong\endcsname{8.6}
\expandafter\def\csname BAval@t12.r12.recovery\endcsname{73.9}
\expandafter\def\csname BAval@t12.r12.t5\endcsname{2.2}
\expandafter\def\csname BAval@t12.r13.sid\endcsname{74.1}
\expandafter\def\csname BAval@t12.r13.wrong\endcsname{7.4}
\expandafter\def\csname BAval@t12.r13.recovery\endcsname{77.1}
\expandafter\def\csname BAval@t12.r13.t5\endcsname{2.1}
\expandafter\def\csname BAval@t12.r14.sid\endcsname{74.6}
\expandafter\def\csname BAval@t12.r14.wrong\endcsname{6.9}
\expandafter\def\csname BAval@t12.r14.recovery\endcsname{77.9}
\expandafter\def\csname BAval@t12.r14.t5\endcsname{2.0}
\expandafter\def\csname BAval@t12.r15.sid\endcsname{75.2}
\expandafter\def\csname BAval@t12.r15.wrong\endcsname{7.3}
\expandafter\def\csname BAval@t12.r15.recovery\endcsname{79.0}
\expandafter\def\csname BAval@t12.r15.t5\endcsname{2.0}
\expandafter\def\csname BAval@t12.r16.sid\endcsname{82.3}
\expandafter\def\csname BAval@t12.r16.wrong\endcsname{4.4}
\expandafter\def\csname BAval@t12.r16.recovery\endcsname{86.2}
\expandafter\def\csname BAval@t12.r16.t5\endcsname{1.4}
\expandafter\def\csname BAval@t13.r01.ao\endcsname{63.9}
\expandafter\def\csname BAval@t13.r01.p20.pct\endcsname{76.6}
\expandafter\def\csname BAval@t13.r01.pn20\endcsname{78.1}
\expandafter\def\csname BAval@t13.r01.sr50.pct\endcsname{74.2}
\expandafter\def\csname BAval@t13.r01.sr75.pct\endcsname{49.6}
\expandafter\def\csname BAval@t13.r01.sao.pct\endcsname{58.3}
\expandafter\def\csname BAval@t13.r01.ssr50.pct\endcsname{66.7}
\expandafter\def\csname BAval@t13.r01.ssr75.pct\endcsname{41.0}
\expandafter\def\csname BAval@t13.r02.ao\endcsname{65.0}
\expandafter\def\csname BAval@t13.r02.p20.pct\endcsname{77.9}
\expandafter\def\csname BAval@t13.r02.pn20\endcsname{79.2}
\expandafter\def\csname BAval@t13.r02.sr50.pct\endcsname{75.5}
\expandafter\def\csname BAval@t13.r02.sr75.pct\endcsname{51.4}
\expandafter\def\csname BAval@t13.r02.sao.pct\endcsname{59.2}
\expandafter\def\csname BAval@t13.r02.ssr50.pct\endcsname{67.9}
\expandafter\def\csname BAval@t13.r02.ssr75.pct\endcsname{42.4}
\expandafter\def\csname BAval@t13.r03.ao\endcsname{67.7}
\expandafter\def\csname BAval@t13.r03.p20.pct\endcsname{79.7}
\expandafter\def\csname BAval@t13.r03.pn20\endcsname{81.5}
\expandafter\def\csname BAval@t13.r03.sr50.pct\endcsname{78.5}
\expandafter\def\csname BAval@t13.r03.sr75.pct\endcsname{55.8}
\expandafter\def\csname BAval@t13.r03.sao.pct\endcsname{61.9}
\expandafter\def\csname BAval@t13.r03.ssr50.pct\endcsname{70.6}
\expandafter\def\csname BAval@t13.r03.ssr75.pct\endcsname{45.7}
\expandafter\def\csname BAval@t13.r04.ao\endcsname{68.6}
\expandafter\def\csname BAval@t13.r04.p20.pct\endcsname{80.2}
\expandafter\def\csname BAval@t13.r04.pn20\endcsname{82.0}
\expandafter\def\csname BAval@t13.r04.sr50.pct\endcsname{79.5}
\expandafter\def\csname BAval@t13.r04.sr75.pct\endcsname{57.1}
\expandafter\def\csname BAval@t13.r04.sao.pct\endcsname{62.5}
\expandafter\def\csname BAval@t13.r04.ssr50.pct\endcsname{71.4}
\expandafter\def\csname BAval@t13.r04.ssr75.pct\endcsname{47.2}
\expandafter\def\csname BAval@t13.r05.ao\endcsname{72.7}
\expandafter\def\csname BAval@t13.r05.p20.pct\endcsname{84.9}
\expandafter\def\csname BAval@t13.r05.pn20\endcsname{86.0}
\expandafter\def\csname BAval@t13.r05.sr50.pct\endcsname{83.6}
\expandafter\def\csname BAval@t13.r05.sr75.pct\endcsname{63.2}
\expandafter\def\csname BAval@t13.r05.sao.pct\endcsname{67.0}
\expandafter\def\csname BAval@t13.r05.ssr50.pct\endcsname{76.1}
\expandafter\def\csname BAval@t13.r05.ssr75.pct\endcsname{53.6}
\expandafter\def\csname BAval@t13.r06.ao\endcsname{63.7}
\expandafter\def\csname BAval@t13.r06.p20.pct\endcsname{75.3}
\expandafter\def\csname BAval@t13.r06.pn20\endcsname{77.1}
\expandafter\def\csname BAval@t13.r06.sr50.pct\endcsname{74.1}
\expandafter\def\csname BAval@t13.r06.sr75.pct\endcsname{48.3}
\expandafter\def\csname BAval@t13.r06.sao.pct\endcsname{57.8}
\expandafter\def\csname BAval@t13.r06.ssr50.pct\endcsname{66.1}
\expandafter\def\csname BAval@t13.r06.ssr75.pct\endcsname{40.6}
\expandafter\def\csname BAval@t13.r07.ao\endcsname{67.0}
\expandafter\def\csname BAval@t13.r07.p20.pct\endcsname{78.9}
\expandafter\def\csname BAval@t13.r07.pn20\endcsname{80.5}
\expandafter\def\csname BAval@t13.r07.sr50.pct\endcsname{77.9}
\expandafter\def\csname BAval@t13.r07.sr75.pct\endcsname{54.1}
\expandafter\def\csname BAval@t13.r07.sao.pct\endcsname{61.9}
\expandafter\def\csname BAval@t13.r07.ssr50.pct\endcsname{69.9}
\expandafter\def\csname BAval@t13.r07.ssr75.pct\endcsname{46.3}
\expandafter\def\csname BAval@t13.r08.ao\endcsname{73.3}
\expandafter\def\csname BAval@t13.r08.p20.pct\endcsname{84.5}
\expandafter\def\csname BAval@t13.r08.pn20\endcsname{85.9}
\expandafter\def\csname BAval@t13.r08.sr50.pct\endcsname{84.3}
\expandafter\def\csname BAval@t13.r08.sr75.pct\endcsname{63.6}
\expandafter\def\csname BAval@t13.r08.sao.pct\endcsname{66.7}
\expandafter\def\csname BAval@t13.r08.ssr50.pct\endcsname{75.8}
\expandafter\def\csname BAval@t13.r08.ssr75.pct\endcsname{53.0}
\expandafter\def\csname BAval@t13.r09.ao\endcsname{67.3}
\expandafter\def\csname BAval@t13.r09.p20.pct\endcsname{79.2}
\expandafter\def\csname BAval@t13.r09.pn20\endcsname{80.6}
\expandafter\def\csname BAval@t13.r09.sr50.pct\endcsname{78.4}
\expandafter\def\csname BAval@t13.r09.sr75.pct\endcsname{54.7}
\expandafter\def\csname BAval@t13.r09.sao.pct\endcsname{64.6}
\expandafter\def\csname BAval@t13.r09.ssr50.pct\endcsname{73.6}
\expandafter\def\csname BAval@t13.r09.ssr75.pct\endcsname{49.9}
\expandafter\def\csname BAval@t13.r10.ao\endcsname{72.0}
\expandafter\def\csname BAval@t13.r10.p20.pct\endcsname{83.2}
\expandafter\def\csname BAval@t13.r10.pn20\endcsname{84.7}
\expandafter\def\csname BAval@t13.r10.sr50.pct\endcsname{82.7}
\expandafter\def\csname BAval@t13.r10.sr75.pct\endcsname{61.8}
\expandafter\def\csname BAval@t13.r10.sao.pct\endcsname{68.3}
\expandafter\def\csname BAval@t13.r10.ssr50.pct\endcsname{77.0}
\expandafter\def\csname BAval@t13.r10.ssr75.pct\endcsname{55.4}
\expandafter\def\csname BAval@t13.r11.ao\endcsname{79.1}
\expandafter\def\csname BAval@t13.r11.p20.pct\endcsname{88.0}
\expandafter\def\csname BAval@t13.r11.pn20\endcsname{89.3}
\expandafter\def\csname BAval@t13.r11.sr50.pct\endcsname{88.0}
\expandafter\def\csname BAval@t13.r11.sr75.pct\endcsname{71.5}
\expandafter\def\csname BAval@t13.r11.sao.pct\endcsname{76.9}
\expandafter\def\csname BAval@t13.r11.ssr50.pct\endcsname{83.9}
\expandafter\def\csname BAval@t13.r11.ssr75.pct\endcsname{67.2}
\expandafter\def\csname BAval@t14.r01.short\endcsname{84.0}
\expandafter\def\csname BAval@t14.r01.similar\endcsname{75.9}
\expandafter\def\csname BAval@t14.r01.long\endcsname{55.5}
\expandafter\def\csname BAval@t14.r01.weighted\endcsname{70.3}
\expandafter\def\csname BAval@t14.r02.short\endcsname{85.5}
\expandafter\def\csname BAval@t14.r02.similar\endcsname{77.2}
\expandafter\def\csname BAval@t14.r02.long\endcsname{59.9}
\expandafter\def\csname BAval@t14.r02.weighted\endcsname{72.8}
\expandafter\def\csname BAval@t14.r03.short\endcsname{84.8}
\expandafter\def\csname BAval@t14.r03.similar\endcsname{76.5}
\expandafter\def\csname BAval@t14.r03.long\endcsname{58.0}
\expandafter\def\csname BAval@t14.r03.weighted\endcsname{71.6}
\expandafter\def\csname BAval@t14.r04.short\endcsname{85.4}
\expandafter\def\csname BAval@t14.r04.similar\endcsname{78.8}
\expandafter\def\csname BAval@t14.r04.long\endcsname{61.9}
\expandafter\def\csname BAval@t14.r04.weighted\endcsname{74.1}
\expandafter\def\csname BAval@t14.r05.short\endcsname{86.2}
\expandafter\def\csname BAval@t14.r05.similar\endcsname{79.2}
\expandafter\def\csname BAval@t14.r05.long\endcsname{63.9}
\expandafter\def\csname BAval@t14.r05.weighted\endcsname{75.2}
\expandafter\def\csname BAval@t14.r06.short\endcsname{90.2}
\expandafter\def\csname BAval@t14.r06.similar\endcsname{85.4}
\expandafter\def\csname BAval@t14.r06.long\endcsname{73.9}
\expandafter\def\csname BAval@t14.r06.weighted\endcsname{82.3}
\expandafter\def\csname BAval@t14.r07.short\endcsname{74.9}
\expandafter\def\csname BAval@t14.r07.similar\endcsname{65.7}
\expandafter\def\csname BAval@t14.r07.long\endcsname{46.8}
\expandafter\def\csname BAval@t14.r07.weighted\endcsname{60.9}
\expandafter\def\csname BAval@t14.r08.short\endcsname{76.5}
\expandafter\def\csname BAval@t14.r08.similar\endcsname{67.3}
\expandafter\def\csname BAval@t14.r08.long\endcsname{48.3}
\expandafter\def\csname BAval@t14.r08.weighted\endcsname{62.5}
\expandafter\def\csname BAval@t14.r09.short\endcsname{79.1}
\expandafter\def\csname BAval@t14.r09.similar\endcsname{70.2}
\expandafter\def\csname BAval@t14.r09.long\endcsname{51.1}
\expandafter\def\csname BAval@t14.r09.weighted\endcsname{65.3}
\expandafter\def\csname BAval@t14.r10.short\endcsname{80.6}
\expandafter\def\csname BAval@t14.r10.similar\endcsname{71.3}
\expandafter\def\csname BAval@t14.r10.long\endcsname{52.1}
\expandafter\def\csname BAval@t14.r10.weighted\endcsname{66.4}
\expandafter\def\csname BAval@t14.r11.short\endcsname{84.9}
\expandafter\def\csname BAval@t14.r11.similar\endcsname{75.8}
\expandafter\def\csname BAval@t14.r11.long\endcsname{57.1}
\expandafter\def\csname BAval@t14.r11.weighted\endcsname{71.0}
\expandafter\def\csname BAval@t14.r12.short\endcsname{76.1}
\expandafter\def\csname BAval@t14.r12.similar\endcsname{66.9}
\expandafter\def\csname BAval@t14.r12.long\endcsname{47.7}
\expandafter\def\csname BAval@t14.r12.weighted\endcsname{62.0}
\expandafter\def\csname BAval@t14.r13.short\endcsname{79.7}
\expandafter\def\csname BAval@t14.r13.similar\endcsname{70.8}
\expandafter\def\csname BAval@t14.r13.long\endcsname{50.9}
\expandafter\def\csname BAval@t14.r13.weighted\endcsname{65.6}
\expandafter\def\csname BAval@t14.r14.short\endcsname{80.6}
\expandafter\def\csname BAval@t14.r14.similar\endcsname{71.7}
\expandafter\def\csname BAval@t14.r14.long\endcsname{52.0}
\expandafter\def\csname BAval@t14.r14.weighted\endcsname{66.5}
\expandafter\def\csname BAval@t14.r15.short\endcsname{82.0}
\expandafter\def\csname BAval@t14.r15.similar\endcsname{73.1}
\expandafter\def\csname BAval@t14.r15.long\endcsname{53.6}
\expandafter\def\csname BAval@t14.r15.weighted\endcsname{68.0}
\expandafter\def\csname BAval@t14.r16.short\endcsname{88.6}
\expandafter\def\csname BAval@t14.r16.similar\endcsname{79.7}
\expandafter\def\csname BAval@t14.r16.long\endcsname{60.3}
\expandafter\def\csname BAval@t14.r16.weighted\endcsname{74.6}
\expandafter\def\csname BAval@t15.r01.common.controller\endcsname{60.9}
\expandafter\def\csname BAval@t15.r01.oa.vat.ptz\endcsname{66.8}
\expandafter\def\csname BAval@t15.r01.chanakya.j\endcsname{68.9}
\expandafter\def\csname BAval@t15.r01.bindadapt\endcsname{77.1}
\expandafter\def\csname BAval@t15.r02.common.controller\endcsname{71.0}
\expandafter\def\csname BAval@t15.r02.oa.vat.ptz\endcsname{73.2}
\expandafter\def\csname BAval@t15.r02.chanakya.j\endcsname{73.8}
\expandafter\def\csname BAval@t15.r02.bindadapt\endcsname{81.5}
\expandafter\def\csname BAval@t15.r03.common.controller\endcsname{70.3}
\expandafter\def\csname BAval@t15.r03.oa.vat.ptz\endcsname{74.3}
\expandafter\def\csname BAval@t15.r03.chanakya.j\endcsname{75.2}
\expandafter\def\csname BAval@t15.r03.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t16.r01.tracking.precision.pct\endcsname{72.9}
\expandafter\def\csname BAval@t16.r01.tracking.recall.pct\endcsname{65.3}
\expandafter\def\csname BAval@t16.r01.fmax.pct\endcsname{68.9}
\expandafter\def\csname BAval@t16.r01.operating.precision.pct\endcsname{72.1}
\expandafter\def\csname BAval@t16.r01.operating.recall.pct\endcsname{63.0}
\expandafter\def\csname BAval@t16.r01.f.operating.pct\endcsname{67.2}
\expandafter\def\csname BAval@t16.r02.tracking.precision.pct\endcsname{75.9}
\expandafter\def\csname BAval@t16.r02.tracking.recall.pct\endcsname{68.2}
\expandafter\def\csname BAval@t16.r02.fmax.pct\endcsname{71.9}
\expandafter\def\csname BAval@t16.r02.operating.precision.pct\endcsname{74.9}
\expandafter\def\csname BAval@t16.r02.operating.recall.pct\endcsname{66.2}
\expandafter\def\csname BAval@t16.r02.f.operating.pct\endcsname{70.2}
\expandafter\def\csname BAval@t16.r03.tracking.precision.pct\endcsname{79.0}
\expandafter\def\csname BAval@t16.r03.tracking.recall.pct\endcsname{73.5}
\expandafter\def\csname BAval@t16.r03.fmax.pct\endcsname{76.1}
\expandafter\def\csname BAval@t16.r03.operating.precision.pct\endcsname{77.9}
\expandafter\def\csname BAval@t16.r03.operating.recall.pct\endcsname{71.4}
\expandafter\def\csname BAval@t16.r03.f.operating.pct\endcsname{74.5}
\expandafter\def\csname BAval@t16.r04.tracking.precision.pct\endcsname{80.0}
\expandafter\def\csname BAval@t16.r04.tracking.recall.pct\endcsname{74.3}
\expandafter\def\csname BAval@t16.r04.fmax.pct\endcsname{77.0}
\expandafter\def\csname BAval@t16.r04.operating.precision.pct\endcsname{79.1}
\expandafter\def\csname BAval@t16.r04.operating.recall.pct\endcsname{72.5}
\expandafter\def\csname BAval@t16.r04.f.operating.pct\endcsname{75.6}
\expandafter\def\csname BAval@t16.r05.tracking.precision.pct\endcsname{80.9}
\expandafter\def\csname BAval@t16.r05.tracking.recall.pct\endcsname{75.0}
\expandafter\def\csname BAval@t16.r05.fmax.pct\endcsname{77.9}
\expandafter\def\csname BAval@t16.r05.operating.precision.pct\endcsname{80.1}
\expandafter\def\csname BAval@t16.r05.operating.recall.pct\endcsname{72.8}
\expandafter\def\csname BAval@t16.r05.f.operating.pct\endcsname{76.3}
\expandafter\def\csname BAval@t16.r06.tracking.precision.pct\endcsname{82.0}
\expandafter\def\csname BAval@t16.r06.tracking.recall.pct\endcsname{76.1}
\expandafter\def\csname BAval@t16.r06.fmax.pct\endcsname{78.9}
\expandafter\def\csname BAval@t16.r06.operating.precision.pct\endcsname{81.1}
\expandafter\def\csname BAval@t16.r06.operating.recall.pct\endcsname{74.1}
\expandafter\def\csname BAval@t16.r06.f.operating.pct\endcsname{77.4}
\expandafter\def\csname BAval@t16.r07.tracking.precision.pct\endcsname{87.4}
\expandafter\def\csname BAval@t16.r07.tracking.recall.pct\endcsname{82.8}
\expandafter\def\csname BAval@t16.r07.fmax.pct\endcsname{85.0}
\expandafter\def\csname BAval@t16.r07.operating.precision.pct\endcsname{86.5}
\expandafter\def\csname BAval@t16.r07.operating.recall.pct\endcsname{81.2}
\expandafter\def\csname BAval@t16.r07.f.operating.pct\endcsname{83.8}
\expandafter\def\csname BAval@t17.r01.dam4sam\endcsname{79.4}
\expandafter\def\csname BAval@t17.r01.oa.vat.ptz\endcsname{81.2}
\expandafter\def\csname BAval@t17.r01.artrack.ac\endcsname{80.1}
\expandafter\def\csname BAval@t17.r01.chanakya.j\endcsname{81.3}
\expandafter\def\csname BAval@t17.r01.dam4sam.chanakya.j\endcsname{82.0}
\expandafter\def\csname BAval@t17.r01.bindadapt\endcsname{86.1}
\expandafter\def\csname BAval@t17.r02.dam4sam\endcsname{78.0}
\expandafter\def\csname BAval@t17.r02.oa.vat.ptz\endcsname{79.8}
\expandafter\def\csname BAval@t17.r02.artrack.ac\endcsname{78.9}
\expandafter\def\csname BAval@t17.r02.chanakya.j\endcsname{80.1}
\expandafter\def\csname BAval@t17.r02.dam4sam.chanakya.j\endcsname{81.1}
\expandafter\def\csname BAval@t17.r02.bindadapt\endcsname{85.3}
\expandafter\def\csname BAval@t17.r03.dam4sam\endcsname{74.5}
\expandafter\def\csname BAval@t17.r03.oa.vat.ptz\endcsname{76.8}
\expandafter\def\csname BAval@t17.r03.artrack.ac\endcsname{75.9}
\expandafter\def\csname BAval@t17.r03.chanakya.j\endcsname{77.8}
\expandafter\def\csname BAval@t17.r03.dam4sam.chanakya.j\endcsname{78.7}
\expandafter\def\csname BAval@t17.r03.bindadapt\endcsname{83.8}
\expandafter\def\csname BAval@t17.r04.dam4sam\endcsname{70.3}
\expandafter\def\csname BAval@t17.r04.oa.vat.ptz\endcsname{72.8}
\expandafter\def\csname BAval@t17.r04.artrack.ac\endcsname{71.6}
\expandafter\def\csname BAval@t17.r04.chanakya.j\endcsname{74.1}
\expandafter\def\csname BAval@t17.r04.dam4sam.chanakya.j\endcsname{75.2}
\expandafter\def\csname BAval@t17.r04.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t17.r05.dam4sam\endcsname{58.6}
\expandafter\def\csname BAval@t17.r05.oa.vat.ptz\endcsname{62.0}
\expandafter\def\csname BAval@t17.r05.artrack.ac\endcsname{61.8}
\expandafter\def\csname BAval@t17.r05.chanakya.j\endcsname{65.7}
\expandafter\def\csname BAval@t17.r05.dam4sam.chanakya.j\endcsname{66.9}
\expandafter\def\csname BAval@t17.r05.bindadapt\endcsname{75.6}
\expandafter\def\csname BAval@t17.r06.dam4sam\endcsname{40.1}
\expandafter\def\csname BAval@t17.r06.oa.vat.ptz\endcsname{45.4}
\expandafter\def\csname BAval@t17.r06.artrack.ac\endcsname{44.9}
\expandafter\def\csname BAval@t17.r06.chanakya.j\endcsname{50.0}
\expandafter\def\csname BAval@t17.r06.dam4sam.chanakya.j\endcsname{51.9}
\expandafter\def\csname BAval@t17.r06.bindadapt\endcsname{64.0}
\expandafter\def\csname BAval@t17.r07.dam4sam\endcsname{52.8}
\expandafter\def\csname BAval@t17.r07.oa.vat.ptz\endcsname{56.9}
\expandafter\def\csname BAval@t17.r07.artrack.ac\endcsname{59.1}
\expandafter\def\csname BAval@t17.r07.chanakya.j\endcsname{60.5}
\expandafter\def\csname BAval@t17.r07.dam4sam.chanakya.j\endcsname{61.5}
\expandafter\def\csname BAval@t17.r07.bindadapt\endcsname{70.2}
\expandafter\def\csname BAval@t17.r08.dam4sam\endcsname{62.8}
\expandafter\def\csname BAval@t17.r08.oa.vat.ptz\endcsname{65.7}
\expandafter\def\csname BAval@t17.r08.artrack.ac\endcsname{66.5}
\expandafter\def\csname BAval@t17.r08.chanakya.j\endcsname{68.2}
\expandafter\def\csname BAval@t17.r08.dam4sam.chanakya.j\endcsname{69.5}
\expandafter\def\csname BAval@t17.r08.bindadapt\endcsname{77.1}
\expandafter\def\csname BAval@t17.r09.dam4sam\endcsname{70.3}
\expandafter\def\csname BAval@t17.r09.oa.vat.ptz\endcsname{72.8}
\expandafter\def\csname BAval@t17.r09.artrack.ac\endcsname{71.6}
\expandafter\def\csname BAval@t17.r09.chanakya.j\endcsname{74.1}
\expandafter\def\csname BAval@t17.r09.dam4sam.chanakya.j\endcsname{75.2}
\expandafter\def\csname BAval@t17.r09.bindadapt\endcsname{82.3}
\expandafter\def\csname BAval@t17.r10.dam4sam\endcsname{73.4}
\expandafter\def\csname BAval@t17.r10.oa.vat.ptz\endcsname{76.0}
\expandafter\def\csname BAval@t17.r10.artrack.ac\endcsname{75.2}
\expandafter\def\csname BAval@t17.r10.chanakya.j\endcsname{77.3}
\expandafter\def\csname BAval@t17.r10.dam4sam.chanakya.j\endcsname{78.7}
\expandafter\def\csname BAval@t17.r10.bindadapt\endcsname{84.5}
\expandafter\def\csname BAval@t17.r11.dam4sam\endcsname{75.5}
\expandafter\def\csname BAval@t17.r11.oa.vat.ptz\endcsname{77.3}
\expandafter\def\csname BAval@t17.r11.artrack.ac\endcsname{76.7}
\expandafter\def\csname BAval@t17.r11.chanakya.j\endcsname{78.6}
\expandafter\def\csname BAval@t17.r11.dam4sam.chanakya.j\endcsname{79.5}
\expandafter\def\csname BAval@t17.r11.bindadapt\endcsname{85.6}
\expandafter\def\csname BAval@t17.r12.dam4sam\endcsname{76.8}
\expandafter\def\csname BAval@t17.r12.oa.vat.ptz\endcsname{78.5}
\expandafter\def\csname BAval@t17.r12.artrack.ac\endcsname{78.0}
\expandafter\def\csname BAval@t17.r12.chanakya.j\endcsname{79.7}
\expandafter\def\csname BAval@t17.r12.dam4sam.chanakya.j\endcsname{80.8}
\expandafter\def\csname BAval@t17.r12.bindadapt\endcsname{86.2}
\expandafter\def\csname BAval@t18.r01.mean.inference.ms\endcsname{16.0}
\expandafter\def\csname BAval@t18.r01.p95.inference.ms\endcsname{21.9}
\expandafter\def\csname BAval@t18.r01.fps\endcsname{62.5}
\expandafter\def\csname BAval@t18.r01.decision.overhead.ms\endcsname{0.5}
\expandafter\def\csname BAval@t18.r02.mean.inference.ms\endcsname{23.1}
\expandafter\def\csname BAval@t18.r02.p95.inference.ms\endcsname{31.2}
\expandafter\def\csname BAval@t18.r02.fps\endcsname{43.4}
\expandafter\def\csname BAval@t18.r02.decision.overhead.ms\endcsname{0.5}
\expandafter\def\csname BAval@t18.r03.mean.inference.ms\endcsname{36.2}
\expandafter\def\csname BAval@t18.r03.p95.inference.ms\endcsname{48.8}
\expandafter\def\csname BAval@t18.r03.fps\endcsname{27.6}
\expandafter\def\csname BAval@t18.r03.decision.overhead.ms\endcsname{0.5}
\expandafter\def\csname BAval@t18.r04.mean.inference.ms\endcsname{19.5}
\expandafter\def\csname BAval@t18.r04.p95.inference.ms\endcsname{28.1}
\expandafter\def\csname BAval@t18.r04.fps\endcsname{51.4}
\expandafter\def\csname BAval@t18.r04.decision.overhead.ms\endcsname{1.5}
\expandafter\def\csname BAval@t18.r05.mean.inference.ms\endcsname{17.1}
\expandafter\def\csname BAval@t18.r05.p95.inference.ms\endcsname{24.8}
\expandafter\def\csname BAval@t18.r05.fps\endcsname{58.6}
\expandafter\def\csname BAval@t18.r05.decision.overhead.ms\endcsname{1.2}
\expandafter\def\csname BAval@t18.r06.mean.inference.ms\endcsname{26.1}
\expandafter\def\csname BAval@t18.r06.p95.inference.ms\endcsname{39.3}
\expandafter\def\csname BAval@t18.r06.fps\endcsname{38.3}
\expandafter\def\csname BAval@t18.r06.decision.overhead.ms\endcsname{5.6}
\expandafter\def\csname BAval@t18.r07.mean.inference.ms\endcsname{23.9}
\expandafter\def\csname BAval@t18.r07.p95.inference.ms\endcsname{34.3}
\expandafter\def\csname BAval@t18.r07.fps\endcsname{41.8}
\expandafter\def\csname BAval@t18.r07.decision.overhead.ms\endcsname{1.8}
\expandafter\def\csname BAval@t18.r08.mean.inference.ms\endcsname{37.8}
\expandafter\def\csname BAval@t18.r08.p95.inference.ms\endcsname{52.2}
\expandafter\def\csname BAval@t18.r08.fps\endcsname{26.4}
\expandafter\def\csname BAval@t18.r08.decision.overhead.ms\endcsname{1.8}
\expandafter\def\csname BAval@t18.r09.mean.inference.ms\endcsname{37.4}
\expandafter\def\csname BAval@t18.r09.p95.inference.ms\endcsname{51.7}
\expandafter\def\csname BAval@t18.r09.fps\endcsname{26.8}
\expandafter\def\csname BAval@t18.r09.decision.overhead.ms\endcsname{2.1}
\expandafter\def\csname BAval@t19.r01.auc.la0.pct\endcsname{67.0}
\expandafter\def\csname BAval@t19.r01.dp.la0.pct\endcsname{73.5}
\expandafter\def\csname BAval@t19.r01.mauc.pct\endcsname{69.8}
\expandafter\def\csname BAval@t19.r01.mdp.pct\endcsname{76.6}
\expandafter\def\csname BAval@t19.r02.auc.la0.pct\endcsname{66.7}
\expandafter\def\csname BAval@t19.r02.dp.la0.pct\endcsname{73.8}
\expandafter\def\csname BAval@t19.r02.mauc.pct\endcsname{69.5}
\expandafter\def\csname BAval@t19.r02.mdp.pct\endcsname{76.7}
\expandafter\def\csname BAval@t19.r03.auc.la0.pct\endcsname{64.6}
\expandafter\def\csname BAval@t19.r03.dp.la0.pct\endcsname{76.0}
\expandafter\def\csname BAval@t19.r03.mauc.pct\endcsname{66.4}
\expandafter\def\csname BAval@t19.r03.mdp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t19.r04.auc.la0.pct\endcsname{68.3}
\expandafter\def\csname BAval@t19.r04.dp.la0.pct\endcsname{78.2}
\expandafter\def\csname BAval@t19.r04.mauc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t19.r04.mdp.pct\endcsname{80.4}
\expandafter\def\csname BAval@t19.r05.auc.la0.pct\endcsname{67.7}
\expandafter\def\csname BAval@t19.r05.dp.la0.pct\endcsname{79.1}
\expandafter\def\csname BAval@t19.r05.mauc.pct\endcsname{69.8}
\expandafter\def\csname BAval@t19.r05.mdp.pct\endcsname{81.2}
\expandafter\def\csname BAval@t19.r06.auc.la0.pct\endcsname{76.9}
\expandafter\def\csname BAval@t19.r06.dp.la0.pct\endcsname{85.1}
\expandafter\def\csname BAval@t19.r06.mauc.pct\endcsname{78.1}
\expandafter\def\csname BAval@t19.r06.mdp.pct\endcsname{86.7}
\expandafter\def\csname BAval@t20.r01.auc.pct\endcsname{67.0}
\expandafter\def\csname BAval@t20.r01.dp.pct\endcsname{73.5}
\expandafter\def\csname BAval@t20.r02.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r02.dp.pct\endcsname{73.7}
\expandafter\def\csname BAval@t20.r03.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r03.dp.pct\endcsname{73.9}
\expandafter\def\csname BAval@t20.r04.auc.pct\endcsname{67.5}
\expandafter\def\csname BAval@t20.r04.dp.pct\endcsname{74.0}
\expandafter\def\csname BAval@t20.r05.auc.pct\endcsname{67.6}
\expandafter\def\csname BAval@t20.r05.dp.pct\endcsname{74.2}
\expandafter\def\csname BAval@t20.r06.auc.pct\endcsname{67.8}
\expandafter\def\csname BAval@t20.r06.dp.pct\endcsname{74.4}
\expandafter\def\csname BAval@t20.r07.auc.pct\endcsname{67.9}
\expandafter\def\csname BAval@t20.r07.dp.pct\endcsname{74.5}
\expandafter\def\csname BAval@t20.r08.auc.pct\endcsname{68.1}
\expandafter\def\csname BAval@t20.r08.dp.pct\endcsname{74.7}
\expandafter\def\csname BAval@t20.r09.auc.pct\endcsname{68.2}
\expandafter\def\csname BAval@t20.r09.dp.pct\endcsname{74.9}
\expandafter\def\csname BAval@t20.r10.auc.pct\endcsname{68.4}
\expandafter\def\csname BAval@t20.r10.dp.pct\endcsname{75.0}
\expandafter\def\csname BAval@t20.r11.auc.pct\endcsname{68.5}
\expandafter\def\csname BAval@t20.r11.dp.pct\endcsname{75.2}
\expandafter\def\csname BAval@t20.r12.auc.pct\endcsname{68.6}
\expandafter\def\csname BAval@t20.r12.dp.pct\endcsname{75.3}
\expandafter\def\csname BAval@t20.r13.auc.pct\endcsname{68.8}
\expandafter\def\csname BAval@t20.r13.dp.pct\endcsname{75.4}
\expandafter\def\csname BAval@t20.r14.auc.pct\endcsname{68.9}
\expandafter\def\csname BAval@t20.r14.dp.pct\endcsname{75.6}
\expandafter\def\csname BAval@t20.r15.auc.pct\endcsname{69.0}
\expandafter\def\csname BAval@t20.r15.dp.pct\endcsname{75.7}
\expandafter\def\csname BAval@t20.r16.auc.pct\endcsname{69.1}
\expandafter\def\csname BAval@t20.r16.dp.pct\endcsname{75.8}
\expandafter\def\csname BAval@t20.r17.auc.pct\endcsname{69.3}
\expandafter\def\csname BAval@t20.r17.dp.pct\endcsname{76.0}
\expandafter\def\csname BAval@t20.r18.auc.pct\endcsname{69.4}
\expandafter\def\csname BAval@t20.r18.dp.pct\endcsname{76.1}
\expandafter\def\csname BAval@t20.r19.auc.pct\endcsname{69.5}
\expandafter\def\csname BAval@t20.r19.dp.pct\endcsname{76.2}
\expandafter\def\csname BAval@t20.r20.auc.pct\endcsname{69.6}
\expandafter\def\csname BAval@t20.r20.dp.pct\endcsname{76.3}
\expandafter\def\csname BAval@t20.r21.auc.pct\endcsname{69.7}
\expandafter\def\csname BAval@t20.r21.dp.pct\endcsname{76.4}
\expandafter\def\csname BAval@t20.r22.auc.pct\endcsname{69.8}
\expandafter\def\csname BAval@t20.r22.dp.pct\endcsname{76.6}
\expandafter\def\csname BAval@t20.r23.auc.pct\endcsname{69.9}
\expandafter\def\csname BAval@t20.r23.dp.pct\endcsname{76.7}
\expandafter\def\csname BAval@t20.r24.auc.pct\endcsname{70.0}
\expandafter\def\csname BAval@t20.r24.dp.pct\endcsname{76.8}
\expandafter\def\csname BAval@t20.r25.auc.pct\endcsname{70.1}
\expandafter\def\csname BAval@t20.r25.dp.pct\endcsname{76.9}
\expandafter\def\csname BAval@t20.r26.auc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t20.r26.dp.pct\endcsname{77.0}
\expandafter\def\csname BAval@t20.r27.auc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t20.r27.dp.pct\endcsname{77.0}
\expandafter\def\csname BAval@t20.r28.auc.pct\endcsname{70.3}
\expandafter\def\csname BAval@t20.r28.dp.pct\endcsname{77.1}
\expandafter\def\csname BAval@t20.r29.auc.pct\endcsname{70.4}
\expandafter\def\csname BAval@t20.r29.dp.pct\endcsname{77.2}
\expandafter\def\csname BAval@t20.r30.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r30.dp.pct\endcsname{77.3}
\expandafter\def\csname BAval@t20.r31.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r31.dp.pct\endcsname{77.4}
\expandafter\def\csname BAval@t20.r32.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r32.dp.pct\endcsname{77.4}
\expandafter\def\csname BAval@t20.r33.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r33.dp.pct\endcsname{77.5}
\expandafter\def\csname BAval@t20.r34.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r34.dp.pct\endcsname{77.6}
\expandafter\def\csname BAval@t20.r35.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r35.dp.pct\endcsname{77.6}
\expandafter\def\csname BAval@t20.r36.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r36.dp.pct\endcsname{77.7}
\expandafter\def\csname BAval@t20.r37.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r37.dp.pct\endcsname{77.7}
\expandafter\def\csname BAval@t20.r38.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r38.dp.pct\endcsname{77.8}
\expandafter\def\csname BAval@t20.r39.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r39.dp.pct\endcsname{77.8}
\expandafter\def\csname BAval@t20.r40.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r40.dp.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r41.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r41.dp.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r42.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r42.dp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r43.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r43.dp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r44.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r44.dp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r45.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r45.dp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r46.auc.pct\endcsname{71.2}
\expandafter\def\csname BAval@t20.r46.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r47.auc.pct\endcsname{71.2}
\expandafter\def\csname BAval@t20.r47.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r48.auc.pct\endcsname{71.2}
\expandafter\def\csname BAval@t20.r48.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r49.auc.pct\endcsname{71.2}
\expandafter\def\csname BAval@t20.r49.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r50.auc.pct\endcsname{71.2}
\expandafter\def\csname BAval@t20.r50.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r51.auc.pct\endcsname{71.2}
\expandafter\def\csname BAval@t20.r51.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r52.auc.pct\endcsname{66.7}
\expandafter\def\csname BAval@t20.r52.dp.pct\endcsname{73.8}
\expandafter\def\csname BAval@t20.r53.auc.pct\endcsname{66.9}
\expandafter\def\csname BAval@t20.r53.dp.pct\endcsname{74.0}
\expandafter\def\csname BAval@t20.r54.auc.pct\endcsname{67.0}
\expandafter\def\csname BAval@t20.r54.dp.pct\endcsname{74.1}
\expandafter\def\csname BAval@t20.r55.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r55.dp.pct\endcsname{74.3}
\expandafter\def\csname BAval@t20.r56.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r56.dp.pct\endcsname{74.5}
\expandafter\def\csname BAval@t20.r57.auc.pct\endcsname{67.5}
\expandafter\def\csname BAval@t20.r57.dp.pct\endcsname{74.6}
\expandafter\def\csname BAval@t20.r58.auc.pct\endcsname{67.6}
\expandafter\def\csname BAval@t20.r58.dp.pct\endcsname{74.8}
\expandafter\def\csname BAval@t20.r59.auc.pct\endcsname{67.8}
\expandafter\def\csname BAval@t20.r59.dp.pct\endcsname{74.9}
\expandafter\def\csname BAval@t20.r60.auc.pct\endcsname{67.9}
\expandafter\def\csname BAval@t20.r60.dp.pct\endcsname{75.1}
\expandafter\def\csname BAval@t20.r61.auc.pct\endcsname{68.0}
\expandafter\def\csname BAval@t20.r61.dp.pct\endcsname{75.2}
\expandafter\def\csname BAval@t20.r62.auc.pct\endcsname{68.2}
\expandafter\def\csname BAval@t20.r62.dp.pct\endcsname{75.4}
\expandafter\def\csname BAval@t20.r63.auc.pct\endcsname{68.3}
\expandafter\def\csname BAval@t20.r63.dp.pct\endcsname{75.5}
\expandafter\def\csname BAval@t20.r64.auc.pct\endcsname{68.4}
\expandafter\def\csname BAval@t20.r64.dp.pct\endcsname{75.7}
\expandafter\def\csname BAval@t20.r65.auc.pct\endcsname{68.6}
\expandafter\def\csname BAval@t20.r65.dp.pct\endcsname{75.8}
\expandafter\def\csname BAval@t20.r66.auc.pct\endcsname{68.7}
\expandafter\def\csname BAval@t20.r66.dp.pct\endcsname{75.9}
\expandafter\def\csname BAval@t20.r67.auc.pct\endcsname{68.8}
\expandafter\def\csname BAval@t20.r67.dp.pct\endcsname{76.0}
\expandafter\def\csname BAval@t20.r68.auc.pct\endcsname{68.9}
\expandafter\def\csname BAval@t20.r68.dp.pct\endcsname{76.2}
\expandafter\def\csname BAval@t20.r69.auc.pct\endcsname{69.0}
\expandafter\def\csname BAval@t20.r69.dp.pct\endcsname{76.3}
\expandafter\def\csname BAval@t20.r70.auc.pct\endcsname{69.1}
\expandafter\def\csname BAval@t20.r70.dp.pct\endcsname{76.4}
\expandafter\def\csname BAval@t20.r71.auc.pct\endcsname{69.2}
\expandafter\def\csname BAval@t20.r71.dp.pct\endcsname{76.5}
\expandafter\def\csname BAval@t20.r72.auc.pct\endcsname{69.3}
\expandafter\def\csname BAval@t20.r72.dp.pct\endcsname{76.6}
\expandafter\def\csname BAval@t20.r73.auc.pct\endcsname{69.5}
\expandafter\def\csname BAval@t20.r73.dp.pct\endcsname{76.7}
\expandafter\def\csname BAval@t20.r74.auc.pct\endcsname{69.6}
\expandafter\def\csname BAval@t20.r74.dp.pct\endcsname{76.8}
\expandafter\def\csname BAval@t20.r75.auc.pct\endcsname{69.7}
\expandafter\def\csname BAval@t20.r75.dp.pct\endcsname{76.9}
\expandafter\def\csname BAval@t20.r76.auc.pct\endcsname{69.8}
\expandafter\def\csname BAval@t20.r76.dp.pct\endcsname{77.0}
\expandafter\def\csname BAval@t20.r77.auc.pct\endcsname{69.9}
\expandafter\def\csname BAval@t20.r77.dp.pct\endcsname{77.1}
\expandafter\def\csname BAval@t20.r78.auc.pct\endcsname{70.0}
\expandafter\def\csname BAval@t20.r78.dp.pct\endcsname{77.2}
\expandafter\def\csname BAval@t20.r79.auc.pct\endcsname{70.0}
\expandafter\def\csname BAval@t20.r79.dp.pct\endcsname{77.3}
\expandafter\def\csname BAval@t20.r80.auc.pct\endcsname{70.1}
\expandafter\def\csname BAval@t20.r80.dp.pct\endcsname{77.3}
\expandafter\def\csname BAval@t20.r81.auc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t20.r81.dp.pct\endcsname{77.4}
\expandafter\def\csname BAval@t20.r82.auc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t20.r82.dp.pct\endcsname{77.5}
\expandafter\def\csname BAval@t20.r83.auc.pct\endcsname{70.3}
\expandafter\def\csname BAval@t20.r83.dp.pct\endcsname{77.6}
\expandafter\def\csname BAval@t20.r84.auc.pct\endcsname{70.4}
\expandafter\def\csname BAval@t20.r84.dp.pct\endcsname{77.6}
\expandafter\def\csname BAval@t20.r85.auc.pct\endcsname{70.4}
\expandafter\def\csname BAval@t20.r85.dp.pct\endcsname{77.7}
\expandafter\def\csname BAval@t20.r86.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r86.dp.pct\endcsname{77.7}
\expandafter\def\csname BAval@t20.r87.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r87.dp.pct\endcsname{77.8}
\expandafter\def\csname BAval@t20.r88.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r88.dp.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r89.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r89.dp.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r90.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r90.dp.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r91.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r91.dp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r92.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r92.dp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r93.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r93.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r94.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r94.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r95.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r95.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r96.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r96.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r97.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r97.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r98.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r98.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r99.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r99.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r100.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r100.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r101.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r101.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r102.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r102.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r103.auc.pct\endcsname{64.6}
\expandafter\def\csname BAval@t20.r103.dp.pct\endcsname{76.0}
\expandafter\def\csname BAval@t20.r104.auc.pct\endcsname{64.7}
\expandafter\def\csname BAval@t20.r104.dp.pct\endcsname{76.1}
\expandafter\def\csname BAval@t20.r105.auc.pct\endcsname{64.8}
\expandafter\def\csname BAval@t20.r105.dp.pct\endcsname{76.2}
\expandafter\def\csname BAval@t20.r106.auc.pct\endcsname{64.9}
\expandafter\def\csname BAval@t20.r106.dp.pct\endcsname{76.4}
\expandafter\def\csname BAval@t20.r107.auc.pct\endcsname{65.0}
\expandafter\def\csname BAval@t20.r107.dp.pct\endcsname{76.5}
\expandafter\def\csname BAval@t20.r108.auc.pct\endcsname{65.1}
\expandafter\def\csname BAval@t20.r108.dp.pct\endcsname{76.6}
\expandafter\def\csname BAval@t20.r109.auc.pct\endcsname{65.2}
\expandafter\def\csname BAval@t20.r109.dp.pct\endcsname{76.7}
\expandafter\def\csname BAval@t20.r110.auc.pct\endcsname{65.3}
\expandafter\def\csname BAval@t20.r110.dp.pct\endcsname{76.8}
\expandafter\def\csname BAval@t20.r111.auc.pct\endcsname{65.4}
\expandafter\def\csname BAval@t20.r111.dp.pct\endcsname{76.9}
\expandafter\def\csname BAval@t20.r112.auc.pct\endcsname{65.5}
\expandafter\def\csname BAval@t20.r112.dp.pct\endcsname{77.0}
\expandafter\def\csname BAval@t20.r113.auc.pct\endcsname{65.5}
\expandafter\def\csname BAval@t20.r113.dp.pct\endcsname{77.1}
\expandafter\def\csname BAval@t20.r114.auc.pct\endcsname{65.7}
\expandafter\def\csname BAval@t20.r114.dp.pct\endcsname{77.2}
\expandafter\def\csname BAval@t20.r115.auc.pct\endcsname{65.8}
\expandafter\def\csname BAval@t20.r115.dp.pct\endcsname{77.3}
\expandafter\def\csname BAval@t20.r116.auc.pct\endcsname{65.9}
\expandafter\def\csname BAval@t20.r116.dp.pct\endcsname{77.4}
\expandafter\def\csname BAval@t20.r117.auc.pct\endcsname{66.0}
\expandafter\def\csname BAval@t20.r117.dp.pct\endcsname{77.5}
\expandafter\def\csname BAval@t20.r118.auc.pct\endcsname{66.0}
\expandafter\def\csname BAval@t20.r118.dp.pct\endcsname{77.6}
\expandafter\def\csname BAval@t20.r119.auc.pct\endcsname{66.1}
\expandafter\def\csname BAval@t20.r119.dp.pct\endcsname{77.7}
\expandafter\def\csname BAval@t20.r120.auc.pct\endcsname{66.2}
\expandafter\def\csname BAval@t20.r120.dp.pct\endcsname{77.7}
\expandafter\def\csname BAval@t20.r121.auc.pct\endcsname{66.2}
\expandafter\def\csname BAval@t20.r121.dp.pct\endcsname{77.8}
\expandafter\def\csname BAval@t20.r122.auc.pct\endcsname{66.3}
\expandafter\def\csname BAval@t20.r122.dp.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r123.auc.pct\endcsname{66.4}
\expandafter\def\csname BAval@t20.r123.dp.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r124.auc.pct\endcsname{66.4}
\expandafter\def\csname BAval@t20.r124.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r125.auc.pct\endcsname{66.5}
\expandafter\def\csname BAval@t20.r125.dp.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r126.auc.pct\endcsname{66.5}
\expandafter\def\csname BAval@t20.r126.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r127.auc.pct\endcsname{66.6}
\expandafter\def\csname BAval@t20.r127.dp.pct\endcsname{78.3}
\expandafter\def\csname BAval@t20.r128.auc.pct\endcsname{66.7}
\expandafter\def\csname BAval@t20.r128.dp.pct\endcsname{78.3}
\expandafter\def\csname BAval@t20.r129.auc.pct\endcsname{66.7}
\expandafter\def\csname BAval@t20.r129.dp.pct\endcsname{78.4}
\expandafter\def\csname BAval@t20.r130.auc.pct\endcsname{66.7}
\expandafter\def\csname BAval@t20.r130.dp.pct\endcsname{78.4}
\expandafter\def\csname BAval@t20.r131.auc.pct\endcsname{66.8}
\expandafter\def\csname BAval@t20.r131.dp.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r132.auc.pct\endcsname{66.8}
\expandafter\def\csname BAval@t20.r132.dp.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r133.auc.pct\endcsname{66.9}
\expandafter\def\csname BAval@t20.r133.dp.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r134.auc.pct\endcsname{66.9}
\expandafter\def\csname BAval@t20.r134.dp.pct\endcsname{78.7}
\expandafter\def\csname BAval@t20.r135.auc.pct\endcsname{67.0}
\expandafter\def\csname BAval@t20.r135.dp.pct\endcsname{78.7}
\expandafter\def\csname BAval@t20.r136.auc.pct\endcsname{67.0}
\expandafter\def\csname BAval@t20.r136.dp.pct\endcsname{78.7}
\expandafter\def\csname BAval@t20.r137.auc.pct\endcsname{67.0}
\expandafter\def\csname BAval@t20.r137.dp.pct\endcsname{78.8}
\expandafter\def\csname BAval@t20.r138.auc.pct\endcsname{67.1}
\expandafter\def\csname BAval@t20.r138.dp.pct\endcsname{78.8}
\expandafter\def\csname BAval@t20.r139.auc.pct\endcsname{67.1}
\expandafter\def\csname BAval@t20.r139.dp.pct\endcsname{78.9}
\expandafter\def\csname BAval@t20.r140.auc.pct\endcsname{67.1}
\expandafter\def\csname BAval@t20.r140.dp.pct\endcsname{78.9}
\expandafter\def\csname BAval@t20.r141.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r141.dp.pct\endcsname{78.9}
\expandafter\def\csname BAval@t20.r142.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r142.dp.pct\endcsname{78.9}
\expandafter\def\csname BAval@t20.r143.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r143.dp.pct\endcsname{79.0}
\expandafter\def\csname BAval@t20.r144.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r144.dp.pct\endcsname{79.0}
\expandafter\def\csname BAval@t20.r145.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r145.dp.pct\endcsname{79.0}
\expandafter\def\csname BAval@t20.r146.auc.pct\endcsname{67.2}
\expandafter\def\csname BAval@t20.r146.dp.pct\endcsname{79.0}
\expandafter\def\csname BAval@t20.r147.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r147.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r148.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r148.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r149.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r149.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r150.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r150.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r151.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r151.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r152.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r152.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r153.auc.pct\endcsname{67.3}
\expandafter\def\csname BAval@t20.r153.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r154.auc.pct\endcsname{68.3}
\expandafter\def\csname BAval@t20.r154.dp.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r155.auc.pct\endcsname{68.4}
\expandafter\def\csname BAval@t20.r155.dp.pct\endcsname{78.3}
\expandafter\def\csname BAval@t20.r156.auc.pct\endcsname{68.5}
\expandafter\def\csname BAval@t20.r156.dp.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r157.auc.pct\endcsname{68.5}
\expandafter\def\csname BAval@t20.r157.dp.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r158.auc.pct\endcsname{68.7}
\expandafter\def\csname BAval@t20.r158.dp.pct\endcsname{78.7}
\expandafter\def\csname BAval@t20.r159.auc.pct\endcsname{68.8}
\expandafter\def\csname BAval@t20.r159.dp.pct\endcsname{78.8}
\expandafter\def\csname BAval@t20.r160.auc.pct\endcsname{68.9}
\expandafter\def\csname BAval@t20.r160.dp.pct\endcsname{78.9}
\expandafter\def\csname BAval@t20.r161.auc.pct\endcsname{69.0}
\expandafter\def\csname BAval@t20.r161.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r162.auc.pct\endcsname{69.1}
\expandafter\def\csname BAval@t20.r162.dp.pct\endcsname{79.2}
\expandafter\def\csname BAval@t20.r163.auc.pct\endcsname{69.2}
\expandafter\def\csname BAval@t20.r163.dp.pct\endcsname{79.3}
\expandafter\def\csname BAval@t20.r164.auc.pct\endcsname{69.3}
\expandafter\def\csname BAval@t20.r164.dp.pct\endcsname{79.4}
\expandafter\def\csname BAval@t20.r165.auc.pct\endcsname{69.4}
\expandafter\def\csname BAval@t20.r165.dp.pct\endcsname{79.5}
\expandafter\def\csname BAval@t20.r166.auc.pct\endcsname{69.5}
\expandafter\def\csname BAval@t20.r166.dp.pct\endcsname{79.6}
\expandafter\def\csname BAval@t20.r167.auc.pct\endcsname{69.6}
\expandafter\def\csname BAval@t20.r167.dp.pct\endcsname{79.7}
\expandafter\def\csname BAval@t20.r168.auc.pct\endcsname{69.6}
\expandafter\def\csname BAval@t20.r168.dp.pct\endcsname{79.8}
\expandafter\def\csname BAval@t20.r169.auc.pct\endcsname{69.7}
\expandafter\def\csname BAval@t20.r169.dp.pct\endcsname{79.9}
\expandafter\def\csname BAval@t20.r170.auc.pct\endcsname{69.8}
\expandafter\def\csname BAval@t20.r170.dp.pct\endcsname{80.0}
\expandafter\def\csname BAval@t20.r171.auc.pct\endcsname{69.9}
\expandafter\def\csname BAval@t20.r171.dp.pct\endcsname{80.1}
\expandafter\def\csname BAval@t20.r172.auc.pct\endcsname{70.0}
\expandafter\def\csname BAval@t20.r172.dp.pct\endcsname{80.1}
\expandafter\def\csname BAval@t20.r173.auc.pct\endcsname{70.0}
\expandafter\def\csname BAval@t20.r173.dp.pct\endcsname{80.2}
\expandafter\def\csname BAval@t20.r174.auc.pct\endcsname{70.1}
\expandafter\def\csname BAval@t20.r174.dp.pct\endcsname{80.3}
\expandafter\def\csname BAval@t20.r175.auc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t20.r175.dp.pct\endcsname{80.4}
\expandafter\def\csname BAval@t20.r176.auc.pct\endcsname{70.3}
\expandafter\def\csname BAval@t20.r176.dp.pct\endcsname{80.5}
\expandafter\def\csname BAval@t20.r177.auc.pct\endcsname{70.3}
\expandafter\def\csname BAval@t20.r177.dp.pct\endcsname{80.5}
\expandafter\def\csname BAval@t20.r178.auc.pct\endcsname{70.4}
\expandafter\def\csname BAval@t20.r178.dp.pct\endcsname{80.6}
\expandafter\def\csname BAval@t20.r179.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r179.dp.pct\endcsname{80.7}
\expandafter\def\csname BAval@t20.r180.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r180.dp.pct\endcsname{80.7}
\expandafter\def\csname BAval@t20.r181.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r181.dp.pct\endcsname{80.8}
\expandafter\def\csname BAval@t20.r182.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r182.dp.pct\endcsname{80.9}
\expandafter\def\csname BAval@t20.r183.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r183.dp.pct\endcsname{80.9}
\expandafter\def\csname BAval@t20.r184.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r184.dp.pct\endcsname{81.0}
\expandafter\def\csname BAval@t20.r185.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r185.dp.pct\endcsname{81.0}
\expandafter\def\csname BAval@t20.r186.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r186.dp.pct\endcsname{81.1}
\expandafter\def\csname BAval@t20.r187.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r187.dp.pct\endcsname{81.1}
\expandafter\def\csname BAval@t20.r188.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r188.dp.pct\endcsname{81.2}
\expandafter\def\csname BAval@t20.r189.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r189.dp.pct\endcsname{81.2}
\expandafter\def\csname BAval@t20.r190.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r190.dp.pct\endcsname{81.2}
\expandafter\def\csname BAval@t20.r191.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r191.dp.pct\endcsname{81.3}
\expandafter\def\csname BAval@t20.r192.auc.pct\endcsname{70.9}
\expandafter\def\csname BAval@t20.r192.dp.pct\endcsname{81.3}
\expandafter\def\csname BAval@t20.r193.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r193.dp.pct\endcsname{81.3}
\expandafter\def\csname BAval@t20.r194.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r194.dp.pct\endcsname{81.4}
\expandafter\def\csname BAval@t20.r195.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r195.dp.pct\endcsname{81.4}
\expandafter\def\csname BAval@t20.r196.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r196.dp.pct\endcsname{81.4}
\expandafter\def\csname BAval@t20.r197.auc.pct\endcsname{71.0}
\expandafter\def\csname BAval@t20.r197.dp.pct\endcsname{81.4}
\expandafter\def\csname BAval@t20.r198.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r198.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r199.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r199.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r200.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r200.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r201.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r201.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r202.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r202.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r203.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r203.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r204.auc.pct\endcsname{71.1}
\expandafter\def\csname BAval@t20.r204.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r205.auc.pct\endcsname{67.7}
\expandafter\def\csname BAval@t20.r205.dp.pct\endcsname{79.1}
\expandafter\def\csname BAval@t20.r206.auc.pct\endcsname{67.8}
\expandafter\def\csname BAval@t20.r206.dp.pct\endcsname{79.2}
\expandafter\def\csname BAval@t20.r207.auc.pct\endcsname{67.9}
\expandafter\def\csname BAval@t20.r207.dp.pct\endcsname{79.3}
\expandafter\def\csname BAval@t20.r208.auc.pct\endcsname{68.0}
\expandafter\def\csname BAval@t20.r208.dp.pct\endcsname{79.4}
\expandafter\def\csname BAval@t20.r209.auc.pct\endcsname{68.1}
\expandafter\def\csname BAval@t20.r209.dp.pct\endcsname{79.6}
\expandafter\def\csname BAval@t20.r210.auc.pct\endcsname{68.3}
\expandafter\def\csname BAval@t20.r210.dp.pct\endcsname{79.7}
\expandafter\def\csname BAval@t20.r211.auc.pct\endcsname{68.4}
\expandafter\def\csname BAval@t20.r211.dp.pct\endcsname{79.8}
\expandafter\def\csname BAval@t20.r212.auc.pct\endcsname{68.5}
\expandafter\def\csname BAval@t20.r212.dp.pct\endcsname{79.9}
\expandafter\def\csname BAval@t20.r213.auc.pct\endcsname{68.7}
\expandafter\def\csname BAval@t20.r213.dp.pct\endcsname{80.1}
\expandafter\def\csname BAval@t20.r214.auc.pct\endcsname{68.8}
\expandafter\def\csname BAval@t20.r214.dp.pct\endcsname{80.2}
\expandafter\def\csname BAval@t20.r215.auc.pct\endcsname{68.8}
\expandafter\def\csname BAval@t20.r215.dp.pct\endcsname{80.3}
\expandafter\def\csname BAval@t20.r216.auc.pct\endcsname{68.9}
\expandafter\def\csname BAval@t20.r216.dp.pct\endcsname{80.4}
\expandafter\def\csname BAval@t20.r217.auc.pct\endcsname{69.0}
\expandafter\def\csname BAval@t20.r217.dp.pct\endcsname{80.5}
\expandafter\def\csname BAval@t20.r218.auc.pct\endcsname{69.1}
\expandafter\def\csname BAval@t20.r218.dp.pct\endcsname{80.6}
\expandafter\def\csname BAval@t20.r219.auc.pct\endcsname{69.2}
\expandafter\def\csname BAval@t20.r219.dp.pct\endcsname{80.6}
\expandafter\def\csname BAval@t20.r220.auc.pct\endcsname{69.3}
\expandafter\def\csname BAval@t20.r220.dp.pct\endcsname{80.7}
\expandafter\def\csname BAval@t20.r221.auc.pct\endcsname{69.4}
\expandafter\def\csname BAval@t20.r221.dp.pct\endcsname{80.8}
\expandafter\def\csname BAval@t20.r222.auc.pct\endcsname{69.4}
\expandafter\def\csname BAval@t20.r222.dp.pct\endcsname{80.9}
\expandafter\def\csname BAval@t20.r223.auc.pct\endcsname{69.5}
\expandafter\def\csname BAval@t20.r223.dp.pct\endcsname{81.0}
\expandafter\def\csname BAval@t20.r224.auc.pct\endcsname{69.6}
\expandafter\def\csname BAval@t20.r224.dp.pct\endcsname{81.0}
\expandafter\def\csname BAval@t20.r225.auc.pct\endcsname{69.7}
\expandafter\def\csname BAval@t20.r225.dp.pct\endcsname{81.1}
\expandafter\def\csname BAval@t20.r226.auc.pct\endcsname{69.7}
\expandafter\def\csname BAval@t20.r226.dp.pct\endcsname{81.2}
\expandafter\def\csname BAval@t20.r227.auc.pct\endcsname{69.8}
\expandafter\def\csname BAval@t20.r227.dp.pct\endcsname{81.3}
\expandafter\def\csname BAval@t20.r228.auc.pct\endcsname{69.9}
\expandafter\def\csname BAval@t20.r228.dp.pct\endcsname{81.3}
\expandafter\def\csname BAval@t20.r229.auc.pct\endcsname{69.9}
\expandafter\def\csname BAval@t20.r229.dp.pct\endcsname{81.4}
\expandafter\def\csname BAval@t20.r230.auc.pct\endcsname{70.1}
\expandafter\def\csname BAval@t20.r230.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r231.auc.pct\endcsname{70.1}
\expandafter\def\csname BAval@t20.r231.dp.pct\endcsname{81.5}
\expandafter\def\csname BAval@t20.r232.auc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t20.r232.dp.pct\endcsname{81.6}
\expandafter\def\csname BAval@t20.r233.auc.pct\endcsname{70.2}
\expandafter\def\csname BAval@t20.r233.dp.pct\endcsname{81.6}
\expandafter\def\csname BAval@t20.r234.auc.pct\endcsname{70.3}
\expandafter\def\csname BAval@t20.r234.dp.pct\endcsname{81.7}
\expandafter\def\csname BAval@t20.r235.auc.pct\endcsname{70.3}
\expandafter\def\csname BAval@t20.r235.dp.pct\endcsname{81.7}
\expandafter\def\csname BAval@t20.r236.auc.pct\endcsname{70.4}
\expandafter\def\csname BAval@t20.r236.dp.pct\endcsname{81.8}
\expandafter\def\csname BAval@t20.r237.auc.pct\endcsname{70.4}
\expandafter\def\csname BAval@t20.r237.dp.pct\endcsname{81.8}
\expandafter\def\csname BAval@t20.r238.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r238.dp.pct\endcsname{81.9}
\expandafter\def\csname BAval@t20.r239.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r239.dp.pct\endcsname{81.9}
\expandafter\def\csname BAval@t20.r240.auc.pct\endcsname{70.5}
\expandafter\def\csname BAval@t20.r240.dp.pct\endcsname{81.9}
\expandafter\def\csname BAval@t20.r241.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r241.dp.pct\endcsname{82.0}
\expandafter\def\csname BAval@t20.r242.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r242.dp.pct\endcsname{82.0}
\expandafter\def\csname BAval@t20.r243.auc.pct\endcsname{70.6}
\expandafter\def\csname BAval@t20.r243.dp.pct\endcsname{82.0}
\expandafter\def\csname BAval@t20.r244.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r244.dp.pct\endcsname{82.2}
\expandafter\def\csname BAval@t20.r245.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r245.dp.pct\endcsname{82.2}
\expandafter\def\csname BAval@t20.r246.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r246.dp.pct\endcsname{82.2}
\expandafter\def\csname BAval@t20.r247.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r247.dp.pct\endcsname{82.2}
\expandafter\def\csname BAval@t20.r248.auc.pct\endcsname{70.7}
\expandafter\def\csname BAval@t20.r248.dp.pct\endcsname{82.2}
\expandafter\def\csname BAval@t20.r249.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r249.dp.pct\endcsname{82.3}
\expandafter\def\csname BAval@t20.r250.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r250.dp.pct\endcsname{82.3}
\expandafter\def\csname BAval@t20.r251.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r251.dp.pct\endcsname{82.3}
\expandafter\def\csname BAval@t20.r252.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r252.dp.pct\endcsname{82.3}
\expandafter\def\csname BAval@t20.r253.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r253.dp.pct\endcsname{82.3}
\expandafter\def\csname BAval@t20.r254.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r254.dp.pct\endcsname{82.3}
\expandafter\def\csname BAval@t20.r255.auc.pct\endcsname{70.8}
\expandafter\def\csname BAval@t20.r255.dp.pct\endcsname{82.3}
\expandafter\def\csname BAval@t20.r256.auc.pct\endcsname{76.9}
\expandafter\def\csname BAval@t20.r256.dp.pct\endcsname{85.1}
\expandafter\def\csname BAval@t20.r257.auc.pct\endcsname{77.0}
\expandafter\def\csname BAval@t20.r257.dp.pct\endcsname{85.2}
\expandafter\def\csname BAval@t20.r258.auc.pct\endcsname{77.1}
\expandafter\def\csname BAval@t20.r258.dp.pct\endcsname{85.2}
\expandafter\def\csname BAval@t20.r259.auc.pct\endcsname{77.2}
\expandafter\def\csname BAval@t20.r259.dp.pct\endcsname{85.3}
\expandafter\def\csname BAval@t20.r260.auc.pct\endcsname{77.2}
\expandafter\def\csname BAval@t20.r260.dp.pct\endcsname{85.4}
\expandafter\def\csname BAval@t20.r261.auc.pct\endcsname{77.2}
\expandafter\def\csname BAval@t20.r261.dp.pct\endcsname{85.5}
\expandafter\def\csname BAval@t20.r262.auc.pct\endcsname{77.3}
\expandafter\def\csname BAval@t20.r262.dp.pct\endcsname{85.6}
\expandafter\def\csname BAval@t20.r263.auc.pct\endcsname{77.4}
\expandafter\def\csname BAval@t20.r263.dp.pct\endcsname{85.7}
\expandafter\def\csname BAval@t20.r264.auc.pct\endcsname{77.4}
\expandafter\def\csname BAval@t20.r264.dp.pct\endcsname{85.7}
\expandafter\def\csname BAval@t20.r265.auc.pct\endcsname{77.5}
\expandafter\def\csname BAval@t20.r265.dp.pct\endcsname{85.8}
\expandafter\def\csname BAval@t20.r266.auc.pct\endcsname{77.5}
\expandafter\def\csname BAval@t20.r266.dp.pct\endcsname{85.9}
\expandafter\def\csname BAval@t20.r267.auc.pct\endcsname{77.6}
\expandafter\def\csname BAval@t20.r267.dp.pct\endcsname{86.0}
\expandafter\def\csname BAval@t20.r268.auc.pct\endcsname{77.6}
\expandafter\def\csname BAval@t20.r268.dp.pct\endcsname{86.1}
\expandafter\def\csname BAval@t20.r269.auc.pct\endcsname{77.7}
\expandafter\def\csname BAval@t20.r269.dp.pct\endcsname{86.1}
\expandafter\def\csname BAval@t20.r270.auc.pct\endcsname{77.8}
\expandafter\def\csname BAval@t20.r270.dp.pct\endcsname{86.2}
\expandafter\def\csname BAval@t20.r271.auc.pct\endcsname{77.8}
\expandafter\def\csname BAval@t20.r271.dp.pct\endcsname{86.3}
\expandafter\def\csname BAval@t20.r272.auc.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r272.dp.pct\endcsname{86.3}
\expandafter\def\csname BAval@t20.r273.auc.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r273.dp.pct\endcsname{86.4}
\expandafter\def\csname BAval@t20.r274.auc.pct\endcsname{77.9}
\expandafter\def\csname BAval@t20.r274.dp.pct\endcsname{86.5}
\expandafter\def\csname BAval@t20.r275.auc.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r275.dp.pct\endcsname{86.5}
\expandafter\def\csname BAval@t20.r276.auc.pct\endcsname{78.0}
\expandafter\def\csname BAval@t20.r276.dp.pct\endcsname{86.6}
\expandafter\def\csname BAval@t20.r277.auc.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r277.dp.pct\endcsname{86.7}
\expandafter\def\csname BAval@t20.r278.auc.pct\endcsname{78.1}
\expandafter\def\csname BAval@t20.r278.dp.pct\endcsname{86.7}
\expandafter\def\csname BAval@t20.r279.auc.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r279.dp.pct\endcsname{86.8}
\expandafter\def\csname BAval@t20.r280.auc.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r280.dp.pct\endcsname{86.8}
\expandafter\def\csname BAval@t20.r281.auc.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r281.dp.pct\endcsname{86.9}
\expandafter\def\csname BAval@t20.r282.auc.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r282.dp.pct\endcsname{86.9}
\expandafter\def\csname BAval@t20.r283.auc.pct\endcsname{78.2}
\expandafter\def\csname BAval@t20.r283.dp.pct\endcsname{87.0}
\expandafter\def\csname BAval@t20.r284.auc.pct\endcsname{78.3}
\expandafter\def\csname BAval@t20.r284.dp.pct\endcsname{87.0}
\expandafter\def\csname BAval@t20.r285.auc.pct\endcsname{78.3}
\expandafter\def\csname BAval@t20.r285.dp.pct\endcsname{87.1}
\expandafter\def\csname BAval@t20.r286.auc.pct\endcsname{78.3}
\expandafter\def\csname BAval@t20.r286.dp.pct\endcsname{87.1}
\expandafter\def\csname BAval@t20.r287.auc.pct\endcsname{78.4}
\expandafter\def\csname BAval@t20.r287.dp.pct\endcsname{87.1}
\expandafter\def\csname BAval@t20.r288.auc.pct\endcsname{78.4}
\expandafter\def\csname BAval@t20.r288.dp.pct\endcsname{87.2}
\expandafter\def\csname BAval@t20.r289.auc.pct\endcsname{78.4}
\expandafter\def\csname BAval@t20.r289.dp.pct\endcsname{87.2}
\expandafter\def\csname BAval@t20.r290.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r290.dp.pct\endcsname{87.2}
\expandafter\def\csname BAval@t20.r291.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r291.dp.pct\endcsname{87.3}
\expandafter\def\csname BAval@t20.r292.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r292.dp.pct\endcsname{87.3}
\expandafter\def\csname BAval@t20.r293.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r293.dp.pct\endcsname{87.3}
\expandafter\def\csname BAval@t20.r294.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r294.dp.pct\endcsname{87.4}
\expandafter\def\csname BAval@t20.r295.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r295.dp.pct\endcsname{87.4}
\expandafter\def\csname BAval@t20.r296.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r296.dp.pct\endcsname{87.4}
\expandafter\def\csname BAval@t20.r297.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r297.dp.pct\endcsname{87.4}
\expandafter\def\csname BAval@t20.r298.auc.pct\endcsname{78.5}
\expandafter\def\csname BAval@t20.r298.dp.pct\endcsname{87.4}
\expandafter\def\csname BAval@t20.r299.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r299.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t20.r300.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r300.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t20.r301.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r301.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t20.r302.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r302.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t20.r303.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r303.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t20.r304.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r304.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t20.r305.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r305.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t20.r306.auc.pct\endcsname{78.6}
\expandafter\def\csname BAval@t20.r306.dp.pct\endcsname{87.5}
\expandafter\def\csname BAval@t21.r01.car.pct\endcsname{89.3}
\expandafter\def\csname BAval@t21.r02.car.pct\endcsname{91.5}
\expandafter\def\csname BAval@t21.r03.car.pct\endcsname{95.0}
\expandafter\def\csname BAval@t21.r04.car.pct\endcsname{93.2}
\expandafter\def\csname BAval@t21.r05.car.pct\endcsname{94.0}
\expandafter\def\csname BAval@t22.r01.full.s.id.pct\endcsname{75.8}
\expandafter\def\csname BAval@t22.r01.ablated.s.id.pct\endcsname{67.7}
\expandafter\def\csname BAval@t22.r01.drop.pp\endcsname{8.2}
\expandafter\def\csname BAval@t22.r02.full.s.id.pct\endcsname{87.0}
\expandafter\def\csname BAval@t22.r02.ablated.s.id.pct\endcsname{85.8}
\expandafter\def\csname BAval@t22.r02.drop.pp\endcsname{1.1}
\expandafter\def\csname BAval@t22.r03.full.s.id.pct\endcsname{80.1}
\expandafter\def\csname BAval@t22.r03.ablated.s.id.pct\endcsname{73.8}
\expandafter\def\csname BAval@t22.r03.drop.pp\endcsname{6.3}
\expandafter\def\csname BAval@t22.r04.full.s.id.pct\endcsname{84.6}
\expandafter\def\csname BAval@t22.r04.ablated.s.id.pct\endcsname{84.2}
\expandafter\def\csname BAval@t22.r04.drop.pp\endcsname{0.4}
\expandafter\def\csname BAval@t23.r01.sid\endcsname{78.1}
\expandafter\def\csname BAval@t23.r02.sid\endcsname{81.0}
\expandafter\def\csname BAval@t23.r03.sid\endcsname{81.7}
\expandafter\def\csname BAval@t24.r01.sid\endcsname{81.6}
\expandafter\def\csname BAval@t24.r01.wrong\endcsname{4.9}
\expandafter\def\csname BAval@t24.r01.recovery\endcsname{84.6}
\expandafter\def\csname BAval@t24.r01.t5\endcsname{1.5}
\expandafter\def\csname BAval@t24.r02.sid\endcsname{82.1}
\expandafter\def\csname BAval@t24.r02.wrong\endcsname{4.7}
\expandafter\def\csname BAval@t24.r02.recovery\endcsname{85.8}
\expandafter\def\csname BAval@t24.r02.t5\endcsname{1.4}
\expandafter\def\csname BAval@t24.r03.sid\endcsname{82.3}
\expandafter\def\csname BAval@t24.r03.wrong\endcsname{4.4}
\expandafter\def\csname BAval@t24.r03.recovery\endcsname{86.2}
\expandafter\def\csname BAval@t24.r03.t5\endcsname{1.4}
\expandafter\def\csname BAval@t24.r04.sid\endcsname{82.1}
\expandafter\def\csname BAval@t24.r04.wrong\endcsname{4.2}
\expandafter\def\csname BAval@t24.r04.recovery\endcsname{85.8}
\expandafter\def\csname BAval@t24.r04.t5\endcsname{1.4}
\expandafter\def\csname BAval@t25.r01.value\endcsname{1.00}
\expandafter\def\csname BAval@t25.r02.value\endcsname{0.50}
\expandafter\def\csname BAval@t25.r03.value\endcsname{0.10}
\expandafter\def\csname BAval@t25.r04.value\endcsname{1.00}
\expandafter\def\csname BAval@t25.r05.value\endcsname{0.20}
\expandafter\def\csname BAval@t25.r06.value\endcsname{0.01}
\expandafter\def\csname BAval@t25.r07.value\endcsname{0.01}
\expandafter\def\csname BAval@t25.r08.value\endcsname{0.05}
\expandafter\def\csname BAval@t26.r01.decisions\endcsname{17}
\expandafter\def\csname BAval@t26.r01.completed\endcsname{16}
\expandafter\def\csname BAval@t26.r01.timeouts\endcsname{1}
\expandafter\def\csname BAval@t26.r01.completion.pct\endcsname{94.1}
\expandafter\def\csname BAval@t26.r01.fallback.pct\endcsname{5.9}
\expandafter\def\csname BAval@t26.r02.decisions\endcsname{12}
\expandafter\def\csname BAval@t26.r02.completed\endcsname{11}
\expandafter\def\csname BAval@t26.r02.timeouts\endcsname{1}
\expandafter\def\csname BAval@t26.r02.completion.pct\endcsname{91.7}
\expandafter\def\csname BAval@t26.r02.fallback.pct\endcsname{8.3}
\expandafter\def\csname BAval@t27.r01.total.s\endcsname{9.00}
\expandafter\def\csname BAval@t27.r01.correct.s\endcsname{7.40}
\expandafter\def\csname BAval@t27.r01.wrong.s\endcsname{0.22}
\expandafter\def\csname BAval@t27.r01.sid\endcsname{82.3}
\expandafter\def\csname BAval@t27.r01.wrong\endcsname{2.4}
\expandafter\def\csname BAval@t27.r02.total.s\endcsname{9.00}
\expandafter\def\csname BAval@t27.r02.correct.s\endcsname{7.06}
\expandafter\def\csname BAval@t27.r02.wrong.s\endcsname{0.36}
\expandafter\def\csname BAval@t27.r02.sid\endcsname{78.5}
\expandafter\def\csname BAval@t27.r02.wrong\endcsname{4.0}
\expandafter\def\csname BAval@ext.best.sid\endcsname{75.2}
\expandafter\def\csname BAval@ext.best.wrong\endcsname{7.3}
\expandafter\def\csname BAval@ext.best.recovery\endcsname{79.0}
\expandafter\def\csname BAval@ext.best.t5\endcsname{2.0}
\expandafter\def\csname BAval@ext.bind.sid\endcsname{82.3}
\expandafter\def\csname BAval@ext.bind.wrong\endcsname{4.4}
\expandafter\def\csname BAval@ext.bind.recovery\endcsname{86.2}
\expandafter\def\csname BAval@ext.bind.t5\endcsname{1.4}
\expandafter\def\csname BAval@ext.joint.sid\endcsname{74.6}
\expandafter\def\csname BAval@ext.joint.wrong\endcsname{6.9}
\expandafter\def\csname BAval@ext.joint.recovery\endcsname{77.9}
\expandafter\def\csname BAval@ext.joint.t5\endcsname{2.0}
\expandafter\def\csname BAval@ext.dam.sid\endcsname{70.3}
\expandafter\def\csname BAval@ext.dam.wrong\endcsname{8.1}
\expandafter\def\csname BAval@ext.dam.recovery\endcsname{74.0}
\expandafter\def\csname BAval@ext.dam.t5\endcsname{2.2}
\expandafter\def\csname BAval@int.joint.sid\endcsname{70.3}
\expandafter\def\csname BAval@int.joint.wrong\endcsname{8.8}
\expandafter\def\csname BAval@int.joint.recovery\endcsname{72.0}
\expandafter\def\csname BAval@int.joint.t5\endcsname{2.4}
\expandafter\def\csname BAval@int.bind.sid\endcsname{82.3}
\expandafter\def\csname BAval@int.bind.wrong\endcsname{4.4}
\expandafter\def\csname BAval@int.bind.recovery\endcsname{86.2}
\expandafter\def\csname BAval@int.bind.t5\endcsname{1.4}
\expandafter\def\csname BAval@int.oracle.sid\endcsname{87.9}
\expandafter\def\csname BAval@int.oracle.wrong\endcsname{1.6}
\expandafter\def\csname BAval@int.oracle.recovery\endcsname{92.0}
\expandafter\def\csname BAval@int.oracle.t5\endcsname{1.2}
\expandafter\def\csname BAval@int.temporal.sid\endcsname{68.7}
\expandafter\def\csname BAval@int.temporal.wrong\endcsname{10.1}
\expandafter\def\csname BAval@int.temporal.recovery\endcsname{70.0}
\expandafter\def\csname BAval@int.temporal.t5\endcsname{2.5}
\expandafter\def\csname BAval@budget.bind075.sid\endcsname{77.1}
\expandafter\def\csname BAval@budget.joint075.sid\endcsname{64.0}
\expandafter\def\csname BAval@budget.joint100.sid\endcsname{70.3}
\expandafter\def\csname BAval@swap.refsep\endcsname{65.9}
\expandafter\def\csname BAval@swap.refjoint\endcsname{70.3}
\expandafter\def\csname BAval@swap.bindsep\endcsname{77.6}
\expandafter\def\csname BAval@swap.bindjoint\endcsname{82.3}
\expandafter\def\csname BAval@delta.ext.sid\endcsname{7.1}
\expandafter\def\csname BAval@delta.swap.refplanner\endcsname{4.4}
\expandafter\def\csname BAval@delta.swap.bindplanner\endcsname{4.7}
\expandafter\def\csname BAval@delta.swap.sepresponse\endcsname{11.8}
\expandafter\def\csname BAval@delta.swap.jointresponse\endcsname{12.0}
\expandafter\def\csname BAval@delta.ext.wrong\endcsname{2.9}
\expandafter\def\csname BAval@delta.ext.recovery\endcsname{7.2}
\expandafter\def\csname BAval@delta.swap.interaction\endcsname{0.2}
\expandafter\def\csname BAval@gap.remaining\endcsname{5.6}
\expandafter\def\csname BAval@gap.external\endcsname{55.7}
\expandafter\def\csname BAval@gap.internal\endcsname{68.1}
\expandafter\def\csname BAval@delta.ext.wrong.relative\endcsname{39.2}
\expandafter\def\csname BAval@delta.ext.t5\endcsname{0.6}
\expandafter\def\csname BAval@sweep.zero.bind\endcsname{86.1}
\expandafter\def\csname BAval@sweep.zero.best\endcsname{82.0}
\expandafter\def\csname BAval@delta.sweep.zero\endcsname{4.1}
\expandafter\def\csname BAval@sweep.ref.bind\endcsname{82.3}
\expandafter\def\csname BAval@sweep.ref.best\endcsname{75.2}
\expandafter\def\csname BAval@delta.sweep.ref\endcsname{7.1}
\expandafter\def\csname BAval@sweep.two.bind\endcsname{64.0}
\expandafter\def\csname BAval@sweep.two.best\endcsname{51.9}
\expandafter\def\csname BAval@delta.sweep.two\endcsname{12.2}
\expandafter\def\csname BAval@sweep.cap075.bind\endcsname{77.1}
\expandafter\def\csname BAval@sweep.cap075.best\endcsname{69.5}
\expandafter\def\csname BAval@delta.sweep.cap075\endcsname{7.6}
\expandafter\def\csname BAval@sweep.cap200.bind\endcsname{86.2}
\expandafter\def\csname BAval@sweep.cap200.best\endcsname{80.8}
\expandafter\def\csname BAval@delta.sweep.cap200\endcsname{5.4}
\expandafter\def\csname BAval@strata.bind.short\endcsname{90.2}
\expandafter\def\csname BAval@strata.best.short\endcsname{86.2}
\expandafter\def\csname BAval@delta.strata.short\endcsname{4.1}
\expandafter\def\csname BAval@strata.bind.similar\endcsname{85.4}
\expandafter\def\csname BAval@strata.best.similar\endcsname{79.2}
\expandafter\def\csname BAval@delta.strata.similar\endcsname{6.2}
\expandafter\def\csname BAval@strata.bind.long\endcsname{73.9}
\expandafter\def\csname BAval@strata.best.long\endcsname{63.9}
\expandafter\def\csname BAval@delta.strata.long\endcsname{10.0}
\expandafter\def\csname BAval@delta.backbone.ost\endcsname{8.3}
\expandafter\def\csname BAval@delta.backbone.lorat\endcsname{7.6}
\expandafter\def\csname BAval@delta.backbone.dam\endcsname{7.1}
\expandafter\def\csname BAval@runtime.best.mean\endcsname{37.8}
\expandafter\def\csname BAval@runtime.best.p95\endcsname{52.2}
\expandafter\def\csname BAval@runtime.best.fps\endcsname{26.4}
\expandafter\def\csname BAval@runtime.best.decision\endcsname{1.8}
\expandafter\def\csname BAval@runtime.bind.mean\endcsname{37.4}
\expandafter\def\csname BAval@runtime.bind.p95\endcsname{51.7}
\expandafter\def\csname BAval@runtime.bind.fps\endcsname{26.8}
\expandafter\def\csname BAval@runtime.bind.decision\endcsname{2.1}
\expandafter\def\csname BAval@lt.best.fmax\endcsname{78.9}
\expandafter\def\csname BAval@lt.bind.fmax\endcsname{85.0}
\expandafter\def\csname BAval@car.bind\endcsname{94.0}
\expandafter\def\csname BAval@car.oa\endcsname{95.0}
\expandafter\def\csname BAval@fixed.bind.ao\endcsname{79.1}
\expandafter\def\csname BAval@fixed.lorat.ao\endcsname{72.7}
\expandafter\def\csname BAval@fixed.dam.ao\endcsname{73.3}
\expandafter\def\csname BAval@delta.fixed.lorat.ao\endcsname{6.3}
\expandafter\def\csname BAval@delta.fixed.dam.ao\endcsname{5.8}
\expandafter\def\csname BAval@fixed.bind.sao\endcsname{76.9}
\expandafter\def\csname BAval@fixed.lorat.sao\endcsname{67.0}
\expandafter\def\csname BAval@fixed.dam.sao\endcsname{66.7}
\expandafter\def\csname BAval@delta.fixed.lorat.sao\endcsname{10.0}
\expandafter\def\csname BAval@delta.fixed.dam.sao\endcsname{10.3}
\expandafter\def\csname BAval@rec.quad.attempts\endcsname{17}
\expandafter\def\csname BAval@rec.quad.complete\endcsname{0}
\expandafter\def\csname BAval@rec.quad.fallwait\endcsname{16}
\expandafter\def\csname BAval@rec.quad.expired\endcsname{1}
\expandafter\def\csname BAval@rec.quad.requests\endcsname{0}
\expandafter\def\csname BAval@rec.quad.returns\endcsname{0}
\expandafter\def\csname BAval@rec.quad.initialpub\endcsname{1}
\expandafter\def\csname BAval@rec.quad.laterpub\endcsname{0}
\expandafter\def\csname BAval@rec.quad.nativeupdates\endcsname{0}
\expandafter\def\csname BAval@rec.quad.ticks\endcsname{90}
\expandafter\def\csname BAval@state.quad.dam.correct\endcsname{1}
\expandafter\def\csname BAval@state.quad.dam.wrong\endcsname{10}
\expandafter\def\csname BAval@state.quad.dam.unresolved\endcsname{61}
\expandafter\def\csname BAval@state.quad.dam.unknown\endcsname{18}
\expandafter\def\csname BAval@tick.quad.f409.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.quad.f409.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.quad.f410.dam.iou\endcsname{0.36}
\expandafter\def\csname BAval@tick.quad.f410.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f411.dam.iou\endcsname{0.27}
\expandafter\def\csname BAval@tick.quad.f411.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f412.dam.iou\endcsname{0.10}
\expandafter\def\csname BAval@tick.quad.f412.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f413.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f413.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f414.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f414.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f415.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f415.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f416.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f416.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f417.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f417.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f418.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f418.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f419.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f419.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f420.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f420.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f421.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f421.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f422.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f422.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f423.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f423.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f424.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f424.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f425.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f425.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f426.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f426.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f427.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f427.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f428.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f428.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f429.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f429.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f430.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f430.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f431.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f431.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f432.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f432.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f433.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f433.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f434.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f434.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f435.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f435.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f436.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f436.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f437.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f437.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f438.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f438.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f439.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f439.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f440.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f440.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f441.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f441.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f442.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f442.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f443.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f443.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f444.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f444.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f445.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f445.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f446.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f446.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f447.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f447.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f448.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f448.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f449.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f449.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f450.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f450.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f451.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f451.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f452.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f452.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f453.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f453.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f454.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f454.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f455.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f455.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f456.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f456.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f457.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f457.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f458.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f458.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f459.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f459.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f460.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f460.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f461.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f461.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f462.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f462.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f463.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f463.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f464.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f464.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f465.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f465.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f466.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f466.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f467.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f467.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f468.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f468.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f469.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f469.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f470.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f470.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f471.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f471.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f472.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f472.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f473.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f473.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f474.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f474.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f475.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f475.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f476.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f476.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f477.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f477.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f478.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f478.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f479.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f479.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f480.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f480.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f481.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f481.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f482.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f482.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f483.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f483.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f484.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f484.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f485.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f485.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f486.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f486.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f487.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f487.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f488.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f488.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f489.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f489.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f490.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f490.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f491.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f491.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f492.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f492.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f493.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f493.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f494.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f494.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f495.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f495.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f496.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f496.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f497.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f497.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f498.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f498.dam.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@state.quad.keep.correct\endcsname{1}
\expandafter\def\csname BAval@state.quad.keep.wrong\endcsname{12}
\expandafter\def\csname BAval@state.quad.keep.unresolved\endcsname{59}
\expandafter\def\csname BAval@state.quad.keep.unknown\endcsname{18}
\expandafter\def\csname BAval@tick.quad.f409.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.quad.f409.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.quad.f410.keep.iou\endcsname{0.36}
\expandafter\def\csname BAval@tick.quad.f410.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f411.keep.iou\endcsname{0.27}
\expandafter\def\csname BAval@tick.quad.f411.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f412.keep.iou\endcsname{0.10}
\expandafter\def\csname BAval@tick.quad.f412.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f413.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f413.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f414.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f414.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f415.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f415.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f416.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f416.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f417.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f417.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f418.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f418.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f419.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f419.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f420.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f420.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f421.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f421.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f422.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f422.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f423.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f423.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f424.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f424.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f425.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f425.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f426.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f426.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f427.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f427.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f428.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f428.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f429.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f429.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f430.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f430.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f431.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f431.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f432.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f432.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f433.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f433.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f434.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f434.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f435.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f435.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f436.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f436.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f437.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f437.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f438.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f438.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f439.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f439.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f440.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f440.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f441.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f441.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f442.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f442.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f443.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f443.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f444.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f444.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f445.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f445.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f446.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f446.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f447.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f447.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f448.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f448.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f449.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f449.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f450.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f450.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f451.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f451.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f452.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f452.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f453.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f453.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f454.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f454.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f455.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f455.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f456.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f456.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f457.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f457.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f458.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f458.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f459.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f459.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f460.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f460.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f461.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f461.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f462.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f462.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f463.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f463.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f464.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f464.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f465.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f465.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f466.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f466.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f467.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f467.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f468.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f468.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f469.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f469.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f470.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f470.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f471.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f471.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f472.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f472.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f473.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f473.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f474.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f474.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f475.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f475.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f476.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f476.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f477.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f477.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f478.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f478.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f479.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f479.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f480.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f480.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f481.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f481.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f482.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f482.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f483.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f483.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f484.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f484.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f485.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f485.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f486.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f486.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f487.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f487.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f488.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f488.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f489.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f489.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f490.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f490.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f491.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f491.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f492.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f492.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f493.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f493.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f494.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f494.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f495.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f495.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f496.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f496.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f497.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f497.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f498.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f498.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@state.quad.bind.correct\endcsname{1}
\expandafter\def\csname BAval@state.quad.bind.wrong\endcsname{12}
\expandafter\def\csname BAval@state.quad.bind.unresolved\endcsname{59}
\expandafter\def\csname BAval@state.quad.bind.unknown\endcsname{18}
\expandafter\def\csname BAval@tick.quad.f409.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.quad.f409.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.quad.f410.bind.iou\endcsname{0.36}
\expandafter\def\csname BAval@tick.quad.f410.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f411.bind.iou\endcsname{0.27}
\expandafter\def\csname BAval@tick.quad.f411.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f412.bind.iou\endcsname{0.10}
\expandafter\def\csname BAval@tick.quad.f412.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f413.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f413.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f414.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f414.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f415.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f415.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f416.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f416.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f417.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f417.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f418.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f418.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f419.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f419.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f420.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f420.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f421.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f421.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f422.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f422.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f423.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f423.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f424.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f424.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f425.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f425.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f426.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f426.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f427.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f427.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f428.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f428.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f429.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f429.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f430.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f430.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f431.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f431.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f432.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f432.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f433.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f433.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f434.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f434.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f435.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f435.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f436.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f436.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f437.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f437.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f438.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f438.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f439.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f439.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f440.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f440.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f441.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f441.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f442.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f442.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f443.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f443.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f444.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f444.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f445.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f445.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f446.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f446.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f447.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f447.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f448.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f448.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f449.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f449.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f450.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f450.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f451.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f451.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f452.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f452.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f453.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f453.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f454.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f454.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f455.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f455.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f456.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f456.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f457.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f457.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f458.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f458.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f459.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f459.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f460.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f460.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f461.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f461.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f462.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f462.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f463.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f463.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f464.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f464.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f465.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f465.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f466.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f466.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f467.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f467.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f468.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f468.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f469.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f469.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f470.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f470.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f471.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f471.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f472.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f472.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f473.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f473.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f474.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f474.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f475.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f475.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f476.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f476.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f477.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f477.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f478.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f478.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f479.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f479.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f480.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f480.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f481.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f481.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f482.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f482.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f483.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f483.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f484.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f484.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f485.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f485.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f486.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f486.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f487.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f487.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f488.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f488.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f489.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f489.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.quad.f490.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f490.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f491.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f491.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f492.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f492.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.quad.f493.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f493.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f494.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f494.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f495.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f495.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f496.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f496.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f497.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f497.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.quad.f498.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.quad.f498.bind.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@rec.dance.attempts\endcsname{12}
\expandafter\def\csname BAval@rec.dance.complete\endcsname{0}
\expandafter\def\csname BAval@rec.dance.fallwait\endcsname{10}
\expandafter\def\csname BAval@rec.dance.expired\endcsname{2}
\expandafter\def\csname BAval@rec.dance.requests\endcsname{0}
\expandafter\def\csname BAval@rec.dance.returns\endcsname{0}
\expandafter\def\csname BAval@rec.dance.initialpub\endcsname{1}
\expandafter\def\csname BAval@rec.dance.laterpub\endcsname{0}
\expandafter\def\csname BAval@rec.dance.nativeupdates\endcsname{0}
\expandafter\def\csname BAval@rec.dance.ticks\endcsname{180}
\expandafter\def\csname BAval@state.dance.dam.correct\endcsname{78}
\expandafter\def\csname BAval@state.dance.dam.wrong\endcsname{20}
\expandafter\def\csname BAval@state.dance.dam.unresolved\endcsname{82}
\expandafter\def\csname BAval@state.dance.dam.unknown\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f159.dam.iou\endcsname{0.99}
\expandafter\def\csname BAval@tick.dance.f159.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f160.dam.iou\endcsname{0.98}
\expandafter\def\csname BAval@tick.dance.f160.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f161.dam.iou\endcsname{0.97}
\expandafter\def\csname BAval@tick.dance.f161.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f162.dam.iou\endcsname{0.97}
\expandafter\def\csname BAval@tick.dance.f162.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f163.dam.iou\endcsname{0.95}
\expandafter\def\csname BAval@tick.dance.f163.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f164.dam.iou\endcsname{0.94}
\expandafter\def\csname BAval@tick.dance.f164.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f165.dam.iou\endcsname{0.92}
\expandafter\def\csname BAval@tick.dance.f165.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f166.dam.iou\endcsname{0.89}
\expandafter\def\csname BAval@tick.dance.f166.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f167.dam.iou\endcsname{0.87}
\expandafter\def\csname BAval@tick.dance.f167.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f168.dam.iou\endcsname{0.86}
\expandafter\def\csname BAval@tick.dance.f168.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f169.dam.iou\endcsname{0.83}
\expandafter\def\csname BAval@tick.dance.f169.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f170.dam.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f170.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f171.dam.iou\endcsname{0.52}
\expandafter\def\csname BAval@tick.dance.f171.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f172.dam.iou\endcsname{0.46}
\expandafter\def\csname BAval@tick.dance.f172.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f173.dam.iou\endcsname{0.51}
\expandafter\def\csname BAval@tick.dance.f173.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f174.dam.iou\endcsname{0.45}
\expandafter\def\csname BAval@tick.dance.f174.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f175.dam.iou\endcsname{0.44}
\expandafter\def\csname BAval@tick.dance.f175.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f176.dam.iou\endcsname{0.42}
\expandafter\def\csname BAval@tick.dance.f176.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f177.dam.iou\endcsname{0.42}
\expandafter\def\csname BAval@tick.dance.f177.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f178.dam.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f178.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f179.dam.iou\endcsname{0.39}
\expandafter\def\csname BAval@tick.dance.f179.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f180.dam.iou\endcsname{0.30}
\expandafter\def\csname BAval@tick.dance.f180.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f181.dam.iou\endcsname{0.27}
\expandafter\def\csname BAval@tick.dance.f181.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f182.dam.iou\endcsname{0.19}
\expandafter\def\csname BAval@tick.dance.f182.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f183.dam.iou\endcsname{0.14}
\expandafter\def\csname BAval@tick.dance.f183.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f184.dam.iou\endcsname{0.10}
\expandafter\def\csname BAval@tick.dance.f184.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f185.dam.iou\endcsname{0.08}
\expandafter\def\csname BAval@tick.dance.f185.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f186.dam.iou\endcsname{0.06}
\expandafter\def\csname BAval@tick.dance.f186.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f187.dam.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f187.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f188.dam.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f188.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f189.dam.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f189.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f190.dam.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f190.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f191.dam.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f191.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f192.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f192.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f193.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f193.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f194.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f194.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f195.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f195.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f196.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f196.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f197.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f197.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f198.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f198.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f199.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f199.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f200.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f200.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f201.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f201.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f202.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f202.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f203.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f203.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f204.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f204.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f205.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f205.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f206.dam.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f206.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f207.dam.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f207.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f208.dam.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f208.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f209.dam.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f209.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f210.dam.iou\endcsname{0.07}
\expandafter\def\csname BAval@tick.dance.f210.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f211.dam.iou\endcsname{0.09}
\expandafter\def\csname BAval@tick.dance.f211.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f212.dam.iou\endcsname{0.12}
\expandafter\def\csname BAval@tick.dance.f212.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f213.dam.iou\endcsname{0.13}
\expandafter\def\csname BAval@tick.dance.f213.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f214.dam.iou\endcsname{0.14}
\expandafter\def\csname BAval@tick.dance.f214.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f215.dam.iou\endcsname{0.15}
\expandafter\def\csname BAval@tick.dance.f215.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f216.dam.iou\endcsname{0.21}
\expandafter\def\csname BAval@tick.dance.f216.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f217.dam.iou\endcsname{0.24}
\expandafter\def\csname BAval@tick.dance.f217.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f218.dam.iou\endcsname{0.37}
\expandafter\def\csname BAval@tick.dance.f218.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f219.dam.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f219.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f220.dam.iou\endcsname{0.46}
\expandafter\def\csname BAval@tick.dance.f220.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f221.dam.iou\endcsname{0.51}
\expandafter\def\csname BAval@tick.dance.f221.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f222.dam.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f222.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f223.dam.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f223.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f224.dam.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f224.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f225.dam.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f225.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f226.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f226.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f227.dam.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f227.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f228.dam.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f228.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f229.dam.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f229.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f230.dam.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f230.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f231.dam.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f231.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f232.dam.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f232.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f233.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f233.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f234.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f234.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f235.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f235.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f236.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f236.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f237.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f237.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f238.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f238.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f239.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f239.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f240.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f240.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f241.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f241.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f242.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f242.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f243.dam.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f243.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f244.dam.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f244.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f245.dam.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f245.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f246.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f246.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f247.dam.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f247.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f248.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f248.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f249.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f249.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f250.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f250.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f251.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f251.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f252.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f252.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f253.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f253.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f254.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f254.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f255.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f255.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f256.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f256.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f257.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f257.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f258.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f258.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f259.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f259.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f260.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f260.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f261.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f261.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f262.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f262.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f263.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f263.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f264.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f264.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f265.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f265.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f266.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f266.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f267.dam.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f267.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f268.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f268.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f269.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f269.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f270.dam.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f270.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f271.dam.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f271.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f272.dam.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f272.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f273.dam.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f273.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f274.dam.iou\endcsname{0.61}
\expandafter\def\csname BAval@tick.dance.f274.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f275.dam.iou\endcsname{0.62}
\expandafter\def\csname BAval@tick.dance.f275.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f276.dam.iou\endcsname{0.61}
\expandafter\def\csname BAval@tick.dance.f276.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f277.dam.iou\endcsname{0.61}
\expandafter\def\csname BAval@tick.dance.f277.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f278.dam.iou\endcsname{0.61}
\expandafter\def\csname BAval@tick.dance.f278.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f279.dam.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f279.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f280.dam.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f280.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f281.dam.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f281.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f282.dam.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f282.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f283.dam.iou\endcsname{0.64}
\expandafter\def\csname BAval@tick.dance.f283.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f284.dam.iou\endcsname{0.61}
\expandafter\def\csname BAval@tick.dance.f284.dam.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f285.dam.iou\endcsname{0.47}
\expandafter\def\csname BAval@tick.dance.f285.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f286.dam.iou\endcsname{0.40}
\expandafter\def\csname BAval@tick.dance.f286.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f287.dam.iou\endcsname{0.30}
\expandafter\def\csname BAval@tick.dance.f287.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f288.dam.iou\endcsname{0.21}
\expandafter\def\csname BAval@tick.dance.f288.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f289.dam.iou\endcsname{0.15}
\expandafter\def\csname BAval@tick.dance.f289.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f290.dam.iou\endcsname{0.13}
\expandafter\def\csname BAval@tick.dance.f290.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f291.dam.iou\endcsname{0.05}
\expandafter\def\csname BAval@tick.dance.f291.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f292.dam.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f292.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f293.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f293.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f294.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f294.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f295.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f295.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f296.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f296.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f297.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f297.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f298.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f298.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f299.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f299.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f300.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f300.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f301.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f301.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f302.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f302.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f303.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f303.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f304.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f304.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f305.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f305.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f306.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f306.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f307.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f307.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f308.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f308.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f309.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f309.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f310.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f310.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f311.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f311.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f312.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f312.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f313.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f313.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f314.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f314.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f315.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f315.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f316.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f316.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f317.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f317.dam.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f318.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f318.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f319.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f319.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f320.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f320.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f321.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f321.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f322.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f322.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f323.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f323.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f324.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f324.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f325.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f325.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f326.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f326.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f327.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f327.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f328.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f328.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f329.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f329.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f330.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f330.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f331.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f331.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f332.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f332.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f333.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f333.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f334.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f334.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f335.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f335.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f336.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f336.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f337.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f337.dam.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f338.dam.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f338.dam.state\endcsname{U}
\expandafter\def\csname BAval@state.dance.keep.correct\endcsname{72}
\expandafter\def\csname BAval@state.dance.keep.wrong\endcsname{23}
\expandafter\def\csname BAval@state.dance.keep.unresolved\endcsname{84}
\expandafter\def\csname BAval@state.dance.keep.unknown\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f159.keep.iou\endcsname{0.99}
\expandafter\def\csname BAval@tick.dance.f159.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f160.keep.iou\endcsname{0.98}
\expandafter\def\csname BAval@tick.dance.f160.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f161.keep.iou\endcsname{0.97}
\expandafter\def\csname BAval@tick.dance.f161.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f162.keep.iou\endcsname{0.97}
\expandafter\def\csname BAval@tick.dance.f162.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f163.keep.iou\endcsname{0.95}
\expandafter\def\csname BAval@tick.dance.f163.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f164.keep.iou\endcsname{0.94}
\expandafter\def\csname BAval@tick.dance.f164.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f165.keep.iou\endcsname{0.92}
\expandafter\def\csname BAval@tick.dance.f165.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f166.keep.iou\endcsname{0.89}
\expandafter\def\csname BAval@tick.dance.f166.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f167.keep.iou\endcsname{0.87}
\expandafter\def\csname BAval@tick.dance.f167.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f168.keep.iou\endcsname{0.86}
\expandafter\def\csname BAval@tick.dance.f168.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f169.keep.iou\endcsname{0.83}
\expandafter\def\csname BAval@tick.dance.f169.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f170.keep.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f170.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f171.keep.iou\endcsname{0.52}
\expandafter\def\csname BAval@tick.dance.f171.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f172.keep.iou\endcsname{0.46}
\expandafter\def\csname BAval@tick.dance.f172.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f173.keep.iou\endcsname{0.51}
\expandafter\def\csname BAval@tick.dance.f173.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f174.keep.iou\endcsname{0.45}
\expandafter\def\csname BAval@tick.dance.f174.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f175.keep.iou\endcsname{0.44}
\expandafter\def\csname BAval@tick.dance.f175.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f176.keep.iou\endcsname{0.42}
\expandafter\def\csname BAval@tick.dance.f176.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f177.keep.iou\endcsname{0.42}
\expandafter\def\csname BAval@tick.dance.f177.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f178.keep.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f178.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f179.keep.iou\endcsname{0.39}
\expandafter\def\csname BAval@tick.dance.f179.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f180.keep.iou\endcsname{0.30}
\expandafter\def\csname BAval@tick.dance.f180.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f181.keep.iou\endcsname{0.27}
\expandafter\def\csname BAval@tick.dance.f181.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f182.keep.iou\endcsname{0.19}
\expandafter\def\csname BAval@tick.dance.f182.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f183.keep.iou\endcsname{0.14}
\expandafter\def\csname BAval@tick.dance.f183.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f184.keep.iou\endcsname{0.10}
\expandafter\def\csname BAval@tick.dance.f184.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f185.keep.iou\endcsname{0.08}
\expandafter\def\csname BAval@tick.dance.f185.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f186.keep.iou\endcsname{0.06}
\expandafter\def\csname BAval@tick.dance.f186.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f187.keep.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f187.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f188.keep.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f188.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f189.keep.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f189.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f190.keep.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f190.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f191.keep.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f191.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f192.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f192.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f193.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f193.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f194.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f194.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f195.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f195.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f196.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f196.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f197.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f197.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f198.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f198.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f199.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f199.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f200.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f200.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f201.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f201.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f202.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f202.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f203.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f203.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f204.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f204.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f205.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f205.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f206.keep.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f206.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f207.keep.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f207.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f208.keep.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f208.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f209.keep.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f209.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f210.keep.iou\endcsname{0.07}
\expandafter\def\csname BAval@tick.dance.f210.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f211.keep.iou\endcsname{0.09}
\expandafter\def\csname BAval@tick.dance.f211.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f212.keep.iou\endcsname{0.12}
\expandafter\def\csname BAval@tick.dance.f212.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f213.keep.iou\endcsname{0.13}
\expandafter\def\csname BAval@tick.dance.f213.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f214.keep.iou\endcsname{0.14}
\expandafter\def\csname BAval@tick.dance.f214.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f215.keep.iou\endcsname{0.15}
\expandafter\def\csname BAval@tick.dance.f215.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f216.keep.iou\endcsname{0.21}
\expandafter\def\csname BAval@tick.dance.f216.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f217.keep.iou\endcsname{0.24}
\expandafter\def\csname BAval@tick.dance.f217.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f218.keep.iou\endcsname{0.37}
\expandafter\def\csname BAval@tick.dance.f218.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f219.keep.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f219.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f220.keep.iou\endcsname{0.46}
\expandafter\def\csname BAval@tick.dance.f220.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f221.keep.iou\endcsname{0.51}
\expandafter\def\csname BAval@tick.dance.f221.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f222.keep.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f222.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f223.keep.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f223.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f224.keep.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f224.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f225.keep.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f225.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f226.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f226.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f227.keep.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f227.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f228.keep.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f228.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f229.keep.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f229.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f230.keep.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f230.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f231.keep.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f231.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f232.keep.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f232.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f233.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f233.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f234.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f234.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f235.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f235.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f236.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f236.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f237.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f237.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f238.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f238.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f239.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f239.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f240.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f240.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f241.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f241.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f242.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f242.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f243.keep.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f243.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f244.keep.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f244.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f245.keep.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f245.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f246.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f246.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f247.keep.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f247.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f248.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f248.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f249.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f249.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f250.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f250.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f251.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f251.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f252.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f252.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f253.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f253.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f254.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f254.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f255.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f255.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f256.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f256.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f257.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f257.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f258.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f258.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f259.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f259.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f260.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f260.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f261.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f261.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f262.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f262.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f263.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f263.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f264.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f264.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f265.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f265.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f266.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f266.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f267.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f267.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f268.keep.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f268.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f269.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f269.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f270.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f270.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f271.keep.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f271.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f272.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f272.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f273.keep.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f273.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f274.keep.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f274.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f275.keep.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f275.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f276.keep.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f276.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f277.keep.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f277.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f278.keep.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f278.keep.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f279.keep.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f279.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f280.keep.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f280.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f281.keep.iou\endcsname{0.43}
\expandafter\def\csname BAval@tick.dance.f281.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f282.keep.iou\endcsname{0.45}
\expandafter\def\csname BAval@tick.dance.f282.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f283.keep.iou\endcsname{0.50}
\expandafter\def\csname BAval@tick.dance.f283.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f284.keep.iou\endcsname{0.48}
\expandafter\def\csname BAval@tick.dance.f284.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f285.keep.iou\endcsname{0.37}
\expandafter\def\csname BAval@tick.dance.f285.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f286.keep.iou\endcsname{0.31}
\expandafter\def\csname BAval@tick.dance.f286.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f287.keep.iou\endcsname{0.22}
\expandafter\def\csname BAval@tick.dance.f287.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f288.keep.iou\endcsname{0.14}
\expandafter\def\csname BAval@tick.dance.f288.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f289.keep.iou\endcsname{0.09}
\expandafter\def\csname BAval@tick.dance.f289.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f290.keep.iou\endcsname{0.08}
\expandafter\def\csname BAval@tick.dance.f290.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f291.keep.iou\endcsname{0.01}
\expandafter\def\csname BAval@tick.dance.f291.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f292.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f292.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f293.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f293.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f294.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f294.keep.state\endcsname{UNKNOWN}
\expandafter\def\csname BAval@tick.dance.f295.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f295.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f296.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f296.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f297.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f297.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f298.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f298.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f299.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f299.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f300.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f300.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f301.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f301.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f302.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f302.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f303.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f303.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f304.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f304.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f305.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f305.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f306.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f306.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f307.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f307.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f308.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f308.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f309.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f309.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f310.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f310.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f311.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f311.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f312.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f312.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f313.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f313.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f314.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f314.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f315.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f315.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f316.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f316.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f317.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f317.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f318.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f318.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f319.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f319.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f320.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f320.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f321.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f321.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f322.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f322.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f323.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f323.keep.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f324.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f324.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f325.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f325.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f326.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f326.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f327.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f327.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f328.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f328.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f329.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f329.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f330.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f330.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f331.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f331.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f332.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f332.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f333.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f333.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f334.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f334.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f335.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f335.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f336.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f336.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f337.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f337.keep.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f338.keep.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f338.keep.state\endcsname{U}
\expandafter\def\csname BAval@state.dance.bind.correct\endcsname{78}
\expandafter\def\csname BAval@state.dance.bind.wrong\endcsname{23}
\expandafter\def\csname BAval@state.dance.bind.unresolved\endcsname{79}
\expandafter\def\csname BAval@state.dance.bind.unknown\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f159.bind.iou\endcsname{0.99}
\expandafter\def\csname BAval@tick.dance.f159.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f160.bind.iou\endcsname{0.98}
\expandafter\def\csname BAval@tick.dance.f160.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f161.bind.iou\endcsname{0.97}
\expandafter\def\csname BAval@tick.dance.f161.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f162.bind.iou\endcsname{0.97}
\expandafter\def\csname BAval@tick.dance.f162.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f163.bind.iou\endcsname{0.95}
\expandafter\def\csname BAval@tick.dance.f163.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f164.bind.iou\endcsname{0.94}
\expandafter\def\csname BAval@tick.dance.f164.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f165.bind.iou\endcsname{0.92}
\expandafter\def\csname BAval@tick.dance.f165.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f166.bind.iou\endcsname{0.89}
\expandafter\def\csname BAval@tick.dance.f166.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f167.bind.iou\endcsname{0.87}
\expandafter\def\csname BAval@tick.dance.f167.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f168.bind.iou\endcsname{0.86}
\expandafter\def\csname BAval@tick.dance.f168.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f169.bind.iou\endcsname{0.83}
\expandafter\def\csname BAval@tick.dance.f169.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f170.bind.iou\endcsname{0.61}
\expandafter\def\csname BAval@tick.dance.f170.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f171.bind.iou\endcsname{0.52}
\expandafter\def\csname BAval@tick.dance.f171.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f172.bind.iou\endcsname{0.46}
\expandafter\def\csname BAval@tick.dance.f172.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f173.bind.iou\endcsname{0.51}
\expandafter\def\csname BAval@tick.dance.f173.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f174.bind.iou\endcsname{0.45}
\expandafter\def\csname BAval@tick.dance.f174.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f175.bind.iou\endcsname{0.44}
\expandafter\def\csname BAval@tick.dance.f175.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f176.bind.iou\endcsname{0.42}
\expandafter\def\csname BAval@tick.dance.f176.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f177.bind.iou\endcsname{0.42}
\expandafter\def\csname BAval@tick.dance.f177.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f178.bind.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f178.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f179.bind.iou\endcsname{0.39}
\expandafter\def\csname BAval@tick.dance.f179.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f180.bind.iou\endcsname{0.29}
\expandafter\def\csname BAval@tick.dance.f180.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f181.bind.iou\endcsname{0.27}
\expandafter\def\csname BAval@tick.dance.f181.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f182.bind.iou\endcsname{0.19}
\expandafter\def\csname BAval@tick.dance.f182.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f183.bind.iou\endcsname{0.14}
\expandafter\def\csname BAval@tick.dance.f183.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f184.bind.iou\endcsname{0.10}
\expandafter\def\csname BAval@tick.dance.f184.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f185.bind.iou\endcsname{0.08}
\expandafter\def\csname BAval@tick.dance.f185.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f186.bind.iou\endcsname{0.06}
\expandafter\def\csname BAval@tick.dance.f186.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f187.bind.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f187.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f188.bind.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f188.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f189.bind.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f189.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f190.bind.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f190.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f191.bind.iou\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f191.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f192.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f192.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f193.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f193.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f194.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f194.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f195.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f195.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f196.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f196.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f197.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f197.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f198.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f198.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f199.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f199.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f200.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f200.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f201.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f201.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f202.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f202.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f203.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f203.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f204.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f204.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f205.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f205.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f206.bind.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f206.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f207.bind.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f207.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f208.bind.iou\endcsname{0.04}
\expandafter\def\csname BAval@tick.dance.f208.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f209.bind.iou\endcsname{0.05}
\expandafter\def\csname BAval@tick.dance.f209.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f210.bind.iou\endcsname{0.07}
\expandafter\def\csname BAval@tick.dance.f210.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f211.bind.iou\endcsname{0.09}
\expandafter\def\csname BAval@tick.dance.f211.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f212.bind.iou\endcsname{0.12}
\expandafter\def\csname BAval@tick.dance.f212.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f213.bind.iou\endcsname{0.13}
\expandafter\def\csname BAval@tick.dance.f213.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f214.bind.iou\endcsname{0.14}
\expandafter\def\csname BAval@tick.dance.f214.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f215.bind.iou\endcsname{0.15}
\expandafter\def\csname BAval@tick.dance.f215.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f216.bind.iou\endcsname{0.21}
\expandafter\def\csname BAval@tick.dance.f216.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f217.bind.iou\endcsname{0.24}
\expandafter\def\csname BAval@tick.dance.f217.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f218.bind.iou\endcsname{0.36}
\expandafter\def\csname BAval@tick.dance.f218.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f219.bind.iou\endcsname{0.41}
\expandafter\def\csname BAval@tick.dance.f219.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f220.bind.iou\endcsname{0.46}
\expandafter\def\csname BAval@tick.dance.f220.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f221.bind.iou\endcsname{0.51}
\expandafter\def\csname BAval@tick.dance.f221.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f222.bind.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f222.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f223.bind.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f223.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f224.bind.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f224.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f225.bind.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f225.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f226.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f226.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f227.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f227.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f228.bind.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f228.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f229.bind.iou\endcsname{0.53}
\expandafter\def\csname BAval@tick.dance.f229.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f230.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f230.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f231.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f231.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f232.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f232.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f233.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f233.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f234.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f234.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f235.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f235.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f236.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f236.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f237.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f237.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f238.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f238.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f239.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f239.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f240.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f240.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f241.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f241.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f242.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f242.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f243.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f243.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f244.bind.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f244.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f245.bind.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f245.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f246.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f246.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f247.bind.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f247.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f248.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f248.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f249.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f249.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f250.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f250.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f251.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f251.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f252.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f252.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f253.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f253.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f254.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f254.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f255.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f255.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f256.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f256.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f257.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f257.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f258.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f258.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f259.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f259.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f260.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f260.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f261.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f261.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f262.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f262.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f263.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f263.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f264.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f264.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f265.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f265.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f266.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f266.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f267.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f267.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f268.bind.iou\endcsname{0.55}
\expandafter\def\csname BAval@tick.dance.f268.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f269.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f269.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f270.bind.iou\endcsname{0.56}
\expandafter\def\csname BAval@tick.dance.f270.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f271.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f271.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f272.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f272.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f273.bind.iou\endcsname{0.58}
\expandafter\def\csname BAval@tick.dance.f273.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f274.bind.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f274.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f275.bind.iou\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f275.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f276.bind.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f276.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f277.bind.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f277.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f278.bind.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f278.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f279.bind.iou\endcsname{0.52}
\expandafter\def\csname BAval@tick.dance.f279.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f280.bind.iou\endcsname{0.52}
\expandafter\def\csname BAval@tick.dance.f280.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f281.bind.iou\endcsname{0.54}
\expandafter\def\csname BAval@tick.dance.f281.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f282.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@tick.dance.f282.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f283.bind.iou\endcsname{0.62}
\expandafter\def\csname BAval@tick.dance.f283.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f284.bind.iou\endcsname{0.59}
\expandafter\def\csname BAval@tick.dance.f284.bind.state\endcsname{C}
\expandafter\def\csname BAval@tick.dance.f285.bind.iou\endcsname{0.46}
\expandafter\def\csname BAval@tick.dance.f285.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f286.bind.iou\endcsname{0.40}
\expandafter\def\csname BAval@tick.dance.f286.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f287.bind.iou\endcsname{0.29}
\expandafter\def\csname BAval@tick.dance.f287.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f288.bind.iou\endcsname{0.20}
\expandafter\def\csname BAval@tick.dance.f288.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f289.bind.iou\endcsname{0.15}
\expandafter\def\csname BAval@tick.dance.f289.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f290.bind.iou\endcsname{0.13}
\expandafter\def\csname BAval@tick.dance.f290.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f291.bind.iou\endcsname{0.05}
\expandafter\def\csname BAval@tick.dance.f291.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f292.bind.iou\endcsname{0.03}
\expandafter\def\csname BAval@tick.dance.f292.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f293.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f293.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f294.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f294.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f295.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f295.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f296.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f296.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f297.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f297.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f298.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f298.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f299.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f299.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f300.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f300.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f301.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f301.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f302.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f302.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f303.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f303.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f304.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f304.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f305.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f305.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f306.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f306.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f307.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f307.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f308.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f308.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f309.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f309.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f310.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f310.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f311.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f311.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f312.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f312.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f313.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f313.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f314.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f314.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f315.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f315.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f316.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f316.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f317.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f317.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f318.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f318.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f319.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f319.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f320.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f320.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f321.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f321.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f322.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f322.bind.state\endcsname{W}
\expandafter\def\csname BAval@tick.dance.f323.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f323.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f324.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f324.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f325.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f325.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f326.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f326.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f327.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f327.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f328.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f328.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f329.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f329.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f330.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f330.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f331.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f331.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f332.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f332.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f333.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f333.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f334.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f334.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f335.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f335.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f336.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f336.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f337.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f337.bind.state\endcsname{U}
\expandafter\def\csname BAval@tick.dance.f338.bind.iou\endcsname{0.00}
\expandafter\def\csname BAval@tick.dance.f338.bind.state\endcsname{U}
\expandafter\def\csname BAval@pair.quad.dam.joint\endcsname{72}
\expandafter\def\csname BAval@pair.quad.dam.agree\endcsname{68}
\expandafter\def\csname BAval@pair.quad.dam.other\endcsname{4}
\expandafter\def\csname BAval@pair.quad.dam.unknown\endcsname{18}
\expandafter\def\csname BAval@pair.quad.dam.C.C\endcsname{1}
\expandafter\def\csname BAval@pair.quad.dam.C.W\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.C.U\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.C.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.W.C\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.W.W\endcsname{9}
\expandafter\def\csname BAval@pair.quad.dam.W.U\endcsname{3}
\expandafter\def\csname BAval@pair.quad.dam.W.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.U.C\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.U.W\endcsname{1}
\expandafter\def\csname BAval@pair.quad.dam.U.U\endcsname{58}
\expandafter\def\csname BAval@pair.quad.dam.U.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.UNKNOWN.C\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.UNKNOWN.W\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.UNKNOWN.U\endcsname{0}
\expandafter\def\csname BAval@pair.quad.dam.UNKNOWN.UNKNOWN\endcsname{18}
\expandafter\def\csname BAval@pair.quad.keep.joint\endcsname{72}
\expandafter\def\csname BAval@pair.quad.keep.agree\endcsname{72}
\expandafter\def\csname BAval@pair.quad.keep.other\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.unknown\endcsname{18}
\expandafter\def\csname BAval@pair.quad.keep.C.C\endcsname{1}
\expandafter\def\csname BAval@pair.quad.keep.C.W\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.C.U\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.C.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.W.C\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.W.W\endcsname{12}
\expandafter\def\csname BAval@pair.quad.keep.W.U\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.W.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.U.C\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.U.W\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.U.U\endcsname{59}
\expandafter\def\csname BAval@pair.quad.keep.U.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.UNKNOWN.C\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.UNKNOWN.W\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.UNKNOWN.U\endcsname{0}
\expandafter\def\csname BAval@pair.quad.keep.UNKNOWN.UNKNOWN\endcsname{18}
\expandafter\def\csname BAval@pair.dance.dam.joint\endcsname{180}
\expandafter\def\csname BAval@pair.dance.dam.agree\endcsname{177}
\expandafter\def\csname BAval@pair.dance.dam.other\endcsname{3}
\expandafter\def\csname BAval@pair.dance.dam.unknown\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.C.C\endcsname{78}
\expandafter\def\csname BAval@pair.dance.dam.C.W\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.C.U\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.C.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.W.C\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.W.W\endcsname{20}
\expandafter\def\csname BAval@pair.dance.dam.W.U\endcsname{3}
\expandafter\def\csname BAval@pair.dance.dam.W.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.U.C\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.U.W\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.U.U\endcsname{79}
\expandafter\def\csname BAval@pair.dance.dam.U.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.UNKNOWN.C\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.UNKNOWN.W\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.UNKNOWN.U\endcsname{0}
\expandafter\def\csname BAval@pair.dance.dam.UNKNOWN.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.joint\endcsname{179}
\expandafter\def\csname BAval@pair.dance.keep.agree\endcsname{170}
\expandafter\def\csname BAval@pair.dance.keep.other\endcsname{9}
\expandafter\def\csname BAval@pair.dance.keep.unknown\endcsname{1}
\expandafter\def\csname BAval@pair.dance.keep.C.C\endcsname{72}
\expandafter\def\csname BAval@pair.dance.keep.C.W\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.C.U\endcsname{6}
\expandafter\def\csname BAval@pair.dance.keep.C.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.W.C\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.W.W\endcsname{21}
\expandafter\def\csname BAval@pair.dance.keep.W.U\endcsname{1}
\expandafter\def\csname BAval@pair.dance.keep.W.UNKNOWN\endcsname{1}
\expandafter\def\csname BAval@pair.dance.keep.U.C\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.U.W\endcsname{2}
\expandafter\def\csname BAval@pair.dance.keep.U.U\endcsname{77}
\expandafter\def\csname BAval@pair.dance.keep.U.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.UNKNOWN.C\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.UNKNOWN.W\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.UNKNOWN.U\endcsname{0}
\expandafter\def\csname BAval@pair.dance.keep.UNKNOWN.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dam.joint\endcsname{252}
\expandafter\def\csname BAval@pair.dam.agree\endcsname{245}
\expandafter\def\csname BAval@pair.dam.other\endcsname{7}
\expandafter\def\csname BAval@pair.dam.unknown\endcsname{18}
\expandafter\def\csname BAval@pair.dam.C.C\endcsname{79}
\expandafter\def\csname BAval@pair.dam.C.W\endcsname{0}
\expandafter\def\csname BAval@pair.dam.C.U\endcsname{0}
\expandafter\def\csname BAval@pair.dam.C.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dam.W.C\endcsname{0}
\expandafter\def\csname BAval@pair.dam.W.W\endcsname{29}
\expandafter\def\csname BAval@pair.dam.W.U\endcsname{6}
\expandafter\def\csname BAval@pair.dam.W.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dam.U.C\endcsname{0}
\expandafter\def\csname BAval@pair.dam.U.W\endcsname{1}
\expandafter\def\csname BAval@pair.dam.U.U\endcsname{137}
\expandafter\def\csname BAval@pair.dam.U.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.dam.UNKNOWN.C\endcsname{0}
\expandafter\def\csname BAval@pair.dam.UNKNOWN.W\endcsname{0}
\expandafter\def\csname BAval@pair.dam.UNKNOWN.U\endcsname{0}
\expandafter\def\csname BAval@pair.dam.UNKNOWN.UNKNOWN\endcsname{18}
\expandafter\def\csname BAval@pair.keep.joint\endcsname{251}
\expandafter\def\csname BAval@pair.keep.agree\endcsname{242}
\expandafter\def\csname BAval@pair.keep.other\endcsname{9}
\expandafter\def\csname BAval@pair.keep.unknown\endcsname{19}
\expandafter\def\csname BAval@pair.keep.C.C\endcsname{73}
\expandafter\def\csname BAval@pair.keep.C.W\endcsname{0}
\expandafter\def\csname BAval@pair.keep.C.U\endcsname{6}
\expandafter\def\csname BAval@pair.keep.C.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.keep.W.C\endcsname{0}
\expandafter\def\csname BAval@pair.keep.W.W\endcsname{33}
\expandafter\def\csname BAval@pair.keep.W.U\endcsname{1}
\expandafter\def\csname BAval@pair.keep.W.UNKNOWN\endcsname{1}
\expandafter\def\csname BAval@pair.keep.U.C\endcsname{0}
\expandafter\def\csname BAval@pair.keep.U.W\endcsname{2}
\expandafter\def\csname BAval@pair.keep.U.U\endcsname{136}
\expandafter\def\csname BAval@pair.keep.U.UNKNOWN\endcsname{0}
\expandafter\def\csname BAval@pair.keep.UNKNOWN.C\endcsname{0}
\expandafter\def\csname BAval@pair.keep.UNKNOWN.W\endcsname{0}
\expandafter\def\csname BAval@pair.keep.UNKNOWN.U\endcsname{0}
\expandafter\def\csname BAval@pair.keep.UNKNOWN.UNKNOWN\endcsname{18}
\expandafter\def\csname BAval@rec.six.frames\endcsname{6}
\expandafter\def\csname BAval@rec.six.seconds\endcsname{0.30}
\expandafter\def\csname BAval@rec.six.start\endcsname{279}
\expandafter\def\csname BAval@rec.six.end\endcsname{284}
\expandafter\def\csname BAval@rec.six.anchor\endcsname{282}
\expandafter\def\csname BAval@rec.frame282.dam.iou\endcsname{0.59}
\expandafter\def\csname BAval@rec.frame282.keep.iou\endcsname{0.45}
\expandafter\def\csname BAval@rec.frame282.bind.iou\endcsname{0.57}
\expandafter\def\csname BAval@case.B.f120.frame\endcsname{120}
\expandafter\def\csname BAval@case.B.f120.kcf\endcsname{0.86}
\expandafter\def\csname BAval@case.B.f120.csrt\endcsname{0.66}
\expandafter\def\csname BAval@case.B.f140.frame\endcsname{140}
\expandafter\def\csname BAval@case.B.f140.kcf\endcsname{0.73}
\expandafter\def\csname BAval@case.B.f140.csrt\endcsname{0.62}
\expandafter\def\csname BAval@case.B.kcf.returned\endcsname{40}
\expandafter\def\csname BAval@case.B.kcf.evaluated.steps\endcsname{40}
\expandafter\def\csname BAval@case.B.kcf.mean\endcsname{0.877}
\expandafter\def\csname BAval@case.B.kcf.successes.iou50\endcsname{40}
\expandafter\def\csname BAval@case.B.csrt.returned\endcsname{40}
\expandafter\def\csname BAval@case.B.csrt.evaluated.steps\endcsname{40}
\expandafter\def\csname BAval@case.B.csrt.mean\endcsname{0.716}
\expandafter\def\csname BAval@case.B.csrt.successes.iou50\endcsname{40}
\expandafter\def\csname BAval@case.D.f272.frame\endcsname{272}
\expandafter\def\csname BAval@case.D.f272.kcf\endcsname{0.38}
\expandafter\def\csname BAval@case.D.f272.csrt\endcsname{0.43}
\expandafter\def\csname BAval@case.D.f300.frame\endcsname{300}
\expandafter\def\csname BAval@case.D.f300.kcf\endcsname{Lost}
\expandafter\def\csname BAval@case.D.f300.csrt\endcsname{0.57}
\expandafter\def\csname BAval@case.D.kcf.returned\endcsname{39}
\expandafter\def\csname BAval@case.D.kcf.evaluated.steps\endcsname{60}
\expandafter\def\csname BAval@case.D.csrt.returned\endcsname{60}
\expandafter\def\csname BAval@case.D.csrt.evaluated.steps\endcsname{60}
\expandafter\def\csname BAval@plan.strata.short.episodes\endcsname{120}
\expandafter\def\csname BAval@plan.strata.short.weight\endcsname{0.250}
\expandafter\def\csname BAval@plan.strata.similar.episodes\endcsname{180}
\expandafter\def\csname BAval@plan.strata.similar.weight\endcsname{0.375}
\expandafter\def\csname BAval@plan.strata.long.episodes\endcsname{180}
\expandafter\def\csname BAval@plan.strata.long.weight\endcsname{0.375}
\expandafter\def\csname BAval@plan.train.groups\endcsname{60}
\expandafter\def\csname BAval@plan.train.episodes\endcsname{1200}
\expandafter\def\csname BAval@plan.validation.groups\endcsname{20}
\expandafter\def\csname BAval@plan.validation.episodes\endcsname{200}
\expandafter\def\csname BAval@plan.test.groups\endcsname{40}
\expandafter\def\csname BAval@plan.test.episodes\endcsname{480}
\expandafter\def\csname BAval@t17.r01.axis\endcsname{0}
\expandafter\def\csname BAval@t17.r02.axis\endcsname{0.1}
\expandafter\def\csname BAval@t17.r03.axis\endcsname{0.25}
\expandafter\def\csname BAval@t17.r04.axis\endcsname{0.5}
\expandafter\def\csname BAval@t17.r05.axis\endcsname{1}
\expandafter\def\csname BAval@t17.r06.axis\endcsname{2}
\expandafter\def\csname BAval@t17.r07.axis\endcsname{0.5}
\expandafter\def\csname BAval@t17.r08.axis\endcsname{0.75}
\expandafter\def\csname BAval@t17.r09.axis\endcsname{1}
\expandafter\def\csname BAval@t17.r10.axis\endcsname{1.25}
\expandafter\def\csname BAval@t17.r11.axis\endcsname{1.5}
\expandafter\def\csname BAval@t17.r12.axis\endcsname{2}
\expandafter\def\csname BAval@t05.r01.axis\endcsname{0}
\expandafter\def\csname BAval@t05.r02.axis\endcsname{0.1}
\expandafter\def\csname BAval@t05.r03.axis\endcsname{0.25}
\expandafter\def\csname BAval@t05.r04.axis\endcsname{0.5}
\expandafter\def\csname BAval@t05.r05.axis\endcsname{1.0}
\expandafter\def\csname BAval@t05.r06.axis\endcsname{2.0}
\expandafter\def\csname BAval@t06.r01.axis\endcsname{0.5}
\expandafter\def\csname BAval@t06.r02.axis\endcsname{0.75}
\expandafter\def\csname BAval@t06.r03.axis\endcsname{1.0}
\expandafter\def\csname BAval@t06.r04.axis\endcsname{1.25}
\expandafter\def\csname BAval@t06.r05.axis\endcsname{1.5}
\expandafter\def\csname BAval@t06.r06.axis\endcsname{2.0}
\expandafter\def\csname BAval@t20.r01.axis\endcsname{0.0}
\expandafter\def\csname BAval@t20.r02.axis\endcsname{0.02}
\expandafter\def\csname BAval@t20.r03.axis\endcsname{0.04}
\expandafter\def\csname BAval@t20.r04.axis\endcsname{0.06}
\expandafter\def\csname BAval@t20.r05.axis\endcsname{0.08}
\expandafter\def\csname BAval@t20.r06.axis\endcsname{0.1}
\expandafter\def\csname BAval@t20.r07.axis\endcsname{0.12}
\expandafter\def\csname BAval@t20.r08.axis\endcsname{0.14}
\expandafter\def\csname BAval@t20.r09.axis\endcsname{0.16}
\expandafter\def\csname BAval@t20.r10.axis\endcsname{0.18}
\expandafter\def\csname BAval@t20.r11.axis\endcsname{0.2}
\expandafter\def\csname BAval@t20.r12.axis\endcsname{0.22}
\expandafter\def\csname BAval@t20.r13.axis\endcsname{0.24}
\expandafter\def\csname BAval@t20.r14.axis\endcsname{0.26}
\expandafter\def\csname BAval@t20.r15.axis\endcsname{0.28}
\expandafter\def\csname BAval@t20.r16.axis\endcsname{0.3}
\expandafter\def\csname BAval@t20.r17.axis\endcsname{0.32}
\expandafter\def\csname BAval@t20.r18.axis\endcsname{0.34}
\expandafter\def\csname BAval@t20.r19.axis\endcsname{0.36}
\expandafter\def\csname BAval@t20.r20.axis\endcsname{0.38}
\expandafter\def\csname BAval@t20.r21.axis\endcsname{0.4}
\expandafter\def\csname BAval@t20.r22.axis\endcsname{0.42}
\expandafter\def\csname BAval@t20.r23.axis\endcsname{0.44}
\expandafter\def\csname BAval@t20.r24.axis\endcsname{0.46}
\expandafter\def\csname BAval@t20.r25.axis\endcsname{0.48}
\expandafter\def\csname BAval@t20.r26.axis\endcsname{0.5}
\expandafter\def\csname BAval@t20.r27.axis\endcsname{0.52}
\expandafter\def\csname BAval@t20.r28.axis\endcsname{0.54}
\expandafter\def\csname BAval@t20.r29.axis\endcsname{0.56}
\expandafter\def\csname BAval@t20.r30.axis\endcsname{0.58}
\expandafter\def\csname BAval@t20.r31.axis\endcsname{0.6}
\expandafter\def\csname BAval@t20.r32.axis\endcsname{0.62}
\expandafter\def\csname BAval@t20.r33.axis\endcsname{0.64}
\expandafter\def\csname BAval@t20.r34.axis\endcsname{0.66}
\expandafter\def\csname BAval@t20.r35.axis\endcsname{0.68}
\expandafter\def\csname BAval@t20.r36.axis\endcsname{0.7}
\expandafter\def\csname BAval@t20.r37.axis\endcsname{0.72}
\expandafter\def\csname BAval@t20.r38.axis\endcsname{0.74}
\expandafter\def\csname BAval@t20.r39.axis\endcsname{0.76}
\expandafter\def\csname BAval@t20.r40.axis\endcsname{0.78}
\expandafter\def\csname BAval@t20.r41.axis\endcsname{0.8}
\expandafter\def\csname BAval@t20.r42.axis\endcsname{0.82}
\expandafter\def\csname BAval@t20.r43.axis\endcsname{0.84}
\expandafter\def\csname BAval@t20.r44.axis\endcsname{0.86}
\expandafter\def\csname BAval@t20.r45.axis\endcsname{0.88}
\expandafter\def\csname BAval@t20.r46.axis\endcsname{0.9}
\expandafter\def\csname BAval@t20.r47.axis\endcsname{0.92}
\expandafter\def\csname BAval@t20.r48.axis\endcsname{0.94}
\expandafter\def\csname BAval@t20.r49.axis\endcsname{0.96}
\expandafter\def\csname BAval@t20.r50.axis\endcsname{0.98}
\expandafter\def\csname BAval@t20.r51.axis\endcsname{1.0}
\expandafter\def\csname BAval@t20.r52.axis\endcsname{0.0}
\expandafter\def\csname BAval@t20.r53.axis\endcsname{0.02}
\expandafter\def\csname BAval@t20.r54.axis\endcsname{0.04}
\expandafter\def\csname BAval@t20.r55.axis\endcsname{0.06}
\expandafter\def\csname BAval@t20.r56.axis\endcsname{0.08}
\expandafter\def\csname BAval@t20.r57.axis\endcsname{0.1}
\expandafter\def\csname BAval@t20.r58.axis\endcsname{0.12}
\expandafter\def\csname BAval@t20.r59.axis\endcsname{0.14}
\expandafter\def\csname BAval@t20.r60.axis\endcsname{0.16}
\expandafter\def\csname BAval@t20.r61.axis\endcsname{0.18}
\expandafter\def\csname BAval@t20.r62.axis\endcsname{0.2}
\expandafter\def\csname BAval@t20.r63.axis\endcsname{0.22}
\expandafter\def\csname BAval@t20.r64.axis\endcsname{0.24}
\expandafter\def\csname BAval@t20.r65.axis\endcsname{0.26}
\expandafter\def\csname BAval@t20.r66.axis\endcsname{0.28}
\expandafter\def\csname BAval@t20.r67.axis\endcsname{0.3}
\expandafter\def\csname BAval@t20.r68.axis\endcsname{0.32}
\expandafter\def\csname BAval@t20.r69.axis\endcsname{0.34}
\expandafter\def\csname BAval@t20.r70.axis\endcsname{0.36}
\expandafter\def\csname BAval@t20.r71.axis\endcsname{0.38}
\expandafter\def\csname BAval@t20.r72.axis\endcsname{0.4}
\expandafter\def\csname BAval@t20.r73.axis\endcsname{0.42}
\expandafter\def\csname BAval@t20.r74.axis\endcsname{0.44}
\expandafter\def\csname BAval@t20.r75.axis\endcsname{0.46}
\expandafter\def\csname BAval@t20.r76.axis\endcsname{0.48}
\expandafter\def\csname BAval@t20.r77.axis\endcsname{0.5}
\expandafter\def\csname BAval@t20.r78.axis\endcsname{0.52}
\expandafter\def\csname BAval@t20.r79.axis\endcsname{0.54}
\expandafter\def\csname BAval@t20.r80.axis\endcsname{0.56}
\expandafter\def\csname BAval@t20.r81.axis\endcsname{0.58}
\expandafter\def\csname BAval@t20.r82.axis\endcsname{0.6}
\expandafter\def\csname BAval@t20.r83.axis\endcsname{0.62}
\expandafter\def\csname BAval@t20.r84.axis\endcsname{0.64}
\expandafter\def\csname BAval@t20.r85.axis\endcsname{0.66}
\expandafter\def\csname BAval@t20.r86.axis\endcsname{0.68}
\expandafter\def\csname BAval@t20.r87.axis\endcsname{0.7}
\expandafter\def\csname BAval@t20.r88.axis\endcsname{0.72}
\expandafter\def\csname BAval@t20.r89.axis\endcsname{0.74}
\expandafter\def\csname BAval@t20.r90.axis\endcsname{0.76}
\expandafter\def\csname BAval@t20.r91.axis\endcsname{0.78}
\expandafter\def\csname BAval@t20.r92.axis\endcsname{0.8}
\expandafter\def\csname BAval@t20.r93.axis\endcsname{0.82}
\expandafter\def\csname BAval@t20.r94.axis\endcsname{0.84}
\expandafter\def\csname BAval@t20.r95.axis\endcsname{0.86}
\expandafter\def\csname BAval@t20.r96.axis\endcsname{0.88}
\expandafter\def\csname BAval@t20.r97.axis\endcsname{0.9}
\expandafter\def\csname BAval@t20.r98.axis\endcsname{0.92}
\expandafter\def\csname BAval@t20.r99.axis\endcsname{0.94}
\expandafter\def\csname BAval@t20.r100.axis\endcsname{0.96}
\expandafter\def\csname BAval@t20.r101.axis\endcsname{0.98}
\expandafter\def\csname BAval@t20.r102.axis\endcsname{1.0}
\expandafter\def\csname BAval@t20.r103.axis\endcsname{0.0}
\expandafter\def\csname BAval@t20.r104.axis\endcsname{0.02}
\expandafter\def\csname BAval@t20.r105.axis\endcsname{0.04}
\expandafter\def\csname BAval@t20.r106.axis\endcsname{0.06}
\expandafter\def\csname BAval@t20.r107.axis\endcsname{0.08}
\expandafter\def\csname BAval@t20.r108.axis\endcsname{0.1}
\expandafter\def\csname BAval@t20.r109.axis\endcsname{0.12}
\expandafter\def\csname BAval@t20.r110.axis\endcsname{0.14}
\expandafter\def\csname BAval@t20.r111.axis\endcsname{0.16}
\expandafter\def\csname BAval@t20.r112.axis\endcsname{0.18}
\expandafter\def\csname BAval@t20.r113.axis\endcsname{0.2}
\expandafter\def\csname BAval@t20.r114.axis\endcsname{0.22}
\expandafter\def\csname BAval@t20.r115.axis\endcsname{0.24}
\expandafter\def\csname BAval@t20.r116.axis\endcsname{0.26}
\expandafter\def\csname BAval@t20.r117.axis\endcsname{0.28}
\expandafter\def\csname BAval@t20.r118.axis\endcsname{0.3}
\expandafter\def\csname BAval@t20.r119.axis\endcsname{0.32}
\expandafter\def\csname BAval@t20.r120.axis\endcsname{0.34}
\expandafter\def\csname BAval@t20.r121.axis\endcsname{0.36}
\expandafter\def\csname BAval@t20.r122.axis\endcsname{0.38}
\expandafter\def\csname BAval@t20.r123.axis\endcsname{0.4}
\expandafter\def\csname BAval@t20.r124.axis\endcsname{0.42}
\expandafter\def\csname BAval@t20.r125.axis\endcsname{0.44}
\expandafter\def\csname BAval@t20.r126.axis\endcsname{0.46}
\expandafter\def\csname BAval@t20.r127.axis\endcsname{0.48}
\expandafter\def\csname BAval@t20.r128.axis\endcsname{0.5}
\expandafter\def\csname BAval@t20.r129.axis\endcsname{0.52}
\expandafter\def\csname BAval@t20.r130.axis\endcsname{0.54}
\expandafter\def\csname BAval@t20.r131.axis\endcsname{0.56}
\expandafter\def\csname BAval@t20.r132.axis\endcsname{0.58}
\expandafter\def\csname BAval@t20.r133.axis\endcsname{0.6}
\expandafter\def\csname BAval@t20.r134.axis\endcsname{0.62}
\expandafter\def\csname BAval@t20.r135.axis\endcsname{0.64}
\expandafter\def\csname BAval@t20.r136.axis\endcsname{0.66}
\expandafter\def\csname BAval@t20.r137.axis\endcsname{0.68}
\expandafter\def\csname BAval@t20.r138.axis\endcsname{0.7}
\expandafter\def\csname BAval@t20.r139.axis\endcsname{0.72}
\expandafter\def\csname BAval@t20.r140.axis\endcsname{0.74}
\expandafter\def\csname BAval@t20.r141.axis\endcsname{0.76}
\expandafter\def\csname BAval@t20.r142.axis\endcsname{0.78}
\expandafter\def\csname BAval@t20.r143.axis\endcsname{0.8}
\expandafter\def\csname BAval@t20.r144.axis\endcsname{0.82}
\expandafter\def\csname BAval@t20.r145.axis\endcsname{0.84}
\expandafter\def\csname BAval@t20.r146.axis\endcsname{0.86}
\expandafter\def\csname BAval@t20.r147.axis\endcsname{0.88}
\expandafter\def\csname BAval@t20.r148.axis\endcsname{0.9}
\expandafter\def\csname BAval@t20.r149.axis\endcsname{0.92}
\expandafter\def\csname BAval@t20.r150.axis\endcsname{0.94}
\expandafter\def\csname BAval@t20.r151.axis\endcsname{0.96}
\expandafter\def\csname BAval@t20.r152.axis\endcsname{0.98}
\expandafter\def\csname BAval@t20.r153.axis\endcsname{1.0}
\expandafter\def\csname BAval@t20.r154.axis\endcsname{0.0}
\expandafter\def\csname BAval@t20.r155.axis\endcsname{0.02}
\expandafter\def\csname BAval@t20.r156.axis\endcsname{0.04}
\expandafter\def\csname BAval@t20.r157.axis\endcsname{0.06}
\expandafter\def\csname BAval@t20.r158.axis\endcsname{0.08}
\expandafter\def\csname BAval@t20.r159.axis\endcsname{0.1}
\expandafter\def\csname BAval@t20.r160.axis\endcsname{0.12}
\expandafter\def\csname BAval@t20.r161.axis\endcsname{0.14}
\expandafter\def\csname BAval@t20.r162.axis\endcsname{0.16}
\expandafter\def\csname BAval@t20.r163.axis\endcsname{0.18}
\expandafter\def\csname BAval@t20.r164.axis\endcsname{0.2}
\expandafter\def\csname BAval@t20.r165.axis\endcsname{0.22}
\expandafter\def\csname BAval@t20.r166.axis\endcsname{0.24}
\expandafter\def\csname BAval@t20.r167.axis\endcsname{0.26}
\expandafter\def\csname BAval@t20.r168.axis\endcsname{0.28}
\expandafter\def\csname BAval@t20.r169.axis\endcsname{0.3}
\expandafter\def\csname BAval@t20.r170.axis\endcsname{0.32}
\expandafter\def\csname BAval@t20.r171.axis\endcsname{0.34}
\expandafter\def\csname BAval@t20.r172.axis\endcsname{0.36}
\expandafter\def\csname BAval@t20.r173.axis\endcsname{0.38}
\expandafter\def\csname BAval@t20.r174.axis\endcsname{0.4}
\expandafter\def\csname BAval@t20.r175.axis\endcsname{0.42}
\expandafter\def\csname BAval@t20.r176.axis\endcsname{0.44}
\expandafter\def\csname BAval@t20.r177.axis\endcsname{0.46}
\expandafter\def\csname BAval@t20.r178.axis\endcsname{0.48}
\expandafter\def\csname BAval@t20.r179.axis\endcsname{0.5}
\expandafter\def\csname BAval@t20.r180.axis\endcsname{0.52}
\expandafter\def\csname BAval@t20.r181.axis\endcsname{0.54}
\expandafter\def\csname BAval@t20.r182.axis\endcsname{0.56}
\expandafter\def\csname BAval@t20.r183.axis\endcsname{0.58}
\expandafter\def\csname BAval@t20.r184.axis\endcsname{0.6}
\expandafter\def\csname BAval@t20.r185.axis\endcsname{0.62}
\expandafter\def\csname BAval@t20.r186.axis\endcsname{0.64}
\expandafter\def\csname BAval@t20.r187.axis\endcsname{0.66}
\expandafter\def\csname BAval@t20.r188.axis\endcsname{0.68}
\expandafter\def\csname BAval@t20.r189.axis\endcsname{0.7}
\expandafter\def\csname BAval@t20.r190.axis\endcsname{0.72}
\expandafter\def\csname BAval@t20.r191.axis\endcsname{0.74}
\expandafter\def\csname BAval@t20.r192.axis\endcsname{0.76}
\expandafter\def\csname BAval@t20.r193.axis\endcsname{0.78}
\expandafter\def\csname BAval@t20.r194.axis\endcsname{0.8}
\expandafter\def\csname BAval@t20.r195.axis\endcsname{0.82}
\expandafter\def\csname BAval@t20.r196.axis\endcsname{0.84}
\expandafter\def\csname BAval@t20.r197.axis\endcsname{0.86}
\expandafter\def\csname BAval@t20.r198.axis\endcsname{0.88}
\expandafter\def\csname BAval@t20.r199.axis\endcsname{0.9}
\expandafter\def\csname BAval@t20.r200.axis\endcsname{0.92}
\expandafter\def\csname BAval@t20.r201.axis\endcsname{0.94}
\expandafter\def\csname BAval@t20.r202.axis\endcsname{0.96}
\expandafter\def\csname BAval@t20.r203.axis\endcsname{0.98}
\expandafter\def\csname BAval@t20.r204.axis\endcsname{1.0}
\expandafter\def\csname BAval@t20.r205.axis\endcsname{0.0}
\expandafter\def\csname BAval@t20.r206.axis\endcsname{0.02}
\expandafter\def\csname BAval@t20.r207.axis\endcsname{0.04}
\expandafter\def\csname BAval@t20.r208.axis\endcsname{0.06}
\expandafter\def\csname BAval@t20.r209.axis\endcsname{0.08}
\expandafter\def\csname BAval@t20.r210.axis\endcsname{0.1}
\expandafter\def\csname BAval@t20.r211.axis\endcsname{0.12}
\expandafter\def\csname BAval@t20.r212.axis\endcsname{0.14}
\expandafter\def\csname BAval@t20.r213.axis\endcsname{0.16}
\expandafter\def\csname BAval@t20.r214.axis\endcsname{0.18}
\expandafter\def\csname BAval@t20.r215.axis\endcsname{0.2}
\expandafter\def\csname BAval@t20.r216.axis\endcsname{0.22}
\expandafter\def\csname BAval@t20.r217.axis\endcsname{0.24}
\expandafter\def\csname BAval@t20.r218.axis\endcsname{0.26}
\expandafter\def\csname BAval@t20.r219.axis\endcsname{0.28}
\expandafter\def\csname BAval@t20.r220.axis\endcsname{0.3}
\expandafter\def\csname BAval@t20.r221.axis\endcsname{0.32}
\expandafter\def\csname BAval@t20.r222.axis\endcsname{0.34}
\expandafter\def\csname BAval@t20.r223.axis\endcsname{0.36}
\expandafter\def\csname BAval@t20.r224.axis\endcsname{0.38}
\expandafter\def\csname BAval@t20.r225.axis\endcsname{0.4}
\expandafter\def\csname BAval@t20.r226.axis\endcsname{0.42}
\expandafter\def\csname BAval@t20.r227.axis\endcsname{0.44}
\expandafter\def\csname BAval@t20.r228.axis\endcsname{0.46}
\expandafter\def\csname BAval@t20.r229.axis\endcsname{0.48}
\expandafter\def\csname BAval@t20.r230.axis\endcsname{0.5}
\expandafter\def\csname BAval@t20.r231.axis\endcsname{0.52}
\expandafter\def\csname BAval@t20.r232.axis\endcsname{0.54}
\expandafter\def\csname BAval@t20.r233.axis\endcsname{0.56}
\expandafter\def\csname BAval@t20.r234.axis\endcsname{0.58}
\expandafter\def\csname BAval@t20.r235.axis\endcsname{0.6}
\expandafter\def\csname BAval@t20.r236.axis\endcsname{0.62}
\expandafter\def\csname BAval@t20.r237.axis\endcsname{0.64}
\expandafter\def\csname BAval@t20.r238.axis\endcsname{0.66}
\expandafter\def\csname BAval@t20.r239.axis\endcsname{0.68}
\expandafter\def\csname BAval@t20.r240.axis\endcsname{0.7}
\expandafter\def\csname BAval@t20.r241.axis\endcsname{0.72}
\expandafter\def\csname BAval@t20.r242.axis\endcsname{0.74}
\expandafter\def\csname BAval@t20.r243.axis\endcsname{0.76}
\expandafter\def\csname BAval@t20.r244.axis\endcsname{0.78}
\expandafter\def\csname BAval@t20.r245.axis\endcsname{0.8}
\expandafter\def\csname BAval@t20.r246.axis\endcsname{0.82}
\expandafter\def\csname BAval@t20.r247.axis\endcsname{0.84}
\expandafter\def\csname BAval@t20.r248.axis\endcsname{0.86}
\expandafter\def\csname BAval@t20.r249.axis\endcsname{0.88}
\expandafter\def\csname BAval@t20.r250.axis\endcsname{0.9}
\expandafter\def\csname BAval@t20.r251.axis\endcsname{0.92}
\expandafter\def\csname BAval@t20.r252.axis\endcsname{0.94}
\expandafter\def\csname BAval@t20.r253.axis\endcsname{0.96}
\expandafter\def\csname BAval@t20.r254.axis\endcsname{0.98}
\expandafter\def\csname BAval@t20.r255.axis\endcsname{1.0}
\expandafter\def\csname BAval@t20.r256.axis\endcsname{0.0}
\expandafter\def\csname BAval@t20.r257.axis\endcsname{0.02}
\expandafter\def\csname BAval@t20.r258.axis\endcsname{0.04}
\expandafter\def\csname BAval@t20.r259.axis\endcsname{0.06}
\expandafter\def\csname BAval@t20.r260.axis\endcsname{0.08}
\expandafter\def\csname BAval@t20.r261.axis\endcsname{0.1}
\expandafter\def\csname BAval@t20.r262.axis\endcsname{0.12}
\expandafter\def\csname BAval@t20.r263.axis\endcsname{0.14}
\expandafter\def\csname BAval@t20.r264.axis\endcsname{0.16}
\expandafter\def\csname BAval@t20.r265.axis\endcsname{0.18}
\expandafter\def\csname BAval@t20.r266.axis\endcsname{0.2}
\expandafter\def\csname BAval@t20.r267.axis\endcsname{0.22}
\expandafter\def\csname BAval@t20.r268.axis\endcsname{0.24}
\expandafter\def\csname BAval@t20.r269.axis\endcsname{0.26}
\expandafter\def\csname BAval@t20.r270.axis\endcsname{0.28}
\expandafter\def\csname BAval@t20.r271.axis\endcsname{0.3}
\expandafter\def\csname BAval@t20.r272.axis\endcsname{0.32}
\expandafter\def\csname BAval@t20.r273.axis\endcsname{0.34}
\expandafter\def\csname BAval@t20.r274.axis\endcsname{0.36}
\expandafter\def\csname BAval@t20.r275.axis\endcsname{0.38}
\expandafter\def\csname BAval@t20.r276.axis\endcsname{0.4}
\expandafter\def\csname BAval@t20.r277.axis\endcsname{0.42}
\expandafter\def\csname BAval@t20.r278.axis\endcsname{0.44}
\expandafter\def\csname BAval@t20.r279.axis\endcsname{0.46}
\expandafter\def\csname BAval@t20.r280.axis\endcsname{0.48}
\expandafter\def\csname BAval@t20.r281.axis\endcsname{0.5}
\expandafter\def\csname BAval@t20.r282.axis\endcsname{0.52}
\expandafter\def\csname BAval@t20.r283.axis\endcsname{0.54}
\expandafter\def\csname BAval@t20.r284.axis\endcsname{0.56}
\expandafter\def\csname BAval@t20.r285.axis\endcsname{0.58}
\expandafter\def\csname BAval@t20.r286.axis\endcsname{0.6}
\expandafter\def\csname BAval@t20.r287.axis\endcsname{0.62}
\expandafter\def\csname BAval@t20.r288.axis\endcsname{0.64}
\expandafter\def\csname BAval@t20.r289.axis\endcsname{0.66}
\expandafter\def\csname BAval@t20.r290.axis\endcsname{0.68}
\expandafter\def\csname BAval@t20.r291.axis\endcsname{0.7}
\expandafter\def\csname BAval@t20.r292.axis\endcsname{0.72}
\expandafter\def\csname BAval@t20.r293.axis\endcsname{0.74}
\expandafter\def\csname BAval@t20.r294.axis\endcsname{0.76}
\expandafter\def\csname BAval@t20.r295.axis\endcsname{0.78}
\expandafter\def\csname BAval@t20.r296.axis\endcsname{0.8}
\expandafter\def\csname BAval@t20.r297.axis\endcsname{0.82}
\expandafter\def\csname BAval@t20.r298.axis\endcsname{0.84}
\expandafter\def\csname BAval@t20.r299.axis\endcsname{0.86}
\expandafter\def\csname BAval@t20.r300.axis\endcsname{0.88}
\expandafter\def\csname BAval@t20.r301.axis\endcsname{0.9}
\expandafter\def\csname BAval@t20.r302.axis\endcsname{0.92}
\expandafter\def\csname BAval@t20.r303.axis\endcsname{0.94}
\expandafter\def\csname BAval@t20.r304.axis\endcsname{0.96}
\expandafter\def\csname BAval@t20.r305.axis\endcsname{0.98}
\expandafter\def\csname BAval@t20.r306.axis\endcsname{1.0}
\expandafter\def\csname BAval@ladder.step.law\endcsname{0.5}
\expandafter\def\csname BAval@ladder.step.id\endcsname{3.3}
\expandafter\def\csname BAval@ladder.step.future\endcsname{1.8}
\expandafter\def\csname BAval@ladder.step.zerodelay\endcsname{6.2}
\expandafter\def\csname BAval@ladder.step.fullview\endcsname{3.9}
\expandafter\def\csname BAval@gap.external.abs\endcsname{12.7}
\expandafter\def\csname BAval@diag.late.full\endcsname{75.8}
\expandafter\def\csname BAval@diag.late.ablated\endcsname{67.7}
\expandafter\def\csname BAval@diag.late.drop\endcsname{8.2}
\expandafter\def\csname BAval@diag.early.full\endcsname{87.0}
\expandafter\def\csname BAval@diag.early.ablated\endcsname{85.8}
\expandafter\def\csname BAval@diag.early.drop\endcsname{1.1}
\expandafter\def\csname BAval@diag.corr.full\endcsname{80.1}
\expandafter\def\csname BAval@diag.corr.ablated\endcsname{73.8}
\expandafter\def\csname BAval@diag.corr.drop\endcsname{6.3}
\expandafter\def\csname BAval@diag.indep.full\endcsname{84.6}
\expandafter\def\csname BAval@diag.indep.ablated\endcsname{84.2}
\expandafter\def\csname BAval@diag.indep.drop\endcsname{0.4}
\expandafter\def\csname BAval@svc.direct.sid\endcsname{78.1}
\expandafter\def\csname BAval@svc.recal.sid\endcsname{81.0}
\expandafter\def\csname BAval@svc.retrain.sid\endcsname{81.7}
\expandafter\def\csname BAval@delta.svc.recal\endcsname{2.9}
\expandafter\def\csname BAval@delta.svc.retrain\endcsname{0.6}
\expandafter\def\csname BAval@lambda.sens.range\endcsname{0.7}
\expandafter\def\csname BAval@t24.r01.lambda.w\endcsname{1}
\expandafter\def\csname BAval@t24.r01.lambda.u\endcsname{1}
\expandafter\def\csname BAval@t24.r02.lambda.w\endcsname{2}
\expandafter\def\csname BAval@t24.r02.lambda.u\endcsname{1}
\expandafter\def\csname BAval@t24.r03.lambda.w\endcsname{4}
\expandafter\def\csname BAval@t24.r03.lambda.u\endcsname{1}
\expandafter\def\csname BAval@t24.r04.lambda.w\endcsname{8}
\expandafter\def\csname BAval@t24.r04.lambda.u\endcsname{1}
\expandafter\def\csname BAval@lambda.w\endcsname{4}
\expandafter\def\csname BAval@lambda.u\endcsname{1}
\expandafter\def\csname BAval@weight.gamma.state\endcsname{1.00}
\expandafter\def\csname BAval@weight.gamma.return\endcsname{0.50}
\expandafter\def\csname BAval@weight.gamma.cost\endcsname{0.10}
\expandafter\def\csname BAval@weight.gamma.rank\endcsname{1.00}
\expandafter\def\csname BAval@weight.gamma.calibration\endcsname{0.20}
\expandafter\def\csname BAval@weight.soft.compute.penalty\endcsname{0.01}
\expandafter\def\csname BAval@weight.soft.motion.penalty\endcsname{0.01}
\expandafter\def\csname BAval@weight.uncertainty.weight\endcsname{0.05}
\expandafter\def\csname BAval@clip.quad.dam.sid\endcsname{1.1}
\expandafter\def\csname BAval@clip.quad.dam.wrong\endcsname{11.1}
\expandafter\def\csname BAval@clip.quad.keep.sid\endcsname{1.1}
\expandafter\def\csname BAval@clip.quad.keep.wrong\endcsname{13.3}
\expandafter\def\csname BAval@clip.dance.dam.sid\endcsname{43.3}
\expandafter\def\csname BAval@clip.dance.dam.wrong\endcsname{11.1}
\expandafter\def\csname BAval@clip.dance.keep.sid\endcsname{40.0}
\expandafter\def\csname BAval@clip.dance.keep.wrong\endcsname{12.8}
\expandafter\def\csname BAval@tick.dance.f272.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f272.dam.sourceage\endcsname{5.70}
\expandafter\def\csname BAval@tick.dance.f272.dam.pubage\endcsname{0.25}
\expandafter\def\csname BAval@tick.dance.f272.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f272.dam.maxcompiou\endcsname{0.320}
\expandafter\def\csname BAval@tick.dance.f272.keep.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f272.keep.sourceage\endcsname{5.70}
\expandafter\def\csname BAval@tick.dance.f272.keep.pubage\endcsname{5.70}
\expandafter\def\csname BAval@tick.dance.f272.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f272.keep.maxcompiou\endcsname{0.342}
\expandafter\def\csname BAval@tick.dance.f272.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f272.bind.sourceage\endcsname{5.70}
\expandafter\def\csname BAval@tick.dance.f272.bind.pubage\endcsname{5.70}
\expandafter\def\csname BAval@tick.dance.f272.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f272.bind.maxcompiou\endcsname{0.342}
\expandafter\def\csname BAval@tick.dance.f279.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f279.dam.sourceage\endcsname{6.05}
\expandafter\def\csname BAval@tick.dance.f279.dam.pubage\endcsname{0.60}
\expandafter\def\csname BAval@tick.dance.f279.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f279.dam.maxcompiou\endcsname{0.314}
\expandafter\def\csname BAval@tick.dance.f279.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f279.keep.sourceage\endcsname{6.05}
\expandafter\def\csname BAval@tick.dance.f279.keep.pubage\endcsname{0.02}
\expandafter\def\csname BAval@tick.dance.f279.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f279.keep.maxcompiou\endcsname{0.278}
\expandafter\def\csname BAval@tick.dance.f279.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f279.bind.sourceage\endcsname{6.05}
\expandafter\def\csname BAval@tick.dance.f279.bind.pubage\endcsname{6.05}
\expandafter\def\csname BAval@tick.dance.f279.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f279.bind.maxcompiou\endcsname{0.337}
\expandafter\def\csname BAval@tick.dance.f280.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f280.dam.sourceage\endcsname{6.10}
\expandafter\def\csname BAval@tick.dance.f280.dam.pubage\endcsname{0.65}
\expandafter\def\csname BAval@tick.dance.f280.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f280.dam.maxcompiou\endcsname{0.332}
\expandafter\def\csname BAval@tick.dance.f280.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f280.keep.sourceage\endcsname{6.10}
\expandafter\def\csname BAval@tick.dance.f280.keep.pubage\endcsname{0.07}
\expandafter\def\csname BAval@tick.dance.f280.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f280.keep.maxcompiou\endcsname{0.293}
\expandafter\def\csname BAval@tick.dance.f280.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f280.bind.sourceage\endcsname{6.10}
\expandafter\def\csname BAval@tick.dance.f280.bind.pubage\endcsname{6.10}
\expandafter\def\csname BAval@tick.dance.f280.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f280.bind.maxcompiou\endcsname{0.355}
\expandafter\def\csname BAval@tick.dance.f281.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f281.dam.sourceage\endcsname{6.15}
\expandafter\def\csname BAval@tick.dance.f281.dam.pubage\endcsname{0.70}
\expandafter\def\csname BAval@tick.dance.f281.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f281.dam.maxcompiou\endcsname{0.343}
\expandafter\def\csname BAval@tick.dance.f281.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f281.keep.sourceage\endcsname{6.15}
\expandafter\def\csname BAval@tick.dance.f281.keep.pubage\endcsname{0.12}
\expandafter\def\csname BAval@tick.dance.f281.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f281.keep.maxcompiou\endcsname{0.301}
\expandafter\def\csname BAval@tick.dance.f281.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f281.bind.sourceage\endcsname{6.15}
\expandafter\def\csname BAval@tick.dance.f281.bind.pubage\endcsname{6.15}
\expandafter\def\csname BAval@tick.dance.f281.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f281.bind.maxcompiou\endcsname{0.366}
\expandafter\def\csname BAval@tick.dance.f282.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f282.dam.sourceage\endcsname{6.20}
\expandafter\def\csname BAval@tick.dance.f282.dam.pubage\endcsname{0.75}
\expandafter\def\csname BAval@tick.dance.f282.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f282.dam.maxcompiou\endcsname{0.336}
\expandafter\def\csname BAval@tick.dance.f282.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f282.keep.sourceage\endcsname{6.20}
\expandafter\def\csname BAval@tick.dance.f282.keep.pubage\endcsname{0.17}
\expandafter\def\csname BAval@tick.dance.f282.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f282.keep.maxcompiou\endcsname{0.292}
\expandafter\def\csname BAval@tick.dance.f282.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f282.bind.sourceage\endcsname{6.20}
\expandafter\def\csname BAval@tick.dance.f282.bind.pubage\endcsname{6.20}
\expandafter\def\csname BAval@tick.dance.f282.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f282.bind.maxcompiou\endcsname{0.358}
\expandafter\def\csname BAval@tick.dance.f283.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f283.dam.sourceage\endcsname{6.25}
\expandafter\def\csname BAval@tick.dance.f283.dam.pubage\endcsname{0.80}
\expandafter\def\csname BAval@tick.dance.f283.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f283.dam.maxcompiou\endcsname{0.281}
\expandafter\def\csname BAval@tick.dance.f283.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f283.keep.sourceage\endcsname{6.25}
\expandafter\def\csname BAval@tick.dance.f283.keep.pubage\endcsname{0.22}
\expandafter\def\csname BAval@tick.dance.f283.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f283.keep.maxcompiou\endcsname{0.226}
\expandafter\def\csname BAval@tick.dance.f283.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f283.bind.sourceage\endcsname{6.25}
\expandafter\def\csname BAval@tick.dance.f283.bind.pubage\endcsname{6.25}
\expandafter\def\csname BAval@tick.dance.f283.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f283.bind.maxcompiou\endcsname{0.297}
\expandafter\def\csname BAval@tick.dance.f284.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f284.dam.sourceage\endcsname{6.30}
\expandafter\def\csname BAval@tick.dance.f284.dam.pubage\endcsname{0.85}
\expandafter\def\csname BAval@tick.dance.f284.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f284.dam.maxcompiou\endcsname{0.298}
\expandafter\def\csname BAval@tick.dance.f284.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f284.keep.sourceage\endcsname{6.30}
\expandafter\def\csname BAval@tick.dance.f284.keep.pubage\endcsname{0.27}
\expandafter\def\csname BAval@tick.dance.f284.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f284.keep.maxcompiou\endcsname{0.242}
\expandafter\def\csname BAval@tick.dance.f284.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f284.bind.sourceage\endcsname{6.30}
\expandafter\def\csname BAval@tick.dance.f284.bind.pubage\endcsname{6.30}
\expandafter\def\csname BAval@tick.dance.f284.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f284.bind.maxcompiou\endcsname{0.314}
\expandafter\def\csname BAval@tick.dance.f296.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f296.dam.sourceage\endcsname{6.90}
\expandafter\def\csname BAval@tick.dance.f296.dam.pubage\endcsname{1.45}
\expandafter\def\csname BAval@tick.dance.f296.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f296.dam.competitor\endcsname{6}
\expandafter\def\csname BAval@tick.dance.f296.dam.compiou\endcsname{0.822}
\expandafter\def\csname BAval@tick.dance.f296.dam.maxcompiou\endcsname{0.822}
\expandafter\def\csname BAval@tick.dance.f296.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f296.keep.sourceage\endcsname{6.90}
\expandafter\def\csname BAval@tick.dance.f296.keep.pubage\endcsname{0.87}
\expandafter\def\csname BAval@tick.dance.f296.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f296.keep.competitor\endcsname{6}
\expandafter\def\csname BAval@tick.dance.f296.keep.compiou\endcsname{0.792}
\expandafter\def\csname BAval@tick.dance.f296.keep.maxcompiou\endcsname{0.792}
\expandafter\def\csname BAval@tick.dance.f296.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f296.bind.sourceage\endcsname{6.90}
\expandafter\def\csname BAval@tick.dance.f296.bind.pubage\endcsname{6.90}
\expandafter\def\csname BAval@tick.dance.f296.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f296.bind.competitor\endcsname{6}
\expandafter\def\csname BAval@tick.dance.f296.bind.compiou\endcsname{0.786}
\expandafter\def\csname BAval@tick.dance.f296.bind.maxcompiou\endcsname{0.786}
\expandafter\def\csname BAval@tick.dance.f320.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f320.dam.sourceage\endcsname{8.10}
\expandafter\def\csname BAval@tick.dance.f320.dam.pubage\endcsname{2.65}
\expandafter\def\csname BAval@tick.dance.f320.dam.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f320.dam.maxcompiou\endcsname{0.474}
\expandafter\def\csname BAval@tick.dance.f320.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.dance.f320.keep.sourceage\endcsname{8.10}
\expandafter\def\csname BAval@tick.dance.f320.keep.pubage\endcsname{2.07}
\expandafter\def\csname BAval@tick.dance.f320.keep.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f320.keep.competitor\endcsname{4}
\expandafter\def\csname BAval@tick.dance.f320.keep.compiou\endcsname{0.502}
\expandafter\def\csname BAval@tick.dance.f320.keep.maxcompiou\endcsname{0.502}
\expandafter\def\csname BAval@tick.dance.f320.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.dance.f320.bind.sourceage\endcsname{8.10}
\expandafter\def\csname BAval@tick.dance.f320.bind.pubage\endcsname{8.10}
\expandafter\def\csname BAval@tick.dance.f320.bind.id\endcsname{5}
\expandafter\def\csname BAval@tick.dance.f320.bind.maxcompiou\endcsname{0.493}
\expandafter\def\csname BAval@tick.quad.f465.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.quad.f465.dam.sourceage\endcsname{5.70}
\expandafter\def\csname BAval@tick.quad.f465.dam.pubage\endcsname{2.25}
\expandafter\def\csname BAval@tick.quad.f465.dam.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f465.dam.maxcompiou\endcsname{0.192}
\expandafter\def\csname BAval@tick.quad.f465.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.quad.f465.keep.sourceage\endcsname{5.70}
\expandafter\def\csname BAval@tick.quad.f465.keep.pubage\endcsname{0.94}
\expandafter\def\csname BAval@tick.quad.f465.keep.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f465.keep.maxcompiou\endcsname{0.232}
\expandafter\def\csname BAval@tick.quad.f465.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.quad.f465.bind.sourceage\endcsname{5.70}
\expandafter\def\csname BAval@tick.quad.f465.bind.pubage\endcsname{5.70}
\expandafter\def\csname BAval@tick.quad.f465.bind.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f465.bind.maxcompiou\endcsname{0.225}
\expandafter\def\csname BAval@tick.quad.f477.dam.revision\endcsname{1}
\expandafter\def\csname BAval@tick.quad.f477.dam.sourceage\endcsname{6.90}
\expandafter\def\csname BAval@tick.quad.f477.dam.pubage\endcsname{3.45}
\expandafter\def\csname BAval@tick.quad.f477.dam.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f477.dam.maxcompiou\endcsname{0.007}
\expandafter\def\csname BAval@tick.quad.f477.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.quad.f477.keep.sourceage\endcsname{6.90}
\expandafter\def\csname BAval@tick.quad.f477.keep.pubage\endcsname{2.14}
\expandafter\def\csname BAval@tick.quad.f477.keep.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f477.keep.maxcompiou\endcsname{0.030}
\expandafter\def\csname BAval@tick.quad.f477.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.quad.f477.bind.sourceage\endcsname{6.90}
\expandafter\def\csname BAval@tick.quad.f477.bind.pubage\endcsname{6.90}
\expandafter\def\csname BAval@tick.quad.f477.bind.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f477.bind.maxcompiou\endcsname{0.027}
\expandafter\def\csname BAval@tick.quad.f489.dam.revision\endcsname{2}
\expandafter\def\csname BAval@tick.quad.f489.dam.sourceage\endcsname{4.69}
\expandafter\def\csname BAval@tick.quad.f489.dam.pubage\endcsname{0.44}
\expandafter\def\csname BAval@tick.quad.f489.dam.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f489.dam.maxcompiou\endcsname{0.363}
\expandafter\def\csname BAval@tick.quad.f489.keep.revision\endcsname{1}
\expandafter\def\csname BAval@tick.quad.f489.keep.sourceage\endcsname{8.10}
\expandafter\def\csname BAval@tick.quad.f489.keep.pubage\endcsname{3.34}
\expandafter\def\csname BAval@tick.quad.f489.keep.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f489.keep.competitor\endcsname{101}
\expandafter\def\csname BAval@tick.quad.f489.keep.compiou\endcsname{0.547}
\expandafter\def\csname BAval@tick.quad.f489.keep.maxcompiou\endcsname{0.547}
\expandafter\def\csname BAval@tick.quad.f489.bind.revision\endcsname{0}
\expandafter\def\csname BAval@tick.quad.f489.bind.sourceage\endcsname{8.10}
\expandafter\def\csname BAval@tick.quad.f489.bind.pubage\endcsname{8.10}
\expandafter\def\csname BAval@tick.quad.f489.bind.id\endcsname{59}
\expandafter\def\csname BAval@tick.quad.f489.bind.competitor\endcsname{101}
\expandafter\def\csname BAval@tick.quad.f489.bind.compiou\endcsname{0.531}
\expandafter\def\csname BAval@tick.quad.f489.bind.maxcompiou\endcsname{0.531}
\expandafter\def\csname BAval@goal.B.f100.x\endcsname{647}
\expandafter\def\csname BAval@goal.B.f100.y\endcsname{438}
\expandafter\def\csname BAval@goal.B.f100.width\endcsname{100}
\expandafter\def\csname BAval@goal.B.f100.height\endcsname{305}
\expandafter\def\csname BAval@goal.B.f120.x\endcsname{676}
\expandafter\def\csname BAval@goal.B.f120.y\endcsname{438}
\expandafter\def\csname BAval@goal.B.f120.width\endcsname{97}
\expandafter\def\csname BAval@goal.B.f120.height\endcsname{318}
\expandafter\def\csname BAval@goal.B.f140.x\endcsname{693}
\expandafter\def\csname BAval@goal.B.f140.y\endcsname{434}
\expandafter\def\csname BAval@goal.B.f140.width\endcsname{109}
\expandafter\def\csname BAval@goal.B.f140.height\endcsname{328}
\expandafter\def\csname BAval@goal.D.f240.x\endcsname{348}
\expandafter\def\csname BAval@goal.D.f240.y\endcsname{202}
\expandafter\def\csname BAval@goal.D.f240.width\endcsname{50}
\expandafter\def\csname BAval@goal.D.f240.height\endcsname{165}
\expandafter\def\csname BAval@goal.D.f272.x\endcsname{324}
\expandafter\def\csname BAval@goal.D.f272.y\endcsname{295}
\expandafter\def\csname BAval@goal.D.f272.width\endcsname{89}
\expandafter\def\csname BAval@goal.D.f272.height\endcsname{242}
\expandafter\def\csname BAval@goal.D.f300.x\endcsname{634}
\expandafter\def\csname BAval@goal.D.f300.y\endcsname{228}
\expandafter\def\csname BAval@goal.D.f300.width\endcsname{69}
\expandafter\def\csname BAval@goal.D.f300.height\endcsname{212}


==> supp_numbers_update_20261117.tex <==
\expandafter\def\csname BAval@t17.r01.dam4sam.chanakya.j\endcsname{80.12}
\expandafter\def\csname BAval@t17.r01.bindadapt\endcsname{84.22}
\expandafter\def\csname BAval@t17.r02.dam4sam.chanakya.j\endcsname{79.36}
\expandafter\def\csname BAval@t17.r02.bindadapt\endcsname{84.09}
\expandafter\def\csname BAval@t17.r03.dam4sam.chanakya.j\endcsname{77.84}
\expandafter\def\csname BAval@t17.r03.bindadapt\endcsname{83.46}
\expandafter\def\csname BAval@t17.r04.dam4sam.chanakya.j\endcsname{75.20}
\expandafter\def\csname BAval@t17.r04.bindadapt\endcsname{82.30}
\expandafter\def\csname BAval@t17.r05.dam4sam.chanakya.j\endcsname{68.46}
\expandafter\def\csname BAval@t17.r05.bindadapt\endcsname{78.13}
\expandafter\def\csname BAval@t17.r06.dam4sam.chanakya.j\endcsname{54.82}
\expandafter\def\csname BAval@t17.r06.bindadapt\endcsname{67.02}
\expandafter\def\csname BAval@delta.sweep.zero\endcsname{4.10}
\expandafter\def\csname BAval@delta.sweep.ref\endcsname{7.10}
\expandafter\def\csname BAval@delta.sweep.two\endcsname{12.20}
\expandafter\def\csname BAval@svc.direct.sid\endcsname{81.34}
\expandafter\def\csname BAval@svc.recal.sid\endcsname{83.62}
\expandafter\def\csname BAval@svc.retrain.sid\endcsname{84.03}
\expandafter\def\csname BAval@delta.svc.recal\endcsname{2.28}
\expandafter\def\csname BAval@delta.svc.retrain\endcsname{0.41}
\expandafter\def\csname BAval@delta.svc.gap\endcsname{2.69}


==> supp_numbers_v38.tex <==
\expandafter\def\csname BAval@sd.ext.advat\endcsname{0.3}
\expandafter\def\csname BAval@sd.ext.oavat\endcsname{0.2}
\expandafter\def\csname BAval@sd.ext.pvt\endcsname{0.4}
\expandafter\def\csname BAval@sd.ext.artrack\endcsname{0.3}
\expandafter\def\csname BAval@sd.ext.chanakya\endcsname{0.6}
\expandafter\def\csname BAval@sd.ext.joint\endcsname{0.8}
\expandafter\def\csname BAval@sd.ext.best\endcsname{0.2}
\expandafter\def\csname BAval@sd.ext.bind\endcsname{0.3}
\expandafter\def\csname BAval@sd.t03.r01\endcsname{0.6}
\expandafter\def\csname BAval@sd.t03.r02\endcsname{0.9}
\expandafter\def\csname BAval@sd.t03.r03\endcsname{0.3}
\expandafter\def\csname BAval@sd.t03.r04\endcsname{0.3}
\expandafter\def\csname BAval@t03.r01.sidx\endcsname{65.9}
\expandafter\def\csname BAval@t03.r02.sidx\endcsname{70.3}
\expandafter\def\csname BAval@t03.r03.sidx\endcsname{77.6}
\expandafter\def\csname BAval@t03.r04.sidx\endcsname{82.3}
\expandafter\def\csname BAval@sd.t04.r01\endcsname{0.3}
\expandafter\def\csname BAval@sd.t04.r02\endcsname{0.2}
\expandafter\def\csname BAval@sd.t04.r03\endcsname{0.2}
\expandafter\def\csname BAval@sd.t04.r04\endcsname{0.9}
\expandafter\def\csname BAval@sd.t04.r05\endcsname{1.1}
\expandafter\def\csname BAval@sd.t04.r06\endcsname{0.3}
\expandafter\def\csname BAval@sd.t04.r07\endcsname{0.3}
\expandafter\def\csname BAval@abl.unc.sid\endcsname{80.5}
\expandafter\def\csname BAval@abl.unc.wrong\endcsname{5.8}
\expandafter\def\csname BAval@abl.unc.t5\endcsname{1.5}
\expandafter\def\csname BAval@abl.unc.drop\endcsname{1.8}
\expandafter\def\csname BAval@sd.abl.unc\endcsname{0.1}
\expandafter\def\csname BAval@abl.imm.sid\endcsname{76.2}
\expandafter\def\csname BAval@abl.imm.wrong\endcsname{7.1}
\expandafter\def\csname BAval@abl.imm.t5\endcsname{1.7}
\expandafter\def\csname BAval@abl.imm.drop\endcsname{6.1}
\expandafter\def\csname BAval@rule.prox.sid\endcsname{73.6}
\expandafter\def\csname BAval@rule.prox.wrong\endcsname{8.0}
\expandafter\def\csname BAval@rule.prox.t5\endcsname{1.8}
\expandafter\def\csname BAval@rule.prox.drop\endcsname{8.7}
\expandafter\def\csname BAval@rule.prox.k\endcsname{1.5}
\expandafter\def\csname BAval@rule.rate.sid\endcsname{71.4}
\expandafter\def\csname BAval@rule.rate.wrong\endcsname{8.8}
\expandafter\def\csname BAval@rule.rate.t5\endcsname{1.6}
\expandafter\def\csname BAval@rule.rate.drop\endcsname{10.9}
\expandafter\def\csname BAval@rule.rate.period\endcsname{0.6}
\expandafter\def\csname BAval@rule.prox.long\endcsname{61.4}
\expandafter\def\csname BAval@rule.rate.long\endcsname{58.9}
\expandafter\def\csname BAval@ci.lo\endcsname{5.1}
\expandafter\def\csname BAval@ci.hi\endcsname{9.0}
\expandafter\def\csname BAval@ci.groups\endcsname{40}
\expandafter\def\csname BAval@ci.resamples\endcsname{10{,}000}
\expandafter\def\csname BAval@idf1.best\endcsname{77.5}
\expandafter\def\csname BAval@idf1.bind\endcsname{83.5}
\expandafter\def\csname BAval@hota.best\endcsname{61.8}
\expandafter\def\csname BAval@hota.bind\endcsname{67.3}
\expandafter\def\csname BAval@tune.configs\endcsname{24}
\expandafter\def\csname BAval@tune.seeds\endcsname{3}
\expandafter\def\csname BAval@tune.groups\endcsname{20}
\expandafter\def\csname BAval@retsweep.episodes\endcsname{243}
\expandafter\def\csname BAval@retsweep.early\endcsname{94.2}
\expandafter\def\csname BAval@retsweep.zero\endcsname{80.7}
\expandafter\def\csname BAval@retsweep.late\endcsname{56.8}
\expandafter\def\csname BAval@attr.dam.total\endcsname{137}
\expandafter\def\csname BAval@attr.dam.after\endcsname{89}
\expandafter\def\csname BAval@attr.dam.pct\endcsname{65.0}
\expandafter\def\csname BAval@attr.keep.total\endcsname{151}
\expandafter\def\csname BAval@attr.keep.after\endcsname{87}
\expandafter\def\csname BAval@attr.keep.pct\endcsname{57.6}
\expandafter\def\csname BAval@attr.best.total\endcsname{97}
\expandafter\def\csname BAval@attr.best.after\endcsname{61}
\expandafter\def\csname BAval@attr.best.pct\endcsname{62.9}
\expandafter\def\csname BAval@attr.bind.total\endcsname{53}
\expandafter\def\csname BAval@attr.bind.after\endcsname{18}
\expandafter\def\csname BAval@attr.bind.pct\endcsname{34.0}
\expandafter\def\csname BAval@plan.mean\endcsname{2.1}
\expandafter\def\csname BAval@plan.p95\endcsname{3.8}
\expandafter\def\csname BAval@plan.decisions\endcsname{10{,}000}
\expandafter\def\csname BAval@plan.limit\endcsname{10}
\expandafter\def\csname BAval@cost.mixformer\endcsname{19.8}
\expandafter\def\csname BAval@cost.hiptrack\endcsname{27.5}
\expandafter\def\csname BAval@cost.odtrack\endcsname{22.2}
\expandafter\def\csname BAval@cost.ltmu\endcsname{31.8}
\expandafter\def\csname BAval@cost.keeptrack\endcsname{29.1}
\expandafter\def\csname BAval@cost.advat\endcsname{18.6}
\expandafter\def\csname BAval@cost.joint\endcsname{38.1}
\expandafter\def\csname BAval@sens.h1\endcsname{78.6}
\expandafter\def\csname BAval@sens.h15\endcsname{80.9}
\expandafter\def\csname BAval@sens.h2\endcsname{82.3}
\expandafter\def\csname BAval@sens.h3\endcsname{81.9}
\expandafter\def\csname BAval@sens.h1.ms\endcsname{1.38}
\expandafter\def\csname BAval@sens.h15.ms\endcsname{1.72}
\expandafter\def\csname BAval@sens.h2.ms\endcsname{2.09}
\expandafter\def\csname BAval@sens.h3.ms\endcsname{2.73}
\expandafter\def\csname BAval@sens.b4\endcsname{79.8}
\expandafter\def\csname BAval@sens.b8\endcsname{82.3}
\expandafter\def\csname BAval@sens.b16\endcsname{82.4}
\expandafter\def\csname BAval@sens.b4.ms\endcsname{1.42}
\expandafter\def\csname BAval@sens.b8.ms\endcsname{2.09}
\expandafter\def\csname BAval@sens.b16.ms\endcsname{3.61}
\expandafter\def\csname BAval@sens.d2\endcsname{79.9}
\expandafter\def\csname BAval@sens.d3\endcsname{82.3}
\expandafter\def\csname BAval@sens.d4\endcsname{82.4}
\expandafter\def\csname BAval@sens.d2.ms\endcsname{1.26}
\expandafter\def\csname BAval@sens.d3.ms\endcsname{2.09}
\expandafter\def\csname BAval@sens.d4.ms\endcsname{3.84}
\expandafter\def\csname BAval@t27.r01.correct.s\endcsname{7.40}
\expandafter\def\csname BAval@t27.r01.wrong.s\endcsname{0.21}
\expandafter\def\csname BAval@t27.r01.sid\endcsname{82.2}
\expandafter\def\csname BAval@t27.r01.wrong\endcsname{2.4}
\expandafter\def\csname BAval@t27.r02.correct.s\endcsname{7.07}
\expandafter\def\csname BAval@t27.r02.wrong.s\endcsname{0.35}
\expandafter\def\csname BAval@t27.r02.sid\endcsname{78.5}
\expandafter\def\csname BAval@t27.r02.wrong\endcsname{3.9}
\expandafter\def\csname BAval@t10.r01.separable\endcsname{77.6}
\expandafter\def\csname BAval@t10.r01.temporal.q\endcsname{68.7}
\expandafter\def\csname BAval@sens.h.drop\endcsname{3.6}
\expandafter\def\csname BAval@sens.search.gain\endcsname{0.1}


==> supp_numbers_v41.tex <==
\expandafter\def\csname BAval@svc.retrain.sid\endcsname{81.6}
\expandafter\def\csname BAval@delta.svc.gap\endcsname{3.5}


==> supp_unsure_flags.tex <==
\expandafter\def\csname BAflag@int.joint.recovery\endcsname{}
\expandafter\def\csname BAflag@int.joint.t5\endcsname{}
\expandafter\def\csname BAflag@int.oracle.recovery\endcsname{}
\expandafter\def\csname BAflag@int.oracle.t5\endcsname{}
\expandafter\def\csname BAflag@int.oracle.wrong\endcsname{}
\expandafter\def\csname BAflag@t01.r01.recovery\endcsname{}
\expandafter\def\csname BAflag@t01.r01.sid\endcsname{}
\expandafter\def\csname BAflag@t01.r01.t5\endcsname{}
\expandafter\def\csname BAflag@t01.r01.wrong\endcsname{}
\expandafter\def\csname BAflag@t01.r02.recovery\endcsname{}
\expandafter\def\csname BAflag@t01.r02.sid\endcsname{}
\expandafter\def\csname BAflag@t01.r02.t5\endcsname{}
\expandafter\def\csname BAflag@t01.r02.wrong\endcsname{}
\expandafter\def\csname BAflag@t01.r03.recovery\endcsname{}
\expandafter\def\csname BAflag@t01.r03.sid\endcsname{}
\expandafter\def\csname BAflag@t01.r03.t5\endcsname{}
\expandafter\def\csname BAflag@t01.r03.wrong\endcsname{}
\expandafter\def\csname BAflag@t01.r04.recovery\endcsname{}
\expandafter\def\csname BAflag@t01.r04.sid\endcsname{}
\expandafter\def\csname BAflag@t01.r04.t5\endcsname{}
\expandafter\def\csname BAflag@t01.r04.wrong\endcsname{}
\expandafter\def\csname BAflag@t01.r05.recovery\endcsname{}
\expandafter\def\csname BAflag@t01.r05.sid\endcsname{}
\expandafter\def\csname BAflag@t01.r05.t5\endcsname{}
\expandafter\def\csname BAflag@t01.r05.wrong\endcsname{}
\expandafter\def\csname BAflag@t01.r07.recovery\endcsname{}
\expandafter\def\csname BAflag@t01.r07.t5\endcsname{}
\expandafter\def\csname BAflag@t01.r09.recovery\endcsname{}
\expandafter\def\csname BAflag@t01.r09.t5\endcsname{}
\expandafter\def\csname BAflag@t01.r09.wrong\endcsname{}
\expandafter\def\csname BAflag@t02.r01.long\endcsname{}
\expandafter\def\csname BAflag@t02.r01.short\endcsname{}
\expandafter\def\csname BAflag@t02.r01.similar\endcsname{}
\expandafter\def\csname BAflag@t02.r02.long\endcsname{}
\expandafter\def\csname BAflag@t02.r02.short\endcsname{}
\expandafter\def\csname BAflag@t02.r02.similar\endcsname{}
\expandafter\def\csname BAflag@t02.r03.long\endcsname{}
\expandafter\def\csname BAflag@t02.r03.short\endcsname{}
\expandafter\def\csname BAflag@t02.r03.similar\endcsname{}
\expandafter\def\csname BAflag@t02.r04.long\endcsname{}
\expandafter\def\csname BAflag@t02.r04.short\endcsname{}
\expandafter\def\csname BAflag@t02.r04.similar\endcsname{}
\expandafter\def\csname BAflag@t02.r06.long\endcsname{}
\expandafter\def\csname BAflag@t02.r06.short\endcsname{}
\expandafter\def\csname BAflag@t02.r06.similar\endcsname{}


==> tables/ablation_styled.tex <==
\rowcolor{BAours}\textbf{Full BindAdapt} & \textbf{\BAval{t04.r01.sid}}\BApm{\BAval{sd.t04.r01}} & \textcolor{BAdash}{--} & \textbf{\BAval{t04.r01.wrong}} & \textbf{\BAval{t04.r01.t5}}\\
\rowcolor{BAgroup}\multicolumn{5}{@{\hspace{3pt}}l}{\textbf{\textit{\ding{172}~Provenance graph}}}\\
\hspace{3pt}No source dependencies & \BAval{t04.r05.sid}\BApm{\BAval{sd.t04.r05}} & \textcolor{BAloss}{$-$\BAval{tab.abl.src}} & \BAval{t04.r05.wrong} & \BAval{t04.r05.t5}\\
\hspace{3pt}No memory summary & \BAval{t04.r04.sid}\BApm{\BAval{sd.t04.r04}} & \textcolor{BAloss}{$-$\BAval{tab.abl.mem}} & \BAval{t04.r04.wrong} & \BAval{t04.r04.t5}\\
\rowcolor{BAgroup}\multicolumn{5}{@{\hspace{3pt}}l}{\textbf{\textit{\ding{173}~Identity response}}}\\
\hspace{3pt}No target conditioning & \BAval{t04.r03.sid}\BApm{\BAval{sd.t04.r03}} & \textcolor{BAloss}{$-$\BAval{tab.abl.tgt}} & \BAval{t04.r03.wrong} & \BAval{t04.r03.t5}\\
\hspace{3pt}No return time & \BAval{t04.r02.sid}\BApm{\BAval{sd.t04.r02}} & \textcolor{BAloss}{$-$\BAval{tab.abl.ret}} & \BAval{t04.r02.wrong} & \BAval{t04.r02.t5}\\
\hspace{3pt}No uncertainty term & \BAval{abl.unc.sid}\BApm{\BAval{sd.abl.unc}} & \textcolor{BAloss}{$-$\BAval{abl.unc.drop}} & \BAval{abl.unc.wrong} & \BAval{abl.unc.t5}\\
\rowcolor{BAgroup}\multicolumn{5}{@{\hspace{3pt}}l}{\textbf{\textit{\ding{174}~Joint scheduling}}}\\
\hspace{3pt}Immediate start only & \BAval{abl.imm.sid} & \textcolor{BAloss}{$-$\BAval{abl.imm.drop}} & \BAval{abl.imm.wrong} & \BAval{abl.imm.t5}\\
\hspace{3pt}Fixed computation type & \BAval{t04.r06.sid}\BApm{\BAval{sd.t04.r06}} & \textcolor{BAloss}{$-$\BAval{tab.abl.fix}} & \BAval{t04.r06.wrong} & \BAval{t04.r06.t5}\\
\rowcolor{BAgroup}\multicolumn{5}{@{\hspace{3pt}}l}{\textbf{\textit{Rule-based scheduling controls}}}\\
\hspace{3pt}Check when a person approaches & \BAval{rule.prox.sid} & \textcolor{BAloss}{$-$\BAval{rule.prox.drop}} & \BAval{rule.prox.wrong} & \BAval{rule.prox.t5}\\
\hspace{3pt}Check at a fixed rate & \BAval{rule.rate.sid} & \textcolor{BAloss}{$-$\BAval{rule.rate.drop}} & \BAval{rule.rate.wrong} & \BAval{rule.rate.t5}\\


==> tables/backbone_styled.tex <==
OSTrack & \BAval{t15.r01.common.controller} & \BAval{t15.r01.oa.vat.ptz} & \underline{\BAval{t15.r01.chanakya.j}} & \cellcolor{BAours}\textbf{\BAval{t15.r01.bindadapt}} & \textcolor{BAgain}{$+$\BAval{delta.backbone.ost}}\\
LoRATv2 & \BAval{t15.r02.common.controller} & \BAval{t15.r02.oa.vat.ptz} & \underline{\BAval{t15.r02.chanakya.j}} & \cellcolor{BAours}\textbf{\BAval{t15.r02.bindadapt}} & \textcolor{BAgain}{$+$\BAval{delta.backbone.lorat}}\\
DAM4SAM & \BAval{t15.r03.common.controller} & \BAval{t15.r03.oa.vat.ptz} & \underline{\BAval{t15.r03.chanakya.j}} & \cellcolor{BAours}\textbf{\BAval{t15.r03.bindadapt}} & \textcolor{BAgain}{$+$\BAval{delta.backbone.dam}}\\


==> tables/external_full.tex <==
\rowcolor{BAgroup}\multicolumn{12}{@{\hspace{3pt}}l}{\textbf{\textit{Perception trackers under a common PTZ controller}}}\\
OSTrack~\cite{ostrack} & self & \BAval{t12.r01.sid} & \BAval{t12.r01.wrong} & \BAval{t12.r01.recovery} & \BAval{t12.r01.t5} & \BAval{t14.r07.short} & \BAval{t14.r07.similar} & \BAval{t14.r07.long} & \BAval{t13.r01.ao} & \BAval{t13.r01.sao.pct} & \BAval{t18.r01.mean.inference.ms}\\
MixFormerV2~\cite{mixformerv2} & self & \BAval{t12.r02.sid} & \BAval{t12.r02.wrong} & \BAval{t12.r02.recovery} & \BAval{t12.r02.t5} & \BAval{t14.r08.short} & \BAval{t14.r08.similar} & \BAval{t14.r08.long} & \BAval{t13.r02.ao} & \BAval{t13.r02.sao.pct} & \BAval{cost.mixformer}\\
HIPTrack~\cite{hiptrack} & self & \BAval{t12.r03.sid} & \BAval{t12.r03.wrong} & \BAval{t12.r03.recovery} & \BAval{t12.r03.t5} & \BAval{t14.r09.short} & \BAval{t14.r09.similar} & \BAval{t14.r09.long} & \BAval{t13.r03.ao} & \BAval{t13.r03.sao.pct} & \BAval{cost.hiptrack}\\
ODTrack~\cite{odtrack} & self & \BAval{t12.r04.sid} & \BAval{t12.r04.wrong} & \BAval{t12.r04.recovery} & \BAval{t12.r04.t5} & \BAval{t14.r10.short} & \BAval{t14.r10.similar} & \BAval{t14.r10.long} & \BAval{t13.r04.ao} & \BAval{t13.r04.sao.pct} & \BAval{cost.odtrack}\\
LoRATv2~\cite{loratv2} & self & \BAval{t12.r05.sid} & \BAval{t12.r05.wrong} & \BAval{t12.r05.recovery} & \BAval{t12.r05.t5} & \BAval{t14.r11.short} & \BAval{t14.r11.similar} & \BAval{t14.r11.long} & \BAval{t13.r05.ao} & \BAval{t13.r05.sao.pct} & \BAval{t18.r02.mean.inference.ms}\\
LTMU~\cite{ltmu} & self & \BAval{t12.r06.sid} & \BAval{t12.r06.wrong} & \BAval{t12.r06.recovery} & \BAval{t12.r06.t5} & \BAval{t14.r12.short} & \BAval{t14.r12.similar} & \BAval{t14.r12.long} & \BAval{t13.r06.ao} & \BAval{t13.r06.sao.pct} & \BAval{cost.ltmu}\\
KeepTrack~\cite{keeptrack} & self & \BAval{t12.r07.sid} & \BAval{t12.r07.wrong} & \BAval{t12.r07.recovery} & \BAval{t12.r07.t5} & \BAval{t14.r13.short} & \BAval{t14.r13.similar} & \BAval{t14.r13.long} & \BAval{t13.r07.ao} & \BAval{t13.r07.sao.pct} & \BAval{cost.keeptrack}\\
DAM4SAM~\cite{dam4sam} & self & \BAval{t12.r08.sid} & \BAval{t12.r08.wrong} & \BAval{t12.r08.recovery} & \BAval{t12.r08.t5} & \BAval{t14.r01.short} & \BAval{t14.r01.similar} & \BAval{t14.r01.long} & \underline{\BAval{t13.r08.ao}} & \BAval{t13.r08.sao.pct} & \BAval{t18.r03.mean.inference.ms}\\
\rowcolor{BAgroup}\multicolumn{12}{@{\hspace{3pt}}l}{\textbf{\textit{Active camera controllers}}}\\
AD-VAT+-PTZ~\cite{advat} & built-in & \BAval{t12.r09.sid}\BApm{\BAval{sd.ext.advat}} & \BAval{t12.r09.wrong} & \BAval{t12.r09.recovery} & \BAval{t12.r09.t5} & \BAval{t14.r14.short} & \BAval{t14.r14.similar} & \BAval{t14.r14.long} & \textcolor{BAdash}{--} & \textcolor{BAdash}{--} & \BAval{cost.advat}\\
OA-VAT-PTZ~\cite{oavat} & built-in & \BAval{t12.r10.sid}\BApm{\BAval{sd.ext.oavat}} & \BAval{t12.r10.wrong} & \BAval{t12.r10.recovery} & \BAval{t12.r10.t5} & \BAval{t14.r02.short} & \BAval{t14.r02.similar} & \BAval{t14.r02.long} & \textcolor{BAdash}{--} & \textcolor{BAdash}{--} & \BAval{t18.r06.mean.inference.ms}\\
\rowcolor{BAgroup}\multicolumn{12}{@{\hspace{3pt}}l}{\textbf{\textit{Delay- and capacity-adaptive trackers}}}\\
PVT++~\cite{pvtpp} & SiamRPN++~\cite{siamrpnpp} & \BAval{t12.r11.sid}\BApm{\BAval{sd.ext.pvt}} & \BAval{t12.r11.wrong} & \BAval{t12.r11.recovery} & \BAval{t12.r11.t5} & \BAval{t14.r15.short} & \BAval{t14.r15.similar} & \BAval{t14.r15.long} & \BAval{t13.r09.ao} & \BAval{t13.r09.sao.pct} & \BAval{t18.r04.mean.inference.ms}\\
ARTrack-AC~\cite{artrackac} & ARTrack & \BAval{t12.r12.sid}\BApm{\BAval{sd.ext.artrack}} & \BAval{t12.r12.wrong} & \BAval{t12.r12.recovery} & \BAval{t12.r12.t5} & \BAval{t14.r03.short} & \BAval{t14.r03.similar} & \BAval{t14.r03.long} & \BAval{t13.r10.ao} & \underline{\BAval{t13.r10.sao.pct}} & \BAval{t18.r05.mean.inference.ms}\\
\rowcolor{BAgroup}\multicolumn{12}{@{\hspace{3pt}}l}{\textbf{\textit{Joint view and computation policies}}}\\
Chanakya-J~\cite{chanakya} & built-in & \BAval{t12.r13.sid}\BApm{\BAval{sd.ext.chanakya}} & \BAval{t12.r13.wrong} & \BAval{t12.r13.recovery} & \BAval{t12.r13.t5} & \BAval{t14.r04.short} & \BAval{t14.r04.similar} & \BAval{t14.r04.long} & \textcolor{BAdash}{--} & \textcolor{BAdash}{--} & \BAval{t18.r07.mean.inference.ms}\\
DAM4SAM + joint belief~\cite{dam4sam} & DAM4SAM & \BAval{t12.r14.sid}\BApm{\BAval{sd.ext.joint}} & \underline{\BAval{t12.r14.wrong}} & \BAval{t12.r14.recovery} & \underline{\BAval{t12.r14.t5}} & \underline{\BAval{t14.r16.short}} & \underline{\BAval{t14.r16.similar}} & \BAval{t14.r16.long} & \textcolor{BAdash}{--} & \textcolor{BAdash}{--} & \BAval{cost.joint}\\
DAM4SAM + Chanakya-J~\cite{dam4sam,chanakya} & DAM4SAM & \underline{\BAval{t12.r15.sid}}\BApm{\BAval{sd.ext.best}} & \BAval{t12.r15.wrong} & \underline{\BAval{t12.r15.recovery}} & \underline{\BAval{t12.r15.t5}} & \BAval{t14.r05.short} & \BAval{t14.r05.similar} & \underline{\BAval{t14.r05.long}} & \textcolor{BAdash}{--} & \textcolor{BAdash}{--} & \BAval{t18.r08.mean.inference.ms}\\
\rowcolor{BAours}\textbf{BindAdapt (ours)} & DAM4SAM & \textbf{\BAval{t12.r16.sid}}\BApm{\BAval{sd.ext.bind}} & \textbf{\BAval{t12.r16.wrong}} & \textbf{\BAval{t12.r16.recovery}} & \textbf{\BAval{t12.r16.t5}} & \textbf{\BAval{t14.r06.short}} & \textbf{\BAval{t14.r06.similar}} & \textbf{\BAval{t14.r06.long}} & \textbf{\BAval{t13.r11.ao}} & \textbf{\BAval{t13.r11.sao.pct}} & \BAval{t18.r09.mean.inference.ms}\\
\multicolumn{2}{@{}l}{$\Delta$ vs.\ DAM4SAM + Chanakya-J} & \textcolor{BAgain}{$+$\BAval{tab.delta.sid}} & \textcolor{BAgain}{$-$\BAval{tab.delta.wrong}} & \textcolor{BAgain}{$+$\BAval{tab.delta.recovery}} & \textcolor{BAgain}{$-$\BAval{tab.delta.t5}} & \textcolor{BAgain}{$+$\BAval{tab.delta.short}} & \textcolor{BAgain}{$+$\BAval{tab.delta.similar}} & \textcolor{BAgain}{$+$\BAval{tab.delta.long}} &  &  & \textcolor{BAgain}{$-$\BAval{tab.delta.ms}}\\


==> tables/sablation.tex <==
\rowcolor{BAours}Full model & \BAval{t04.r01.sid} & \BAval{t04.r01.wrong} & \BAval{t04.r01.t5}\\
No source dependencies & \BAval{t04.r05.sid} & \BAval{t04.r05.wrong} & \BAval{t04.r05.t5}\\
No memory summary & \BAval{t04.r04.sid} & \BAval{t04.r04.wrong} & \BAval{t04.r04.t5}\\
No target conditioning & \BAval{t04.r03.sid} & \BAval{t04.r03.wrong} & \BAval{t04.r03.t5}\\
No return time & \BAval{t04.r02.sid} & \BAval{t04.r02.wrong} & \BAval{t04.r02.t5}\\
No uncertainty term & \BAval{t04.r08.sid} & \BAval{t04.r08.wrong} & \BAval{t04.r08.t5}\\
Separable scheduler & \BAval{t04.r07.sid} & \BAval{t04.r07.wrong} & \BAval{t04.r07.t5}\\
Immediate start only & \BAval{abl.imm.sid} & \BAval{abl.imm.wrong} & \BAval{abl.imm.t5}\\
Fixed computation type & \BAval{t04.r06.sid} & \BAval{t04.r06.wrong} & \BAval{t04.r06.t5}\\


==> tables/scar.tex <==
Common PTZ controller & \BAval{t21.r01.car.pct}\\
AD-VAT+-PTZ & \BAval{t21.r02.car.pct}\\
OA-VAT-PTZ & \BAval{t21.r03.car.pct}\\
Chanakya-J & \BAval{t21.r04.car.pct}\\
\rowcolor{BAours}BindAdapt & \BAval{t21.r05.car.pct}\\


==> tables/sceil.tex <==
No identity ambiguity & \BAval{t11.r01.reference} & \BAval{t11.r01.bindadapt} & \BAval{t11.r01.gain.pp}\\
Frozen scene and negligible delay & \BAval{t11.r02.reference} & \BAval{t11.r02.bindadapt} & \BAval{t11.r02.gain.pp}\\
Ambiguity with delayed computation & \BAval{t11.r03.reference} & \BAval{t11.r03.bindadapt} & \BAval{t11.r03.gain.pp}\\
Identity cues withheld & \BAval{t11.r04.reference} & \BAval{t11.r04.bindadapt} & \BAval{t11.r04.gain.pp}\\
Absence outside every reachable view & \BAval{t11.r05.reference} & \BAval{t11.r05.bindadapt} & \BAval{t11.r05.gain.pp}\\


==> tables/selae.tex <==
LoRATv2 & \BAval{t19.r01.auc.la0.pct} & \BAval{t19.r01.dp.la0.pct} & \BAval{t19.r01.mauc.pct} & \BAval{t19.r01.mdp.pct}\\
DAM4SAM & \BAval{t19.r02.auc.la0.pct} & \BAval{t19.r02.dp.la0.pct} & \BAval{t19.r02.mauc.pct} & \BAval{t19.r02.mdp.pct}\\
PVT++ & \BAval{t19.r03.auc.la0.pct} & \BAval{t19.r03.dp.la0.pct} & \BAval{t19.r03.mauc.pct} & \BAval{t19.r03.mdp.pct}\\
ARTrack-AC & \BAval{t19.r04.auc.la0.pct} & \BAval{t19.r04.dp.la0.pct} & \BAval{t19.r04.mauc.pct} & \BAval{t19.r04.mdp.pct}\\
Chanakya-J & \BAval{t19.r05.auc.la0.pct} & \BAval{t19.r05.dp.la0.pct} & \BAval{t19.r05.mauc.pct} & \BAval{t19.r05.mdp.pct}\\
\rowcolor{BAours}BindAdapt & \textbf{\BAval{t19.r06.auc.la0.pct}} & \textbf{\BAval{t19.r06.dp.la0.pct}} & \textbf{\BAval{t19.r06.mauc.pct}} & \textbf{\BAval{t19.r06.mdp.pct}}\\


==> tables/sgen.tex <==
Unseen scene groups & \BAval{t10.r01.separable} & \BAval{t10.r01.temporal.q} & \textbf{\BAval{t10.r01.bindadapt}}\\
Unseen target identities & \BAval{t10.r02.separable} & \BAval{t10.r02.temporal.q} & \textbf{\BAval{t10.r02.bindadapt}}\\
Unseen service profiles & \BAval{t10.r03.separable} & \BAval{t10.r03.temporal.q} & \textbf{\BAval{t10.r03.bindadapt}}\\
Unseen motion statistics & \BAval{t10.r04.separable} & \BAval{t10.r04.temporal.q} & \textbf{\BAval{t10.r04.bindadapt}}\\
Changed tracker backbone & \BAval{t10.r05.separable} & \BAval{t10.r05.temporal.q} & \textbf{\BAval{t10.r05.bindadapt}}\\


==> tables/slt.tex <==
LTMU & \BAval{t16.r01.tracking.precision.pct} & \BAval{t16.r01.tracking.recall.pct} & \BAval{t16.r01.fmax.pct} & \BAval{t16.r01.operating.precision.pct} & \BAval{t16.r01.operating.recall.pct} & \BAval{t16.r01.f.operating.pct}\\
KeepTrack & \BAval{t16.r02.tracking.precision.pct} & \BAval{t16.r02.tracking.recall.pct} & \BAval{t16.r02.fmax.pct} & \BAval{t16.r02.operating.precision.pct} & \BAval{t16.r02.operating.recall.pct} & \BAval{t16.r02.f.operating.pct}\\
DAM4SAM & \BAval{t16.r03.tracking.precision.pct} & \BAval{t16.r03.tracking.recall.pct} & \BAval{t16.r03.fmax.pct} & \BAval{t16.r03.operating.precision.pct} & \BAval{t16.r03.operating.recall.pct} & \BAval{t16.r03.f.operating.pct}\\
OA-VAT-PTZ & \BAval{t16.r04.tracking.precision.pct} & \BAval{t16.r04.tracking.recall.pct} & \BAval{t16.r04.fmax.pct} & \BAval{t16.r04.operating.precision.pct} & \BAval{t16.r04.operating.recall.pct} & \BAval{t16.r04.f.operating.pct}\\
Chanakya-J & \BAval{t16.r05.tracking.precision.pct} & \BAval{t16.r05.tracking.recall.pct} & \BAval{t16.r05.fmax.pct} & \BAval{t16.r05.operating.precision.pct} & \BAval{t16.r05.operating.recall.pct} & \BAval{t16.r05.f.operating.pct}\\
DAM4SAM + Chanakya-J & \BAval{t16.r06.tracking.precision.pct} & \BAval{t16.r06.tracking.recall.pct} & \BAval{t16.r06.fmax.pct} & \BAval{t16.r06.operating.precision.pct} & \BAval{t16.r06.operating.recall.pct} & \BAval{t16.r06.f.operating.pct}\\
\rowcolor{BAours}BindAdapt & \textbf{\BAval{t16.r07.tracking.precision.pct}} & \textbf{\BAval{t16.r07.tracking.recall.pct}} & \textbf{\BAval{t16.r07.fmax.pct}} & \textbf{\BAval{t16.r07.operating.precision.pct}} & \textbf{\BAval{t16.r07.operating.recall.pct}} & \textbf{\BAval{t16.r07.f.operating.pct}}\\


==> tables/sresponse.tex <==
Direct $Q$ & \BAval{t07.r01.pair.rank.pct} & \BAval{t07.r01.risk.mae} & \BAval{t07.r01.calibration.error} & \BAval{t07.r01.action.regret}\\
Temporal direct-$Q$ & \BAval{t07.r02.pair.rank.pct} & \BAval{t07.r02.risk.mae} & \BAval{t07.r02.calibration.error} & \BAval{t07.r02.action.regret}\\
Matched dependency model & \BAval{t07.r03.pair.rank.pct} & \BAval{t07.r03.risk.mae} & \BAval{t07.r03.calibration.error} & \BAval{t07.r03.action.regret}\\
\rowcolor{BAours}BindAdapt response & \textbf{\BAval{t07.r04.pair.rank.pct}} & \textbf{\BAval{t07.r04.risk.mae}} & \textbf{\BAval{t07.r04.calibration.error}} & \textbf{\BAval{t07.r04.action.regret}}\\


==> tables/sruntime.tex <==
OSTrack & \BAval{t18.r01.mean.inference.ms} & \BAval{t18.r01.p95.inference.ms} & \BAval{t18.r01.fps} & \BAval{t18.r01.decision.overhead.ms}\\
LoRATv2 & \BAval{t18.r02.mean.inference.ms} & \BAval{t18.r02.p95.inference.ms} & \BAval{t18.r02.fps} & \BAval{t18.r02.decision.overhead.ms}\\
DAM4SAM & \BAval{t18.r03.mean.inference.ms} & \BAval{t18.r03.p95.inference.ms} & \BAval{t18.r03.fps} & \BAval{t18.r03.decision.overhead.ms}\\
PVT++ & \BAval{t18.r04.mean.inference.ms} & \BAval{t18.r04.p95.inference.ms} & \BAval{t18.r04.fps} & \BAval{t18.r04.decision.overhead.ms}\\
ARTrack-AC & \BAval{t18.r05.mean.inference.ms} & \BAval{t18.r05.p95.inference.ms} & \BAval{t18.r05.fps} & \BAval{t18.r05.decision.overhead.ms}\\
OA-VAT-PTZ & \BAval{t18.r06.mean.inference.ms} & \BAval{t18.r06.p95.inference.ms} & \BAval{t18.r06.fps} & \BAval{t18.r06.decision.overhead.ms}\\
Chanakya-J & \BAval{t18.r07.mean.inference.ms} & \BAval{t18.r07.p95.inference.ms} & \BAval{t18.r07.fps} & \BAval{t18.r07.decision.overhead.ms}\\
DAM4SAM + Chanakya-J & \BAval{t18.r08.mean.inference.ms} & \BAval{t18.r08.p95.inference.ms} & \BAval{t18.r08.fps} & \BAval{t18.r08.decision.overhead.ms}\\
\rowcolor{BAours}BindAdapt & \BAval{t18.r09.mean.inference.ms} & \BAval{t18.r09.p95.inference.ms} & \BAval{t18.r09.fps} & \BAval{t18.r09.decision.overhead.ms}\\


==> tables/sstandard.tex <==
OSTrack & \BAval{t13.r01.ao} & \BAval{t13.r01.p20.pct} & \BAval{t13.r01.pn20} & \BAval{t13.r01.sr50.pct} & \BAval{t13.r01.sr75.pct} & \BAval{t13.r01.sao.pct} & \BAval{t13.r01.ssr50.pct} & \BAval{t13.r01.ssr75.pct}\\
MixFormerV2 & \BAval{t13.r02.ao} & \BAval{t13.r02.p20.pct} & \BAval{t13.r02.pn20} & \BAval{t13.r02.sr50.pct} & \BAval{t13.r02.sr75.pct} & \BAval{t13.r02.sao.pct} & \BAval{t13.r02.ssr50.pct} & \BAval{t13.r02.ssr75.pct}\\
HIPTrack & \BAval{t13.r03.ao} & \BAval{t13.r03.p20.pct} & \BAval{t13.r03.pn20} & \BAval{t13.r03.sr50.pct} & \BAval{t13.r03.sr75.pct} & \BAval{t13.r03.sao.pct} & \BAval{t13.r03.ssr50.pct} & \BAval{t13.r03.ssr75.pct}\\
ODTrack & \BAval{t13.r04.ao} & \BAval{t13.r04.p20.pct} & \BAval{t13.r04.pn20} & \BAval{t13.r04.sr50.pct} & \BAval{t13.r04.sr75.pct} & \BAval{t13.r04.sao.pct} & \BAval{t13.r04.ssr50.pct} & \BAval{t13.r04.ssr75.pct}\\
LoRATv2 & \BAval{t13.r05.ao} & \BAval{t13.r05.p20.pct} & \BAval{t13.r05.pn20} & \BAval{t13.r05.sr50.pct} & \BAval{t13.r05.sr75.pct} & \BAval{t13.r05.sao.pct} & \BAval{t13.r05.ssr50.pct} & \BAval{t13.r05.ssr75.pct}\\
LTMU & \BAval{t13.r06.ao} & \BAval{t13.r06.p20.pct} & \BAval{t13.r06.pn20} & \BAval{t13.r06.sr50.pct} & \BAval{t13.r06.sr75.pct} & \BAval{t13.r06.sao.pct} & \BAval{t13.r06.ssr50.pct} & \BAval{t13.r06.ssr75.pct}\\
KeepTrack & \BAval{t13.r07.ao} & \BAval{t13.r07.p20.pct} & \BAval{t13.r07.pn20} & \BAval{t13.r07.sr50.pct} & \BAval{t13.r07.sr75.pct} & \BAval{t13.r07.sao.pct} & \BAval{t13.r07.ssr50.pct} & \BAval{t13.r07.ssr75.pct}\\
DAM4SAM & \BAval{t13.r08.ao} & \BAval{t13.r08.p20.pct} & \BAval{t13.r08.pn20} & \BAval{t13.r08.sr50.pct} & \BAval{t13.r08.sr75.pct} & \BAval{t13.r08.sao.pct} & \BAval{t13.r08.ssr50.pct} & \BAval{t13.r08.ssr75.pct}\\
PVT++ & \BAval{t13.r09.ao} & \BAval{t13.r09.p20.pct} & \BAval{t13.r09.pn20} & \BAval{t13.r09.sr50.pct} & \BAval{t13.r09.sr75.pct} & \BAval{t13.r09.sao.pct} & \BAval{t13.r09.ssr50.pct} & \BAval{t13.r09.ssr75.pct}\\
ARTrack-AC & \BAval{t13.r10.ao} & \BAval{t13.r10.p20.pct} & \BAval{t13.r10.pn20} & \BAval{t13.r10.sr50.pct} & \BAval{t13.r10.sr75.pct} & \BAval{t13.r10.sao.pct} & \BAval{t13.r10.ssr50.pct} & \BAval{t13.r10.ssr75.pct}\\
\rowcolor{BAours}BindAdapt fixed-view & \textbf{\BAval{t13.r11.ao}} & \textbf{\BAval{t13.r11.p20.pct}} & \textbf{\BAval{t13.r11.pn20}} & \textbf{\BAval{t13.r11.sr50.pct}} & \textbf{\BAval{t13.r11.sr75.pct}} & \textbf{\BAval{t13.r11.sao.pct}} & \textbf{\BAval{t13.r11.ssr50.pct}} & \textbf{\BAval{t13.r11.ssr75.pct}}\\


==> tables/sstrata.tex <==
OSTrack & \BAval{t14.r07.short} & \BAval{t14.r07.similar} & \BAval{t14.r07.long} & \BAval{t14.r07.weighted}\\
MixFormerV2 & \BAval{t14.r08.short} & \BAval{t14.r08.similar} & \BAval{t14.r08.long} & \BAval{t14.r08.weighted}\\
HIPTrack & \BAval{t14.r09.short} & \BAval{t14.r09.similar} & \BAval{t14.r09.long} & \BAval{t14.r09.weighted}\\
ODTrack & \BAval{t14.r10.short} & \BAval{t14.r10.similar} & \BAval{t14.r10.long} & \BAval{t14.r10.weighted}\\
LoRATv2 & \BAval{t14.r11.short} & \BAval{t14.r11.similar} & \BAval{t14.r11.long} & \BAval{t14.r11.weighted}\\
LTMU & \BAval{t14.r12.short} & \BAval{t14.r12.similar} & \BAval{t14.r12.long} & \BAval{t14.r12.weighted}\\
KeepTrack & \BAval{t14.r13.short} & \BAval{t14.r13.similar} & \BAval{t14.r13.long} & \BAval{t14.r13.weighted}\\
DAM4SAM & \BAval{t14.r01.short} & \BAval{t14.r01.similar} & \BAval{t14.r01.long} & \BAval{t14.r01.weighted}\\
AD-VAT+-PTZ & \BAval{t14.r14.short} & \BAval{t14.r14.similar} & \BAval{t14.r14.long} & \BAval{t14.r14.weighted}\\
OA-VAT-PTZ & \BAval{t14.r02.short} & \BAval{t14.r02.similar} & \BAval{t14.r02.long} & \BAval{t14.r02.weighted}\\
PVT++ & \BAval{t14.r15.short} & \BAval{t14.r15.similar} & \BAval{t14.r15.long} & \BAval{t14.r15.weighted}\\
ARTrack-AC & \BAval{t14.r03.short} & \BAval{t14.r03.similar} & \BAval{t14.r03.long} & \BAval{t14.r03.weighted}\\
Chanakya-J & \BAval{t14.r04.short} & \BAval{t14.r04.similar} & \BAval{t14.r04.long} & \BAval{t14.r04.weighted}\\
DAM4SAM + joint belief & \BAval{t14.r16.short} & \BAval{t14.r16.similar} & \BAval{t14.r16.long} & \BAval{t14.r16.weighted}\\
DAM4SAM + Chanakya-J & \BAval{t14.r05.short} & \BAval{t14.r05.similar} & \BAval{t14.r05.long} & \BAval{t14.r05.weighted}\\
\rowcolor{BAours}BindAdapt & \textbf{\BAval{t14.r06.short}} & \textbf{\BAval{t14.r06.similar}} & \textbf{\BAval{t14.r06.long}} & \textbf{\BAval{t14.r06.weighted}}\\


==> tables/sswap.tex <==
Reference response / Separable & \BAval{t03.r01.sid} & \BAval{t03.r01.wrong}\\
Reference response / Joint & \BAval{t03.r02.sid} & \BAval{t03.r02.wrong}\\
BindAdapt response / Separable & \BAval{t03.r03.sid} & \BAval{t03.r03.wrong}\\
\rowcolor{BAours}BindAdapt response / Joint & \BAval{t03.r04.sid} & \BAval{t03.r04.wrong}\\


==> tables/supper.tex <==
\rowcolor{BAours}BindAdapt online & \BAval{t08.r01.sid}\\
Plus exact response & \BAval{t08.r02.sid}\\
Plus perfect acquired-frame identity & \BAval{t08.r03.sid}\\
Plus finite-action future outcomes & \BAval{t08.r04.sid}\\
Plus zero service delay & \BAval{t08.r05.sid}\\
Plus full source visibility & \BAval{t08.r06.sid}\\


==> window_numbers.tex <==
\expandafter\def\csname BAval@window.p24.ticks\endcsname{13}
\expandafter\def\csname BAval@window.p24.allcorrect\endcsname{0}
\expandafter\def\csname BAval@window.p24.allwrong\endcsname{1}
\expandafter\def\csname BAval@window.p24.allunresolved\endcsname{7}
\expandafter\def\csname BAval@window.p24.allunknown\endcsname{5}
\expandafter\def\csname BAval@window.p24.allinitial\endcsname{13}
\expandafter\def\csname BAval@window.p24.mixed\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.dam.frame\endcsname{429}
\expandafter\def\csname BAval@window.quad.f429.dam.time\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f429.dam.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f429.dam.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f429.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f429.dam.sourceage\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.dam.pubage\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f429.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f429.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.dam.frame\endcsname{435}
\expandafter\def\csname BAval@window.quad.f435.dam.time\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f435.dam.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f435.dam.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f435.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f435.dam.sourceage\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.dam.pubage\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f435.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f435.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.dam.frame\endcsname{441}
\expandafter\def\csname BAval@window.quad.f441.dam.time\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.dam.state\endcsname{W}
\expandafter\def\csname BAval@window.quad.f441.dam.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f441.dam.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f441.dam.compid\endcsname{110}
\expandafter\def\csname BAval@window.quad.f441.dam.compiou\endcsname{0.675}
\expandafter\def\csname BAval@window.quad.f441.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f441.dam.sourceage\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.dam.pubage\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f441.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f441.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.keep.frame\endcsname{429}
\expandafter\def\csname BAval@window.quad.f429.keep.time\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f429.keep.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f429.keep.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f429.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f429.keep.sourceage\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.keep.pubage\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f429.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.keep.frame\endcsname{435}
\expandafter\def\csname BAval@window.quad.f435.keep.time\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f435.keep.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f435.keep.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f435.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f435.keep.sourceage\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.keep.pubage\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f435.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.keep.frame\endcsname{441}
\expandafter\def\csname BAval@window.quad.f441.keep.time\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.keep.state\endcsname{W}
\expandafter\def\csname BAval@window.quad.f441.keep.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f441.keep.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f441.keep.compid\endcsname{110}
\expandafter\def\csname BAval@window.quad.f441.keep.compiou\endcsname{0.675}
\expandafter\def\csname BAval@window.quad.f441.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f441.keep.sourceage\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.keep.pubage\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f441.keep.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f441.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.bind.frame\endcsname{429}
\expandafter\def\csname BAval@window.quad.f429.bind.time\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f429.bind.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f429.bind.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f429.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f429.bind.sourceage\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.bind.pubage\endcsname{2.10}
\expandafter\def\csname BAval@window.quad.f429.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f429.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.bind.frame\endcsname{435}
\expandafter\def\csname BAval@window.quad.f435.bind.time\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f435.bind.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f435.bind.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f435.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f435.bind.sourceage\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.bind.pubage\endcsname{2.70}
\expandafter\def\csname BAval@window.quad.f435.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f435.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.bind.frame\endcsname{441}
\expandafter\def\csname BAval@window.quad.f441.bind.time\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.bind.state\endcsname{W}
\expandafter\def\csname BAval@window.quad.f441.bind.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f441.bind.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f441.bind.compid\endcsname{110}
\expandafter\def\csname BAval@window.quad.f441.bind.compiou\endcsname{0.675}
\expandafter\def\csname BAval@window.quad.f441.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f441.bind.sourceage\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.bind.pubage\endcsname{3.30}
\expandafter\def\csname BAval@window.quad.f441.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f441.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.p24.revisions\endcsname{0}
\expandafter\def\csname BAval@window.p25.ticks\endcsname{13}
\expandafter\def\csname BAval@window.p25.allcorrect\endcsname{0}
\expandafter\def\csname BAval@window.p25.allwrong\endcsname{0}
\expandafter\def\csname BAval@window.p25.allunresolved\endcsname{9}
\expandafter\def\csname BAval@window.p25.allunknown\endcsname{3}
\expandafter\def\csname BAval@window.p25.allinitial\endcsname{0}
\expandafter\def\csname BAval@window.p25.mixed\endcsname{1}
\expandafter\def\csname BAval@window.quad.f447.dam.frame\endcsname{447}
\expandafter\def\csname BAval@window.quad.f447.dam.time\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f447.dam.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f447.dam.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f447.dam.revision\endcsname{1}
\expandafter\def\csname BAval@window.quad.f447.dam.pubtime\endcsname{3.454}
\expandafter\def\csname BAval@window.quad.f447.dam.sourceage\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.dam.pubage\endcsname{0.45}
\expandafter\def\csname BAval@window.quad.f447.dam.sent\endcsname{2}
\expandafter\def\csname BAval@window.quad.f447.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f447.dam.postpub\endcsname{1}
\expandafter\def\csname BAval@window.quad.f453.dam.frame\endcsname{453}
\expandafter\def\csname BAval@window.quad.f453.dam.time\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f453.dam.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f453.dam.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f453.dam.revision\endcsname{1}
\expandafter\def\csname BAval@window.quad.f453.dam.pubtime\endcsname{3.454}
\expandafter\def\csname BAval@window.quad.f453.dam.sourceage\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.dam.pubage\endcsname{1.05}
\expandafter\def\csname BAval@window.quad.f453.dam.sent\endcsname{2}
\expandafter\def\csname BAval@window.quad.f453.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f453.dam.postpub\endcsname{1}
\expandafter\def\csname BAval@window.quad.f459.dam.frame\endcsname{459}
\expandafter\def\csname BAval@window.quad.f459.dam.time\endcsname{5.10}
\expandafter\def\csname BAval@window.quad.f459.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f459.dam.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f459.dam.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f459.dam.revision\endcsname{1}
\expandafter\def\csname BAval@window.quad.f459.dam.pubtime\endcsname{3.454}
\expandafter\def\csname BAval@window.quad.f459.dam.sourceage\endcsname{5.10}
\expandafter\def\csname BAval@window.quad.f459.dam.pubage\endcsname{1.65}
\expandafter\def\csname BAval@window.quad.f459.dam.sent\endcsname{2}
\expandafter\def\csname BAval@window.quad.f459.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f459.dam.postpub\endcsname{1}
\expandafter\def\csname BAval@window.quad.f447.keep.frame\endcsname{447}
\expandafter\def\csname BAval@window.quad.f447.keep.time\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f447.keep.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f447.keep.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f447.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f447.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f447.keep.sourceage\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.keep.pubage\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f447.keep.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f447.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f453.keep.frame\endcsname{453}
\expandafter\def\csname BAval@window.quad.f453.keep.time\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f453.keep.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f453.keep.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f453.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f453.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f453.keep.sourceage\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.keep.pubage\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.quad.f453.keep.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f453.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f459.keep.frame\endcsname{459}
\expandafter\def\csname BAval@window.quad.f459.keep.time\endcsname{5.10}
\expandafter\def\csname BAval@window.quad.f459.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f459.keep.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f459.keep.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f459.keep.revision\endcsname{1}
\expandafter\def\csname BAval@window.quad.f459.keep.pubtime\endcsname{4.760}
\expandafter\def\csname BAval@window.quad.f459.keep.sourceage\endcsname{5.10}
\expandafter\def\csname BAval@window.quad.f459.keep.pubage\endcsname{0.34}
\expandafter\def\csname BAval@window.quad.f459.keep.sent\endcsname{2}
\expandafter\def\csname BAval@window.quad.f459.keep.arrived\endcsname{1}
\expandafter\def\csname BAval@window.quad.f459.keep.postpub\endcsname{1}
\expandafter\def\csname BAval@window.quad.f447.bind.frame\endcsname{447}
\expandafter\def\csname BAval@window.quad.f447.bind.time\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f447.bind.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f447.bind.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f447.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f447.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f447.bind.sourceage\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.bind.pubage\endcsname{3.90}
\expandafter\def\csname BAval@window.quad.f447.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.quad.f447.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f447.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f453.bind.frame\endcsname{453}
\expandafter\def\csname BAval@window.quad.f453.bind.time\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f453.bind.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f453.bind.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f453.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f453.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f453.bind.sourceage\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.bind.pubage\endcsname{4.50}
\expandafter\def\csname BAval@window.quad.f453.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.quad.f453.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f453.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.quad.f459.bind.frame\endcsname{459}
\expandafter\def\csname BAval@window.quad.f459.bind.time\endcsname{5.10}
\expandafter\def\csname BAval@window.quad.f459.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.quad.f459.bind.id\endcsname{59}
\expandafter\def\csname BAval@window.quad.f459.bind.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f459.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.quad.f459.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.quad.f459.bind.sourceage\endcsname{5.10}
\expandafter\def\csname BAval@window.quad.f459.bind.pubage\endcsname{5.10}
\expandafter\def\csname BAval@window.quad.f459.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.quad.f459.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.quad.f459.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.p25.revisions\endcsname{1}
\expandafter\def\csname BAval@window.p27.ticks\endcsname{25}
\expandafter\def\csname BAval@window.p27.allcorrect\endcsname{9}
\expandafter\def\csname BAval@window.p27.allwrong\endcsname{4}
\expandafter\def\csname BAval@window.p27.allunresolved\endcsname{12}
\expandafter\def\csname BAval@window.p27.allunknown\endcsname{0}
\expandafter\def\csname BAval@window.p27.allinitial\endcsname{25}
\expandafter\def\csname BAval@window.p27.mixed\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.dam.frame\endcsname{164}
\expandafter\def\csname BAval@window.dance.f164.dam.time\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.dam.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f164.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f164.dam.iou\endcsname{0.938}
\expandafter\def\csname BAval@window.dance.f164.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f164.dam.sourceage\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.dam.pubage\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f164.dam.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.dam.frame\endcsname{176}
\expandafter\def\csname BAval@window.dance.f176.dam.time\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f176.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f176.dam.iou\endcsname{0.421}
\expandafter\def\csname BAval@window.dance.f176.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f176.dam.sourceage\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.dam.pubage\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f176.dam.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.dam.frame\endcsname{188}
\expandafter\def\csname BAval@window.dance.f188.dam.time\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.dam.state\endcsname{W}
\expandafter\def\csname BAval@window.dance.f188.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f188.dam.iou\endcsname{0.030}
\expandafter\def\csname BAval@window.dance.f188.dam.compid\endcsname{6}
\expandafter\def\csname BAval@window.dance.f188.dam.compiou\endcsname{0.779}
\expandafter\def\csname BAval@window.dance.f188.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f188.dam.sourceage\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.dam.pubage\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f188.dam.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.keep.frame\endcsname{164}
\expandafter\def\csname BAval@window.dance.f164.keep.time\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.keep.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f164.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f164.keep.iou\endcsname{0.938}
\expandafter\def\csname BAval@window.dance.f164.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f164.keep.sourceage\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.keep.pubage\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f164.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.keep.frame\endcsname{176}
\expandafter\def\csname BAval@window.dance.f176.keep.time\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f176.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f176.keep.iou\endcsname{0.421}
\expandafter\def\csname BAval@window.dance.f176.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f176.keep.sourceage\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.keep.pubage\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f176.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.keep.frame\endcsname{188}
\expandafter\def\csname BAval@window.dance.f188.keep.time\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.keep.state\endcsname{W}
\expandafter\def\csname BAval@window.dance.f188.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f188.keep.iou\endcsname{0.030}
\expandafter\def\csname BAval@window.dance.f188.keep.compid\endcsname{6}
\expandafter\def\csname BAval@window.dance.f188.keep.compiou\endcsname{0.779}
\expandafter\def\csname BAval@window.dance.f188.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f188.keep.sourceage\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.keep.pubage\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f188.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.bind.frame\endcsname{164}
\expandafter\def\csname BAval@window.dance.f164.bind.time\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.bind.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f164.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f164.bind.iou\endcsname{0.938}
\expandafter\def\csname BAval@window.dance.f164.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f164.bind.sourceage\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.bind.pubage\endcsname{0.30}
\expandafter\def\csname BAval@window.dance.f164.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f164.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.bind.frame\endcsname{176}
\expandafter\def\csname BAval@window.dance.f176.bind.time\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f176.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f176.bind.iou\endcsname{0.422}
\expandafter\def\csname BAval@window.dance.f176.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f176.bind.sourceage\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.bind.pubage\endcsname{0.90}
\expandafter\def\csname BAval@window.dance.f176.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f176.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.bind.frame\endcsname{188}
\expandafter\def\csname BAval@window.dance.f188.bind.time\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.bind.state\endcsname{W}
\expandafter\def\csname BAval@window.dance.f188.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f188.bind.iou\endcsname{0.030}
\expandafter\def\csname BAval@window.dance.f188.bind.compid\endcsname{6}
\expandafter\def\csname BAval@window.dance.f188.bind.compiou\endcsname{0.782}
\expandafter\def\csname BAval@window.dance.f188.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f188.bind.sourceage\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.bind.pubage\endcsname{1.50}
\expandafter\def\csname BAval@window.dance.f188.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f188.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.p27.revisions\endcsname{0}
\expandafter\def\csname BAval@window.p28.ticks\endcsname{25}
\expandafter\def\csname BAval@window.p28.allcorrect\endcsname{4}
\expandafter\def\csname BAval@window.p28.allwrong\endcsname{0}
\expandafter\def\csname BAval@window.p28.allunresolved\endcsname{21}
\expandafter\def\csname BAval@window.p28.allunknown\endcsname{0}
\expandafter\def\csname BAval@window.p28.allinitial\endcsname{25}
\expandafter\def\csname BAval@window.p28.mixed\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.dam.frame\endcsname{200}
\expandafter\def\csname BAval@window.dance.f200.dam.time\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f200.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f200.dam.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f200.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f200.dam.sourceage\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.dam.pubage\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f200.dam.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.dam.frame\endcsname{212}
\expandafter\def\csname BAval@window.dance.f212.dam.time\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.dam.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f212.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f212.dam.iou\endcsname{0.124}
\expandafter\def\csname BAval@window.dance.f212.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f212.dam.sourceage\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.dam.pubage\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f212.dam.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.dam.frame\endcsname{224}
\expandafter\def\csname BAval@window.dance.f224.dam.time\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.dam.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f224.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f224.dam.iou\endcsname{0.530}
\expandafter\def\csname BAval@window.dance.f224.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f224.dam.sourceage\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.dam.pubage\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f224.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.dance.f224.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.keep.frame\endcsname{200}
\expandafter\def\csname BAval@window.dance.f200.keep.time\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f200.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f200.keep.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f200.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f200.keep.sourceage\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.keep.pubage\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f200.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.keep.frame\endcsname{212}
\expandafter\def\csname BAval@window.dance.f212.keep.time\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.keep.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f212.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f212.keep.iou\endcsname{0.124}
\expandafter\def\csname BAval@window.dance.f212.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f212.keep.sourceage\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.keep.pubage\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f212.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.keep.frame\endcsname{224}
\expandafter\def\csname BAval@window.dance.f224.keep.time\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.keep.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f224.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f224.keep.iou\endcsname{0.531}
\expandafter\def\csname BAval@window.dance.f224.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f224.keep.sourceage\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.keep.pubage\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f224.keep.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.bind.frame\endcsname{200}
\expandafter\def\csname BAval@window.dance.f200.bind.time\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f200.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f200.bind.iou\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f200.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f200.bind.sourceage\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.bind.pubage\endcsname{2.10}
\expandafter\def\csname BAval@window.dance.f200.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f200.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.bind.frame\endcsname{212}
\expandafter\def\csname BAval@window.dance.f212.bind.time\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.bind.state\endcsname{U}
\expandafter\def\csname BAval@window.dance.f212.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f212.bind.iou\endcsname{0.124}
\expandafter\def\csname BAval@window.dance.f212.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f212.bind.sourceage\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.bind.pubage\endcsname{2.70}
\expandafter\def\csname BAval@window.dance.f212.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f212.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.bind.frame\endcsname{224}
\expandafter\def\csname BAval@window.dance.f224.bind.time\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.bind.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f224.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f224.bind.iou\endcsname{0.528}
\expandafter\def\csname BAval@window.dance.f224.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f224.bind.sourceage\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.bind.pubage\endcsname{3.30}
\expandafter\def\csname BAval@window.dance.f224.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f224.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.p28.revisions\endcsname{0}
\expandafter\def\csname BAval@window.p29.ticks\endcsname{25}
\expandafter\def\csname BAval@window.p29.allcorrect\endcsname{25}
\expandafter\def\csname BAval@window.p29.allwrong\endcsname{0}
\expandafter\def\csname BAval@window.p29.allunresolved\endcsname{0}
\expandafter\def\csname BAval@window.p29.allunknown\endcsname{0}
\expandafter\def\csname BAval@window.p29.allinitial\endcsname{25}
\expandafter\def\csname BAval@window.p29.mixed\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.dam.frame\endcsname{236}
\expandafter\def\csname BAval@window.dance.f236.dam.time\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.dam.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f236.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f236.dam.iou\endcsname{0.568}
\expandafter\def\csname BAval@window.dance.f236.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f236.dam.sourceage\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.dam.pubage\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f236.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.dance.f236.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.dam.frame\endcsname{248}
\expandafter\def\csname BAval@window.dance.f248.dam.time\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.dam.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f248.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f248.dam.iou\endcsname{0.583}
\expandafter\def\csname BAval@window.dance.f248.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f248.dam.sourceage\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.dam.pubage\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f248.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.dance.f248.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.dam.frame\endcsname{260}
\expandafter\def\csname BAval@window.dance.f260.dam.time\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.dam.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f260.dam.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f260.dam.iou\endcsname{0.562}
\expandafter\def\csname BAval@window.dance.f260.dam.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.dam.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f260.dam.sourceage\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.dam.pubage\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.dam.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f260.dam.arrived\endcsname{1}
\expandafter\def\csname BAval@window.dance.f260.dam.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.keep.frame\endcsname{236}
\expandafter\def\csname BAval@window.dance.f236.keep.time\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.keep.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f236.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f236.keep.iou\endcsname{0.568}
\expandafter\def\csname BAval@window.dance.f236.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f236.keep.sourceage\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.keep.pubage\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f236.keep.arrived\endcsname{1}
\expandafter\def\csname BAval@window.dance.f236.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.keep.frame\endcsname{248}
\expandafter\def\csname BAval@window.dance.f248.keep.time\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.keep.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f248.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f248.keep.iou\endcsname{0.583}
\expandafter\def\csname BAval@window.dance.f248.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f248.keep.sourceage\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.keep.pubage\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f248.keep.arrived\endcsname{1}
\expandafter\def\csname BAval@window.dance.f248.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.keep.frame\endcsname{260}
\expandafter\def\csname BAval@window.dance.f260.keep.time\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.keep.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f260.keep.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f260.keep.iou\endcsname{0.562}
\expandafter\def\csname BAval@window.dance.f260.keep.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.keep.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f260.keep.sourceage\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.keep.pubage\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.keep.sent\endcsname{1}
\expandafter\def\csname BAval@window.dance.f260.keep.arrived\endcsname{1}
\expandafter\def\csname BAval@window.dance.f260.keep.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.bind.frame\endcsname{236}
\expandafter\def\csname BAval@window.dance.f236.bind.time\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.bind.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f236.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f236.bind.iou\endcsname{0.566}
\expandafter\def\csname BAval@window.dance.f236.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f236.bind.sourceage\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.bind.pubage\endcsname{3.90}
\expandafter\def\csname BAval@window.dance.f236.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f236.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.bind.frame\endcsname{248}
\expandafter\def\csname BAval@window.dance.f248.bind.time\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.bind.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f248.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f248.bind.iou\endcsname{0.581}
\expandafter\def\csname BAval@window.dance.f248.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f248.bind.sourceage\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.bind.pubage\endcsname{4.50}
\expandafter\def\csname BAval@window.dance.f248.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f248.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.bind.frame\endcsname{260}
\expandafter\def\csname BAval@window.dance.f260.bind.time\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.bind.state\endcsname{C}
\expandafter\def\csname BAval@window.dance.f260.bind.id\endcsname{5}
\expandafter\def\csname BAval@window.dance.f260.bind.iou\endcsname{0.559}
\expandafter\def\csname BAval@window.dance.f260.bind.revision\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.bind.pubtime\endcsname{0.000}
\expandafter\def\csname BAval@window.dance.f260.bind.sourceage\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.bind.pubage\endcsname{5.10}
\expandafter\def\csname BAval@window.dance.f260.bind.sent\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.bind.arrived\endcsname{0}
\expandafter\def\csname BAval@window.dance.f260.bind.postpub\endcsname{0}
\expandafter\def\csname BAval@window.p29.revisions\endcsname{0}

